Type Ia Supernova Nucleosynthesis: Metallicity-Dependent Yields

Type Ia supernova explosions (SNIa) are fundamental sources of elements for the chemical evolution of galaxies. They efficiently produce intermediate-mass (with Z between 11 and 20) and iron group elements - for example, about 70% of the solar iron is expected to be made by SNIa. In this work, we calculate complete abundance yields for 39 models of SNIa explosions, based on three progenitors - a 1.4M deflagration detonation model, a 1.0 double detonation model and a 0.8 M double detonation model - and 13 metallicities, with 22Ne mass fractions of 0, 1x10-7, 1x10-6, 1x10-5, 1x10-4, 1x10-3, 2x10-3, 5x10-3, 1x10-2, 1.4x10-2, 5x10-2, and 0.1 respectively. Nucleosynthesis calculations are done using the NuGrid suite of codes, using a consistent nuclear reaction network between the models. Complete tables with yields and production factors are provided online at Zenodo: Yields. We discuss the main properties of our yields in the light of the present understanding of SNIa nucleosynthesis, depending on different progenitor mass and composition. Finally, we compare our results with a number of relevant models from the literature.

==> Chapters/miles_table_production_factors.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
  Element & A & $^{22}$Ne = 0  & 1e-7 & 1e-6 & 1e-5 & 1e-4 & 1e-3 & 2e-3 & 5e-3 & 1e-2 & 1.4e-2 & 2e-2 & 5e-2 & 1e-1 \\ 
\hline
C  & 12 & 2.85e+00 & 2.85e+00 & 2.85e+00 & 2.85e+00 & 2.85e+00 & 2.84e+00 & 2.83e+00 & 2.81e+00 & 2.79e+00 & 2.78e+00 & 2.76e+00 & 2.70e+00 & 2.61e+00  \\
C  & 13 & 2.17e-06 & 2.17e-06 & 2.16e-06 & 2.12e-06 & 2.64e-06 & 4.90e-05 & 1.31e-04 & 4.17e-04 & 9.47e-04 & 1.41e-03 & 2.19e-03 & 7.39e-03 & 1.97e-02  \\
N  & 14 & 1.02e-04 & 1.02e-04 & 1.02e-04 & 1.01e-04 & 1.14e-04 & 5.51e-04 & 1.07e-03 & 2.44e-03 & 4.41e-03 & 5.83e-03 & 7.76e-03 & 1.53e-02 & 2.34e-02  \\
N  & 15 & 1.65e+00 & 1.65e+00 & 1.65e+00 & 1.59e+00 & 1.04e+00 & 7.96e-02 & 3.11e-02 & 1.07e-02 & 6.42e-03 & 5.76e-03 & 5.87e-03 & 1.28e-02 & 4.90e-02  \\
O  & 16 & 2.94e+01 & 2.94e+01 & 2.94e+01 & 2.94e+01 & 2.95e+01 & 2.97e+01 & 2.99e+01 & 3.07e+01 & 3.16e+01 & 3.21e+01 & 3.25e+01 & 3.30e+01 & 3.15e+01  \\
O  & 17 & 7.61e-04 & 7.62e-04 & 7.67e-04 & 8.21e-04 & 1.56e-03 & 3.04e-02 & 7.10e-02 & 1.70e-01 & 2.80e-01 & 3.41e-01 & 4.08e-01 & 5.40e-01 & 5.35e-01  \\
O  & 18 & 1.33e-06 & 1.33e-06 & 1.34e-06 & 1.40e-06 & 2.36e-06 & 3.60e-05 & 8.22e-05 & 2.14e-04 & 4.33e-04 & 6.11e-04 & 8.88e-04 & 2.76e-03 & 1.06e-02  \\
F  & 19 & 4.90e-03 & 4.90e-03 & 4.87e-03 & 4.65e-03 & 3.29e-03 & 9.46e-04 & 6.58e-04 & 7.86e-04 & 1.51e-03 & 2.20e-03 & 3.32e-03 & 9.38e-03 & 1.54e-02  \\
Ne & 20 & 5.22e+00 & 5.22e+00 & 5.22e+00 & 5.22e+00 & 5.22e+00 & 5.18e+00 & 5.14e+00 & 5.03e+00 & 4.85e+00 & 4.72e+00 & 4.55e+00 & 3.93e+00 & 3.39e+00  \\
Ne & 21 & 1.17e-02 & 1.17e-02 & 1.17e-02 & 1.20e-02 & 1.42e-02 & 7.04e-02 & 1.76e-01 & 5.77e-01 & 1.36e+00 & 2.06e+00 & 3.24e+00 & 1.14e+01 & 3.27e+01  \\
Ne & 22 & 6.86e-04 & 6.89e-04 & 7.17e-04 & 9.97e-04 & 3.82e-03 & 3.38e-02 & 6.94e-02 & 1.87e-01 & 4.08e-01 & 6.05e-01 & 9.29e-01 & 3.01e+00 & 8.28e+00  \\
Na & 23 & 8.75e-01 & 8.75e-01 & 8.75e-01 & 8.73e-01 & 8.56e-01 & 7.92e-01 & 7.96e-01 & 8.64e-01 & 1.09e+00 & 1.32e+00 & 1.72e+00 & 4.55e+00 & 1.31e+01  \\
Mg & 24 & 6.45e+01 & 6.45e+01 & 6.45e+01 & 6.45e+01 & 6.45e+01 & 6.21e+01 & 5.83e+01 & 4.82e+01 & 3.67e+01 & 3.06e+01 & 2.45e+01 & 1.36e+01 & 1.29e+01  \\
Mg & 25 & 6.67e-03 & 6.67e-03 & 6.68e-03 & 6.82e-03 & 8.79e-03 & 9.03e-02 & 1.62e-01 & 4.26e-01 & 9.88e-01 & 1.53e+00 & 2.48e+00 & 9.71e+00 & 3.24e+01  \\
Mg & 26 & 3.91e-02 & 3.91e-02 & 3.92e-02 & 3.97e-02 & 4.49e-02 & 1.06e-01 & 1.68e-01 & 3.45e-01 & 6.47e-01 & 9.05e-01 & 1.32e+00 & 4.28e+00 & 1.76e+01  \\
Al & 27 & 2.36e+00 & 2.36e+00 & 2.36e+00 & 2.36e+00 & 2.33e+00 & 4.78e+00 & 8.03e+00 & 1.43e+01 & 1.96e+01 & 2.18e+01 & 2.35e+01 & 2.73e+01 & 4.14e+01  \\
Si & 28 & 4.68e+02 & 4.68e+02 & 4.68e+02 & 4.68e+02 & 4.69e+02 & 4.78e+02 & 4.84e+02 & 4.91e+02 & 4.94e+02 & 4.94e+02 & 4.94e+02 & 4.87e+02 & 4.70e+02  \\
Si & 29 & 1.77e+00 & 1.77e+00 & 1.77e+00 & 1.79e+00 & 2.19e+00 & 7.99e+00 & 1.01e+01 & 1.49e+01 & 2.14e+01 & 2.67e+01 & 3.53e+01 & 1.05e+02 & 3.96e+02  \\
Si & 30 & 1.27e+00 & 1.27e+00 & 1.26e+00 & 1.22e+00 & 9.63e-01 & 1.86e+00 & 6.10e+00 & 2.44e+01 & 5.96e+01 & 8.82e+01 & 1.31e+02 & 3.64e+02 & 8.52e+02  \\
P  & 31 & 1.44e+01 & 1.44e+01 & 1.43e+01 & 1.38e+01 & 9.58e+00 & 9.69e+00 & 1.72e+01 & 3.81e+01 & 6.89e+01 & 9.08e+01 & 1.20e+02 & 2.30e+02 & 2.64e+02  \\
S  & 32 & 5.02e+02 & 5.02e+02 & 5.02e+02 & 5.02e+02 & 4.99e+02 & 4.91e+02 & 4.88e+02 & 4.85e+02 & 4.81e+02 & 4.77e+02 & 4.69e+02 & 4.12e+02 & 3.06e+02  \\
S  & 33 & 3.65e+01 & 3.65e+01 & 3.66e+01 & 3.69e+01 & 3.97e+01 & 4.52e+01 & 5.24e+01 & 8.02e+01 & 1.16e+02 & 1.38e+02 & 1.64e+02 & 2.26e+02 & 2.06e+02  \\
S  & 34 & 2.89e-01 & 2.89e-01 & 2.87e-01 & 2.72e-01 & 1.70e-01 & 5.21e+00 & 1.56e+01 & 4.89e+01 & 1.09e+02 & 1.60e+02 & 2.40e+02 & 6.26e+02 & 9.83e+02  \\
S  & 36 & 5.07e-07 & 5.07e-07 & 5.09e-07 & 5.29e-07 & 8.40e-07 & 2.03e-03 & 1.36e-02 & 1.17e-01 & 5.38e-01 & 1.16e+00 & 2.91e+00 & 5.25e+01 & 4.79e+02  \\
Cl & 35 & 1.57e+00 & 1.57e+00 & 1.56e+00 & 1.49e+00 & 9.49e-01 & 1.95e+00 & 3.29e+00 & 6.94e+00 & 1.33e+01 & 1.83e+01 & 2.51e+01 & 3.97e+01 & 3.45e+01  \\
Cl & 37 & 2.69e+00 & 2.69e+00 & 2.69e+00 & 2.71e+00 & 2.96e+00 & 3.35e+00 & 4.08e+00 & 6.24e+00 & 9.19e+00 & 1.12e+01 & 1.37e+01 & 2.18e+01 & 2.60e+01  \\
Ar & 36 & 5.09e+02 & 5.09e+02 & 5.09e+02 & 5.09e+02 & 5.04e+02 & 4.80e+02 & 4.66e+02 & 4.43e+02 & 4.20e+02 & 4.04e+02 & 3.83e+02 & 2.90e+02 & 1.92e+02  \\
Ar & 38 & 3.48e-02 & 3.48e-02 & 3.47e-02 & 3.39e-02 & 2.49e-02 & 3.23e+00 & 8.39e+00 & 2.60e+01 & 6.10e+01 & 9.21e+01 & 1.41e+02 & 3.77e+02 & 6.11e+02  \\
Ar & 40 & 3.23e-08 & 3.23e-08 & 3.24e-08 & 3.36e-08 & 4.92e-08 & 8.59e-05 & 4.79e-04 & 3.54e-03 & 1.81e-02 & 4.60e-02 & 1.42e-01 & 3.12e+00 & 1.67e+01  \\
K  & 39 & 4.41e-01 & 4.40e-01 & 4.39e-01 & 4.21e-01 & 3.41e-01 & 3.31e+00 & 5.73e+00 & 1.15e+01 & 1.97e+01 & 2.56e+01 & 3.33e+01 & 5.48e+01 & 5.24e+01  \\
K  & 40 & 3.13e-04 & 3.13e-04 & 3.14e-04 & 3.23e-04 & 4.70e-04 & 1.06e-01 & 2.30e-01 & 7.44e-01 & 2.45e+00 & 4.68e+00 & 9.15e+00 & 2.28e+01 & 8.73e+00  \\
K  & 41 & 1.62e+00 & 1.62e+00 & 1.63e+00 & 1.71e+00 & 2.47e+00 & 5.14e+00 & 6.90e+00 & 1.12e+01 & 1.69e+01 & 2.07e+01 & 2.54e+01 & 3.66e+01 & 3.20e+01  \\
Ca & 40 & 4.11e+02 & 4.11e+02 & 4.11e+02 & 4.10e+02 & 4.06e+02 & 3.77e+02 & 3.58e+02 & 3.27e+02 & 2.97e+02 & 2.79e+02 & 2.57e+02 & 1.81e+02 & 1.15e+02  \\
Ca & 42 & 1.03e-02 & 1.02e-02 & 1.02e-02 & 9.37e-03 & 1.47e-03 & 1.44e+00 & 4.09e+00 & 1.44e+01 & 3.68e+01 & 5.77e+01 & 9.12e+01 & 2.38e+02 & 3.13e+02  \\
Ca & 43 & 2.40e-01 & 2.40e-01 & 2.36e-01 & 1.97e-01 & 1.63e-03 & 7.15e-03 & 2.01e-02 & 8.72e-02 & 2.72e-01 & 4.57e-01 & 7.53e-01 & 1.77e+00 & 2.38e+00  \\
Ca & 44 & 7.95e+00 & 7.95e+00 & 7.95e+00 & 7.94e+00 & 7.82e+00 & 7.06e+00 & 6.59e+00 & 5.82e+00 & 5.13e+00 & 4.75e+00 & 4.32e+00 & 3.02e+00 & 2.01e+00  \\
Ca & 46 & 7.65e-13 & 7.66e-13 & 7.75e-13 & 8.80e-13 & 3.08e-12 & 5.79e-08 & 9.50e-07 & 2.88e-05 & 3.67e-04 & 1.37e-03 & 5.81e-03 & 1.43e-01 & 8.16e-01  \\
Ca & 48 & 3.21e-20 & 3.24e-20 & 3.47e-20 & 5.78e-20 & 2.00e-19 & 2.33e-16 & 1.29e-14 & 1.36e-12 & 4.99e-11 & 3.44e-10 & 3.33e-09 & 1.52e-06 & 1.52e-04  \\
Sc & 45 & 4.51e-01 & 4.52e-01 & 4.57e-01 & 5.11e-01 & 9.85e-01 & 1.56e+00 & 1.90e+00 & 2.58e+00 & 3.35e+00 & 3.84e+00 & 4.41e+00 & 5.03e+00 & 4.17e+00  \\
Ti & 46 & 6.07e-03 & 6.08e-03 & 6.12e-03 & 6.31e-03 & 1.35e-02 & 1.05e+00 & 3.13e+00 & 1.21e+01 & 3.16e+01 & 4.89e+01 & 7.54e+01 & 1.84e+02 & 2.38e+02  \\
Ti & 47 & 8.17e-02 & 8.16e-02 & 8.10e-02 & 7.46e-02 & 1.78e-02 & 7.69e-02 & 1.38e-01 & 3.30e-01 & 7.29e-01 & 1.10e+00 & 1.69e+00 & 4.62e+00 & 8.48e+00  \\
Ti & 48 & 9.19e+01 & 9.19e+01 & 9.19e+01 & 9.18e+01 & 9.13e+01 & 8.70e+01 & 8.34e+01 & 7.53e+01 & 6.56e+01 & 5.95e+01 & 5.22e+01 & 3.14e+01 & 1.98e+01  \\
Ti & 49 & 2.32e+00 & 2.33e+00 & 2.38e+00 & 3.00e+00 & 2.32e+01 & 3.16e+01 & 3.68e+01 & 4.85e+01 & 6.03e+01 & 6.58e+01 & 7.04e+01 & 6.78e+01 & 6.64e+01  \\
Ti & 50 & 5.51e-13 & 5.52e-13 & 5.59e-13 & 6.35e-13 & 2.03e-12 & 2.45e-07 & 4.34e-06 & 1.38e-04 & 1.41e-03 & 3.40e-03 & 6.51e-03 & 1.63e-02 & 6.51e-02  \\
V  & 50 & 1.25e-07 & 1.25e-07 & 1.26e-07 & 1.40e-07 & 5.31e-07 & 3.59e-03 & 2.24e-02 & 3.02e-01 & 2.02e+00 & 3.96e+00 & 5.95e+00 & 1.24e+01 & 6.12e+01  \\
V  & 51 & 8.71e+00 & 8.71e+00 & 8.70e+00 & 8.59e+00 & 1.46e+00 & 1.87e+01 & 3.02e+01 & 5.41e+01 & 8.08e+01 & 9.67e+01 & 1.15e+02 & 1.68e+02 & 3.19e+02  \\
Cr & 50 & 2.71e-01 & 2.72e-01 & 2.75e-01 & 3.14e-01 & 4.24e-01 & 1.01e+01 & 2.40e+01 & 7.18e+01 & 1.63e+02 & 2.42e+02 & 3.69e+02 & 1.09e+03 & 2.02e+03  \\
Cr & 52 & 2.15e+02 & 2.15e+02 & 2.15e+02 & 2.15e+02 & 2.14e+02 & 2.06e+02 & 1.98e+02 & 1.81e+02 & 1.60e+02 & 1.47e+02 & 1.32e+02 & 1.08e+02 & 2.49e+02  \\
Cr & 53 & 2.76e+01 & 2.76e+01 & 2.78e+01 & 2.98e+01 & 5.05e+01 & 6.46e+01 & 7.64e+01 & 1.02e+02 & 1.29e+02 & 1.43e+02 & 1.58e+02 & 2.34e+02 & 5.03e+02  \\
Cr & 54 & 8.11e-10 & 8.13e-10 & 8.37e-10 & 1.15e-09 & 4.05e-08 & 1.49e-04 & 7.23e-04 & 5.89e-03 & 2.60e-02 & 5.35e-02 & 1.19e-01 & 1.25e+00 & 9.00e+00  \\
Mn & 55 & 1.95e+00 & 1.95e+00 & 1.93e+00 & 1.75e+00 & 1.98e+00 & 2.38e+01 & 3.67e+01 & 6.14e+01 & 8.71e+01 & 1.02e+02 & 1.19e+02 & 1.78e+02 & 2.89e+02  \\
Fe & 54 & 1.66e-01 & 1.66e-01 & 1.66e-01 & 1.66e-01 & 1.95e-01 & 9.67e+00 & 2.11e+01 & 5.64e+01 & 1.16e+02 & 1.65e+02 & 2.36e+02 & 5.52e+02 & 8.77e+02  \\
Fe & 56 & 3.86e+01 & 3.86e+01 & 3.86e+01 & 3.85e+01 & 3.85e+01 & 3.72e+01 & 3.61e+01 & 3.33e+01 & 3.00e+01 & 2.79e+01 & 2.55e+01 & 1.91e+01 & 1.84e+01  \\
Fe & 57 & 5.25e+00 & 5.25e+00 & 5.25e+00 & 5.27e+00 & 5.44e+00 & 6.91e+00 & 8.22e+00 & 1.12e+01 & 1.43e+01 & 1.60e+01 & 1.78e+01 & 2.16e+01 & 2.51e+01  \\
Fe & 58 & 6.56e-09 & 6.57e-09 & 6.69e-09 & 7.94e-09 & 4.87e-08 & 1.07e-05 & 3.63e-05 & 2.27e-04 & 9.20e-04 & 1.85e-03 & 3.91e-03 & 3.04e-02 & 1.37e-01  \\
Co & 59 & 5.89e-02 & 5.88e-02 & 5.84e-02 & 5.38e-02 & 4.10e-03 & 4.60e-03 & 1.10e-02 & 4.33e-02 & 1.30e-01 & 2.23e-01 & 3.96e-01 & 1.89e+00 & 4.15e+00  \\
Ni & 58 & 4.84e-01 & 4.84e-01 & 4.86e-01 & 5.01e-01 & 6.30e-01 & 1.60e+00 & 2.69e+00 & 6.08e+00 & 1.18e+01 & 1.63e+01 & 2.27e+01 & 4.76e+01 & 7.07e+01  \\
Ni & 60 & 1.85e-02 & 1.84e-02 & 1.81e-02 & 1.53e-02 & 2.82e-04 & 3.90e-04 & 1.46e-03 & 1.07e-02 & 5.00e-02 & 1.05e-01 & 2.32e-01 & 1.79e+00 & 7.02e+00  \\
Ni & 61 & 7.65e-04 & 7.64e-04 & 7.53e-04 & 6.57e-04 & 3.96e-05 & 7.27e-06 & 1.62e-05 & 7.42e-05 & 2.86e-04 & 5.94e-04 & 1.32e-03 & 1.08e-02 & 5.39e-02  \\
Ni & 62 & 1.98e-06 & 1.98e-06 & 1.99e-06 & 2.05e-06 & 2.66e-06 & 4.88e-06 & 9.59e-06 & 2.78e-05 & 6.32e-05 & 1.05e-04 & 1.99e-04 & 1.69e-03 & 1.26e-02  \\
Ni & 64 & 3.85e-20 & 3.86e-20 & 3.91e-20 & 4.42e-20 & 1.87e-19 & 5.60e-13 & 8.06e-12 & 8.66e-11 & 7.71e-11 & 7.61e-11 & 8.80e-11 & 3.73e-10 & 6.71e-09  \\
Cu & 63 & 1.43e-08 & 1.43e-08 & 1.45e-08 & 1.69e-08 & 6.90e-08 & 4.49e-08 & 1.04e-07 & 4.83e-07 & 2.21e-06 & 5.24e-06 & 1.32e-05 & 1.35e-04 & 6.42e-04  \\
Cu & 65 & 1.60e-10 & 1.60e-10 & 1.57e-10 & 1.32e-10 & 1.47e-11 & 3.36e-10 & 7.34e-10 & 2.29e-09 & 5.38e-09 & 1.17e-08 & 2.81e-08 & 2.46e-07 & 9.85e-07  \\
Zn & 64 & 2.60e-09 & 2.60e-09 & 2.60e-09 & 2.64e-09 & 6.91e-09 & 5.21e-08 & 1.37e-07 & 8.19e-07 & 3.74e-06 & 7.87e-06 & 1.70e-05 & 1.08e-04 & 2.96e-04  \\
Zn & 66 & 7.12e-12 & 7.11e-12 & 7.04e-12 & 6.37e-12 & 3.00e-12 & 2.11e-09 & 1.23e-08 & 4.20e-08 & 1.83e-08 & 1.74e-08 & 3.07e-08 & 4.01e-07 & 2.47e-06  \\
Zn & 67 & 1.89e-12 & 1.89e-12 & 1.90e-12 & 1.96e-12 & 2.30e-12 & 5.75e-12 & 1.68e-11 & 3.62e-11 & 2.29e-11 & 3.66e-11 & 8.30e-11 & 7.53e-10 & 2.73e-09  \\
Zn & 68 & 3.79e-12 & 3.79e-12 & 3.81e-12 & 4.03e-12 & 6.32e-12 & 4.06e-12 & 1.40e-11 & 3.79e-11 & 2.59e-11 & 2.80e-11 & 2.87e-11 & 6.30e-11 & 1.39e-10  \\
Zn & 70 & 2.60e-24 & 2.54e-24 & 2.55e-24 & 2.66e-24 & 8.80e-24 & 1.13e-18 & 1.28e-17 & 7.59e-17 & 2.63e-16 & 9.75e-16 & 2.37e-15 & 5.57e-17 & 2.96e-18  \\
Ga & 69 & 9.49e-14 & 9.50e-14 & 9.57e-14 & 1.03e-13 & 1.88e-13 & 4.34e-12 & 1.74e-11 & 2.75e-11 & 1.29e-11 & 1.12e-11 & 7.43e-12 & 3.06e-12 & 1.82e-11  \\
Ga & 71 & 1.34e-14 & 1.34e-14 & 1.36e-14 & 1.49e-14 & 3.74e-14 & 7.97e-14 & 3.39e-13 & 7.16e-13 & 3.87e-13 & 3.38e-13 & 2.39e-13 & 4.18e-15 & 2.02e-14  \\
Ge & 70 & 4.74e-13 & 4.75e-13 & 4.83e-13 & 5.63e-13 & 2.74e-12 & 1.73e-10 & 6.64e-10 & 1.12e-09 & 4.75e-10 & 3.30e-10 & 1.44e-10 & 2.87e-11 & 1.32e-10  \\
Ge & 72 & 6.28e-13 & 6.28e-13 & 6.31e-13 & 6.65e-13 & 9.68e-13 & 1.37e-11 & 4.65e-11 & 7.47e-11 & 5.48e-11 & 5.10e-11 & 2.78e-11 & 1.47e-14 & 3.35e-14  \\
Ge & 73 & 1.46e-14 & 1.46e-14 & 1.47e-14 & 1.59e-14 & 3.20e-14 & 4.16e-13 & 6.48e-13 & 5.17e-13 & 2.48e-13 & 1.91e-13 & 8.60e-14 & 8.40e-17 & 3.42e-16  \\
Ge & 74 & 9.90e-21 & 9.92e-21 & 1.01e-20 & 1.23e-20 & 9.05e-20 & 2.53e-16 & 1.33e-15 & 4.49e-15 & 1.44e-14 & 3.02e-14 & 2.87e-14 & 1.84e-17 & 7.74e-20  \\
Ge & 76 & 4.57e-25 & 4.60e-25 & 4.53e-25 & 4.79e-25 & 1.07e-24 & 5.66e-23 & 6.31e-22 & 5.29e-21 & 3.75e-19 & 2.40e-18 & 5.47e-18 & 1.84e-20 & 2.88e-24  \\ 
As & 75 & 4.01e-14 & 4.02e-14 & 4.03e-14 & 4.18e-14 & 5.72e-14 & 6.94e-13 & 1.96e-12 & 2.84e-12 & 1.82e-12 & 1.45e-12 & 6.28e-13 & 8.96e-17 & 2.33e-17  \\ \hline
\end{tabular}%
}


==> Chapters/model_comparisons_for_Type_Ias.tex <==
% Chapter Template

\chapter{Results of SNIa Post-Processing} % Main chapter title
\label{all_ele_analysis}



\begin{table}[]
    \centering
    \begin{tabular}{lll}
    \hline
    %Townsley       & Shen          & Miles         \\ \hline
    T1.4Z0         & S1.0Z0         & M0.8Z0        \\
    T1.4Z0.0000001 & S1.0Z0.0000001 & M0.8Z0.0000001\\
    T1.4Z0.000001  & S1.0Z0.000001  & M0.8Z0.000001 \\
    T1.4Z0.00001   & S1.0Z0.00001   & M0.8Z0.00001  \\
    T1.4Z0.0001    & S1.0Z0.0001    & M0.8Z0.0001   \\
    T1.4Z0.001     & S1.0Z0.001     & M0.8Z0.001    \\
    T1.4Z0.002     & S1.0Z0.002     & M0.8Z0.002    \\
    T1.4Z0.005     & S1.0Z0.005     & M0.8Z0.005    \\
    T1.4Z0.014     & S1.0Z0.014     & M0.8Z0.014    \\
    T1.4Z0.01      & S1.0Z0.01      & M0.8Z0.01     \\ 
    T1.4Z0.02      & S1.0Z0.02      & M0.8Z0.02     \\
    T1.4Z0.05      & S1.0Z0.05      & M0.8Z0.05     \\
    T1.4Z0.1       & S1.0Z0.1       & M0.8Z0.1      \\ \hline

    \end{tabular}
    \caption{Table showing the models presented in this chapter, from lowest metallicity to highest. Initial metallicity is exclusively represented by $^{22}$Ne.}
    \label{tab:models_explained}
\end{table}




\label{model_comparison} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

\noindent\enquote{\itshape Through me you go into eternal pain; through me you go amongst the lost people}\bigbreak

\hfill Dante Alighieri, The Inferno

\hfill

Here we present an overview of the isotopes which are over-produced relative to solar abundances in our various models. Models are labeled according to the initial mass of the progenitor and the metallicity. T1.4 corresponds to the \citet{townsley2016tracer} 1.4 M$_{\odot}$ deflagration detonation model, S1.0 the \citet{shen2018sub} 1.0 M$_{\odot}$ double detonation model, and M0.8 the \citet{miles2018quantifying} 0.8 M$_{\odot}$ model. Metallicities range from Z = 0 to Z =0.1, with the initial fraction of metals being represented by the mass fraction of $^{22}$Ne with a uniform distribution through all tracer particles. For example, T1.4Z0 corresponds to a zero metallicity, 1.4 M$_{\odot}$ model. The full list of models is shown in table \ref{tab:models_explained}. 

%Move this bit into an introduction: XXX
 
With the W7 model as a benchmark, \citet{iliadis2015nuclear} describe the nucleosynthesis during the propagation of the SN shock-wave. This shock-wave determines the burning conditions experienced by the material in the progenitor. In the innermost most extreme conditions, the material reaches densities of over 8.0x10$^{8}$\,gcm$^{-3}$. Under these conditions electron captures proceed rapidly, altering the Y$_{e}$ of the material. The Y$_{e}$ is the electron fraction, which is the ratio of electrons to baryons. This changes during the SNIa through $\beta$-decays or electron captures. Below these extreme density conditions, but still at peak temperatures in excess of 5\,GK, the material enters nuclear statistical equilibrium (NSE). NSE is a state in which all of the reaction rates, aside from the weak reactions, are in equilibrium in the system. NSE abundances are determined exclusively by three factors: the temperature, density and initial Y$_{e}$. \citet{iliadis2015nuclear} describes the further burning regimes experienced by material farther out in the WD, as the shockwave propagates forward and cools. Incomplete silicon burning, oxygen burning and neon-carbon burning proceed outwards from the center in mass shells as the peak temperature of the shockwave decreases as it moves outwards in the exploding WD. This is true for the higher mass models we investigate - T1.4 and S1.0 reach higher peak temperatures than the M0.8 model, due to their larger explosion energy. In M0.8 we see that the explosion energy is not sufficient to raise the temperature of any portion of the material above 5\,GK. This results in only products from incomplete silicon, oxygen and carbon-neon burning. A detailed discussion of the isotopic and elemental ejecta are presented in section \ref{section:yields_analysis_by_element}.

%Can this be called Si-burning - have I used the appropriate vocabulary - review paper for burning stages of SNIa XXX


\section{Selected Tables of Data}

\begin{table}
    \input{Chapters/townsley_table_production_factors}
    \caption{Production factors for T1.4 from Z = 0 to 0.1}
    \label{Tab:townsley_table_production_factors}
\end{table}{}

\begin{table}
    \input{Chapters/shen_table_production_factors}
    \caption{Production factors for S1.0 from Z = 0 to 0.1}
    \label{Tab:shen_table_production_factors}
\end{table}{}

\begin{table}
    \input{Chapters/miles_table_production_factors}
    \caption{Production factors for M0.8 from Z = 0 to 0.1}
    \label{Tab:miles_table_production_factors}
\end{table}{}



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=1\linewidth]{figures/production_isotopic_Dean_Yields_HESMA_undecayed_txt_0.eps} 
    \end{subfigure}

    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=1\linewidth]{figures/production_isotopic_Dean_Yields_HESMA_undecayed_txt_0_014.eps} 
    \end{subfigure}

    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=1\linewidth]{figures/production_isotopic_Dean_Yields_HESMA_undecayed_txt_0_1.eps} 
    \end{subfigure}

    \caption{Production factors for models T1.4Z0 (top), T1.4Z0.014 (middle) and T1.4Z0.1 (bottom). }
 \label{fig:dean_production_factors}
\end{figure}





Tables \ref{Tab:townsley_table_production_factors}, \ref{Tab:shen_table_production_factors} and \ref{Tab:miles_table_production_factors} show the production factors for the three models T1.4, S1.0 and M0.8 at all metallicities, C (Z = 6) to As (Z = 33). We now discuss the effect of metallicity of each of the three models.

In figure \ref{fig:dean_production_factors}, the isotopic production factors for models T1.4Z0, T1.4Z0.014 and T1.4Z0.1 are shown.  We observe a large overproduction in the iron group region, as well as peaks in production of Mg, Si, S, Ar and Ca isotopes. Explosive oxygen burning accounts for the majority of the production of the intermediate mass elements (Mg, Si, S and Ar) in these models, with a small contribution from trajectories reaching NSE for sulphur and argon (see section \ref{section:yields_analysis_by_element} for a full description of the burning regimes). Explosive oxygen burning is the direct fusion of two $^{16}$O nuclei, resulting in a number of possible products as described in \citet{woosley2002evolution}:

\begin{equation*} \label{eq1}
    \begin{split}
        ^{16}\mathrm{O} + {}^{16}\mathrm{O} \longrightarrow {}^{32}\mathrm{S}^{*} & \longrightarrow {}^{31}\mathrm{S} + n \\
                                                                                  & \longrightarrow {}^{31}\mathrm{P} + p \\
                                                                                  & \longrightarrow {}^{28}\mathrm{Si} + \alpha
    \end{split}
\end{equation*}

We see production of the intermediate mass elements in the range of 2-5 GK, lighter elements being produced preferentially in cooler conditions. we therefore observe both carbon burning (T$_{9} \sim$ 2 GK) and explosive oxygen burning (T$_{9} \sim$ 3 GK). In the lower peak temperature regime, rates of photodisintegration are low and fusion dominates. In the higher temperature explosive burning, these rates are similar. The majority of burning however follows the reactions stated above - the three decay channels of $\mathrm{S}^{*}$ - which have varying branching ratios which determine the most likely products. $^{28}$Si and $^{32}$S constitute 90\% of the products of oxygen burning \citep{woosley2002evolution}.


%\citet{hirschi2015evolution}
%\citet{el2004evolution} describe oxygen burning in the context of massive stars



%$$ ^{24}\mathrm{Mg} + \alpha \longrightarrow {}^{28}\mathrm{Si} + \gamma$$
%$$ ^{28}\mathrm{Si} + \alpha \longrightarrow {}^{32}\mathrm{S} + \gamma$$

%up to (in principle) $^{56}$Ni in the case of T1.4Z0 $^{44}$Ti is produced only in trace amounts in the outer layers of the SN explosion

The $\alpha$ chain isotopes are produced through freeze out from NSE. These are $^{24}$Mg, $^{28}$Si, $^{32}$S and $^{36}$Ar. 
%Alpha particles are produced through the destruction of $^{12}$C and $^{16}$O as the shock wave passes through the outer layers of the white dwarf, which are then captured on remaining $^{12}$C and $^{16}$O seed nuclei. 
The large peak in production in the iron group arises from the complete destruction of the $^{12}$C and $^{16}$O nuclei to $\alpha$ particles, and their subsequent recombination, as the temperature drops after the passing of the shock wave. For a given Z in the low to intermediate mass isotopes (A < 45), the lightest stable nucleus of that element is the most overproduced at low metallicities. As the metallicity of the system increases, we see a boost in production of the heavier isotopes of a given element. The bulk of the iron group material is formed in the freeze out from NSE, at high central densities. These high density regions modify the Y$_{e}$ of the material undergoing nucleosynthesis through electron capture reactions, resulting in a less pronounced dependence on the initial metallicity of the progenitor. 

\citet{brachwitz2000role} discuss in detail the effect of electron capture rates and the Y$_{e}$ of the progenitor on the ejected composition of the iron group ejecta, finding that their improved electron capture rates determined through a shell model monte carlo simulation changes the production of $^{48}$Ca, $^{48}$Ti, $^{54}$Cr, $^{54,58}$Fe, and $^{58}$Ni. This effect is seen in the composition of the iron group in figure \ref{fig:dean_production_factors}, where the changing Y$_{e}$ is caused by the initial composition shift from T1.4Z0.0 to T1.4Z0 rather than through a change in the electron capture rates. $^{58}$Ni increases by a factor of 2 between the Z = 0 and Z = 0.1 panels. An even larger effect on the abundance of $^{54}$Fe is observed - increasing by a factor of 5 between the same models. Conversely, in the lower iron group region ($^{48}$Ca, $^{48}$Ti) we do not see this same strong dependency on the Y$_{e}$ of the progenitor, for $^{48}$Ti production is consistent across the range of metallicities investigated, for $^{48}$Ca production is very low - going from 1.62x10$^{-12}$ to 6.94x10$^{-12}$ across the metallicity range. Although there is a factor of 4 difference in production, the is only a trace amount of $^{48}$Ca ejected from the system. 

\citet{brachwitz2000role} find that odd-odd nuclei and odd-A nuclei have the largest effect on the Y$_{e}$ of the SNIa explosion. The choice of electron capture reactions for these nuclei in particular are therefore key to our post-processing results. Our Weak rates are taken from \citet{langanke2000shell} and \citet{langanke2001rate}. Gamow-Teller back resonances in astrophysical conditions significantly boost electron capture rates \citep{brachwitz2000role}. Due to the dense conditions in the SNIa explosion, forbidden transitions are negligible and these resonances dominate \citep{fuller1982stellar}. In addition to this \citet{fuller1982stellar} also highlight the importance of the neutron closed shells in SNIa nucleosynthesis, which block further electron captures.    

The middle panel of figure \ref{fig:dean_production_factors} illustrates the effect of the decreased Y$_{e}$ in this model. Through the span of our models we range from a Y$_{e}$ of 0.5 at Z = 0, to a value of Y$_{e}$ of 0.495 at Z = 0.1. We see a significant boost in the production of heavier isotopes in the A < 50 region, and some change in the production in the central region. The odd-even effect begins to appear in the isotopic chains (it is already apparent from the absence of, for example, an overproduction of Al) as the numbers of free neutrons in the supernova increases. We see that there is a larger overproduction of even-even isotopes, due to the larger neutron capture cross-section for those nuclei with odd numbers of neutrons. The odd-even effect is more pronounced in the T1.4Z0.1 run, and the nucleosynthesis shifts in all regions to more neutron rich isotopes, due to the decreased Y$_{e}$. %We see also the effect in the freeze out region, this is again less pronounced than in the A < 50 region due to the electron captures effecting the Y$_{e}$.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=1\linewidth]{figures/production_isotopic_Shen_Yields_HESMA_undecayed_txt_0.eps} 
    \end{subfigure}

    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=1\linewidth]{figures/production_isotopic_Shen_Yields_HESMA_undecayed_txt_0_014.eps} 
    \end{subfigure}

    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=1\linewidth]{figures/production_isotopic_Shen_Yields_HESMA_undecayed_txt_0_1.eps} 
    \end{subfigure}

    \caption{Production factors for models S1.0Z0 (top), S1.0Z0.014 (middle) and S1.0Z0.1 (bottom). }
 \label{fig:shen_production_factors}
\end{figure}

Comparing figures \ref{fig:dean_production_factors} and \ref{fig:shen_production_factors}, S1.0Z0 shows a similar distribution to T1.4Z0 in the A < 50 region, the iron group region is less abundant and efficient production in a given element is spread over a smaller number of isotopes. Trends for the A < 50 isotopes are similar between S1.0Z0 and T1.4Z0, and S1.0Z0.014 and T1.4Z0.014, as these are produced in very similar conditions between the two sets of model. While the most abundant isotopes of a given iron group element are produced in broadly the same proportion as for the T1.4 cases, heavier isotopes of a given element are less produced than in their T1.4 counterpart - $^{64}$Ni has a production factor of 1.16 in the T1.4Z0 model, 17 orders of magnitude larger than the S1.0Z0 model. Similarly, the are 11 orders of magnitude difference in the $^{58}$Fe production factor. 

Increasing the initial metallicity from Z = 0 to Z = 0.014 results in a small overproduction of Ge in the S1.0Z0.014 model. In the S1.0Z0.1 model it results in a further boost, however a number of different elements synthesised in the SN explosion remains the same. We see a similar distribution of the iron group isotopic production factors between T1.4Z0.1 and S1.0Z0.1 as well as in the lower mass region.



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=1\linewidth]{figures/production_isotopic_Brox_Yields_HESMA_undecayed_txt_0.eps} 
    \end{subfigure}

    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=1\linewidth]{figures/production_isotopic_Brox_Yields_HESMA_undecayed_txt_0_014.eps} 
    \end{subfigure}

    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=1\linewidth]{figures/production_isotopic_Brox_Yields_HESMA_undecayed_txt_0_1.eps} 
    \end{subfigure}

    \caption{Production factors for models M0.8Z0 (top), M0.8Z0.014 (middle) and M0.8Z0.1 (bottom). }
 \label{fig:brox_production_factors}
\end{figure}


M0.8Z0 shows a large reduction in the production of iron group isotopes as compared with T1.4Z0 and S1.0Z0, and a reduction in the maximum proton number reached with nucleosynthesis stopping at Ni. Lower mass nuclei such as Si and S dominate, as none of the material in the explosion reaches NSE conditions. The majority of the ejecta is dominated by the products of explosive C and explosive O burning. Whilst the distributions of production factors for individual isotopes is similar, there are significant differences in the magnitude of production between the three Z = 0.1 models. Fe, for instance, is highly suppressed in the M0.8Z0.1 model, where as Cr remains unchanged within a factor of 5 for $^{52}$Cr - the most abundant isotope of Cr. 

%NITROGEN in one of these - FLAG



\section{Yields Analysis By Element} \label{section:yields_analysis_by_element}

In this section we describe the production of each stable isotope of each element between C and Se, for each of the three classes of model investigated. Where possible, in the cooler non-NSE regimes, we highlight the key reactions which drive the production of the stable isotopes and their radiogenic contributions. 

\subsection{Oxygen}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/O_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/O_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/O_brox_yields_.eps} 
    \end{subfigure}

 \caption{
     The ejected mass for the element O and its stable isotopes is shown with respect to initial metallicity. The elemental yields take into account radiogenic contributions. For isotopes, decayed and undecayed abundances are shown (continuous lines with crosses and dot-dashed lines with empty circles, respectively). Data is presented for the T1.4 (upper panel), S1.0 (middle panel) and M0.8 (lower panel).
 }
 \label{fig:Oxygen_metalicity_multi}
\end{figure}





\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_O__16.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_O__16.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_O__16.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_O__16.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_O__16.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_O__16.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_O__16.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_O__16.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_O__16.eps} 
    \end{subfigure}
    
    

 \caption{Top panels: The $^{16}$O abundance is shown with respect to the explosion temperature peak (continuous black line) for the models T1.4Z0 (left), T1.4Z0.014 (middle) and T1.4Z0.1 (right) at Z=0, Z=0.014 and Z=0.1, respectively. $^{16}$O abundances are shown with contributions from radioactive species, which are negligible in this case.
 Middle Panels: As for top panels, but for models S1.0Z0, S1.0Z0.014 and S1.0Z0.1, respectively.
 Bottom Panels: As for top panels, but for models M0.8Z0, M0.8Z0.014 and M0.8Z0.1, respectively.}
 \label{fig:o_16_radiogenic}
\end{sidewaysfigure}




\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_O__17.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_O__17.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_O__17.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_O__17.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_O__17.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_O__17.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_O__17.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_O__17.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_O__17.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{17}$O are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:o_17_radiogenic}
\end{sidewaysfigure}








\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_O__18.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_O__18.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_O__18.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_O__18.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_O__18.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_O__18.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_O__18} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_O__18.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_O__18.eps} 
    \end{subfigure}
    
    

    \caption{The abundance distributions of $^{18}$O are shown, arranged as in figure \ref{fig:o_16_radiogenic}. Radiogenic contributions from $^{18}$F are highlighted.}
 \label{fig:o_18_radiogenic}
\end{sidewaysfigure}


Oxygen has 3 stable isotopes: $^{16}$O, $^{17}$O and $^{18}$O. SNIa are not expected to be a significant source of oxygen - $^{16}$O is largely produced in massive stars during He burning, $^{17}$O is synthesised in novae in the hot CNO cycle \citep{romano2017evolution}, and $^{18}$O is a product of partial He burning, again in massive stars \citep{woosley2002evolution}. \citet{kobayashi2020origin} show that without novae, the evolution of [O/H] vs [Fe/H] can be reproduced for the Milky Way, due to the relatively low abundance of  $^{17}$O and $^{18}$O.

Figure \ref{fig:Oxygen_metalicity_multi} shows our first plot of ejected mass vs metallicity, here for oxygen. These plots are arranged with three panels, the most massive T1.4 models are shown in the top panels, next in the middle panel is the S1.0 models, and in the bottom panel the M0.8 models. Radiogenic contributions are given by the difference between the solid, decayed lines for a given isotope and the dashed lines showing direct production of that isotope. The total ejected elemental mass is also shown with a solid black line.

In figure \ref{fig:Oxygen_metalicity_multi} we show the total ejected mass of elemental oxygen as a function of Z for each model increases with decreasing mass of the progenitor. The oxygen ejected in our models is the unburnt fuel remaining after the explosion, which there is more of in the lower mass model M0.8. We see a very weak trend with metallicity leading to a increase in the ejected mass of  of $^{16}$O with increasing initial metallicity. In model T1.4, we go from an ejected mass of $^{16}$O of 5.37x10$^{-2}$ at Z = 0 to 5.68x10$^{-2}$ at Z = 0.1, the S1.0 models increase from 4.81 to 5.12x10$^{-2}$, and the M0.8 models from 1.79 to 1.91x10$^{-1}$. In all models we see a secondary component contribution to $^{17}$O and $^{18}$O, with similar behavior for all three masses of model, a rise in abundance beginning at Z = 10$^{-4}$ and rising to an ejected mass of approximately 10$^{-7}$M$_{\odot}$ at around solar metallicity, before plateauing. 

Figure \ref{fig:o_16_radiogenic} is the first 9-panel plot in this work. In it, the models investigated are shown in three rows, from T1.4 models in the top row to S1.0 in the middle and M0.8 in the bottom row. In the columns from left to right we increase the initial metallicity from Z = 0 to Z = Z$_{\odot}$ to Z = 0.1. In each of these 9 panels, the peak temperature of each particle is shown on the x-axis, the y-axis shows the mass fraction of a given isotope at in each trajectory at the end of nucleosynthesis. We note an artefact in the plots of the S1.0 models due to the relative sparsity of data (10$^{2}$ particles compared to 10$^{4}$ for the T1.4 and M0.8 models). Because of this the data, at times, appears incomplete in these figures. Where this occurs, we discuss the trends as the would appear without these effects. The use of peak temperature as the defining characteristic for a particle is important for those trajectories in two dimensions, as a simple radial distance would not represent the trends seen in the T1.4 models correctly. Because of this, the trajectories are sorted in order of peak temperature which can be seen to give smooth trends in all models. This is due to the nucleosynthesis being largely defined by the peak temperature of a given trajectory, and to a lesser extent in the more dense models, the peak density of a trajectory.

In figures \ref{fig:o_16_radiogenic}, \ref{fig:o_17_radiogenic} and \ref{fig:o_18_radiogenic} the abundance profile of the ejecta is shown with respect to the peak temperature during the NS explosion. Most of the ejected $^{16}$O comes from the peak temperature range of between 1 and 3.5 GK. This is due to the oxygen fuel remaining unburnt in these relatively cooler regions, which only ignite carbon. Production of $^{17}$O and $^{18}$O in the 1.5 - 2.5 GK range, where 1.5 GK corresponds to the lowest peak temperatures experienced in these three models. Nucleosynthesis is very similar between our set of three models for the production of oxygen. Production of $^{17}$O and $^{18}$O is highly metallicity dependent. Production of $^{17}$O begins at approximately Z = $10^{-4}$ for all models. The sparsity of the data for the S1.0 models does not show production of $^{17}$O at Z = 0 and Z = Z$_{\odot}$, or $^{18}$O for the same metallicities. It can be seen in figure \ref{fig:o_17_radiogenic} however that $^{18}$O has a large radiogenic contribution from $^{18}$F at solar metallicity. This decreases as the initial $^{22}$Ne content of the white dwarf is increased, and at super-solar metallicities it is produced directly as $^{18}$O, with a very small contribution from $^{18}$F of less than 1 percent. 

For $^{16}$O (figure \ref{fig:o_16_radiogenic}), we see that the ejected mass from unburnt $^{16}$O is relatively insensitive to initial metallicity. Differences occur in the intermediate peak temperature range - between 4 and 7\,GK - where destruction of $^{16}$O is more efficient at higher metallicities. We see that no oxygen is ejected above approximately 4 GK in any model, due to its complete burning.





\subsection{Neon}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ne_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ne_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ne_brox_yields_.eps} 
    \end{subfigure}

 \caption{
     As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Ne, and its stable isotopes $^{20}$Ne, $^{21}$Ne and $^{22}$Ne.
 }
 \label{fig:Neon_metalicity_multi}
\end{figure}



Neon has 3 stable isotopes: $^{20}$Ne, $^{21}$Ne and $^{22}$Ne. $^{20}$Ne is by far the dominant contributor to elemental neon abundance in the Solar System, contributing over 90\% . SNIa are not a major contributor to the abundance of elemental neon in the galaxy. \citet{pignatari2016nugrid} show that neon is mostly produced as $^{20}$Ne in massive stars. \citet{woosley2002evolution} identify neon production as occurring during carbon burning. We can see that only trace amounts of neon are produced above 4 GK in our models (that trace amount being produced as $^{20}$Ne), the rest is processed in the outer, cooler layers of the WD in conditions similar to carbon burning. $^{21}$Ne is also produced by carbon burning in massive stars, and $^{22}$Ne in helium burning. In the models presented in this work, the mass fraction of $^{22}$Ne is set as an initial condition for the composition of the WD, with a uniform distribution through all tracer particles. This is as a proxy for the metallicity of the fuel. Careful consideration must therefore be given to our reported ejected abundances of $^{22}$Ne, as the initial conditions of our simulations have $^{22}$Ne as the sole source of metals, and abundances of $^{22}$Ne from these models may differ substantially from values obtained from the nucleosynthesis in the progenitor WD. 
 

From figure \ref{fig:Neon_metalicity_multi} we see that there is a strong metallicity dependency for the production of both $^{21}$Ne and $^{22}$Ne, in the higher mass models a sharp increase in the secondary production of these isotopes is observed around Z = 10$^{-4}$, where as for production of $^{22}$Ne this begins at Z = 10$^{-5}$.



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_NE_20.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_NE_20.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_NE_20.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_NE_20.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_NE_20.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_NE_20.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_NE_20.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_NE_20.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_NE_20.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{20}$Ne are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ne_20_radiogenic}
\end{sidewaysfigure}

$^{20}$Ne is produced here by alpha captures on $^{16}$O, as shown by its large production in the oxygen burning regions of figure \ref{fig:ne_20_radiogenic}. As can be seen in figure \ref{fig:ne_20_radiogenic}, there is a decrease in the amount of $^{20}$Ne produced at intermediate peak temperatures (between 5.5 and 7\,GK here) in models T1.4Z0.014, T1.4Z0.1, S1.0Z0.14 and S1.0Z0.1 and in all models at lower peak temperatures due to the increasing metallicity. This decrease is larger than the increased production of other isotopes of neon, and we see from figure \ref{fig:Neon_metalicity_multi} that this results in a decrease in the total ejected mass of elemental Ne. There is no significant radiogenic contribution to the abundance of $^{20}$Ne in any of the models investigated here. 




\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_NE_21.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_NE_21.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_NE_21.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_NE_21.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_NE_21.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_NE_21.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_NE_21.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_NE_21.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_NE_21.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{21}$Ne are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ne_21_radiogenic}
\end{sidewaysfigure}

$^{21}$Ne is produced largely as a secondary isotope through the $^{20}$Ne(n,$\gamma$)$^{21}$Ne reaction. While trace amounts are produced in the T1.4, S1.0 and M0.8 models at Z = 0, production increases significantly as the initial metallicity is increased due to the increased availability of neutrons in the system. We see a small primary production in the intermediate peak temperature region only in the Z = 0 models. This production is negligible compared to the increase in production at lower peak temperatures between 1 and 3\,GK. At zero metallicity there is a non negligible contribution to the overall production from $^{21}$Na of the order of a few percent. On the other hand, there is no significant radiogenic contribution to $^{21}$Ne above Z = 0.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_NE_22.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_NE_22.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_NE_22.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_NE_22.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_NE_22.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_NE_22.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_NE_22.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_NE_22.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_NE_22.eps} 
    \end{subfigure}
    
    

    \caption{The abundance distributions of $^{22}$Ne are shown, arranged as in figure \ref{fig:o_16_radiogenic}. Radiogenic contributions from $^{22}$Na are included.}
 \label{fig:ne_22_radiogenic}
\end{sidewaysfigure}

The total ejected mass of $^{22}$Ne from our models is likely to be an overestimate, due to unprocessed $^{22}$Ne in the outer layers of the WD which remain after the shockwave has passed through. We are unable to quantify the correct abundance of $^{22}$Ne without a full initial abundance profile for the progenitor. Such work has been undertaken by \citet{battino2020heavy}, who show that due to the neutron flux in the accretion phase of the WD, $^{22}$Ne can be depleted in the outer layers of the WD prior to explosion. It is unlikely that the abundances will vary hugely from those in our outer layer however, as most of the material in the outer layers will be CNO, which is processed to $^{22}$Ne.  




\subsection{Magnesium}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Mg_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Mg_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Mg_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Mg, and its stable isotopes $^{24}$Mg, $^{25}$Mg and $^{26}$Mg.
 }
 \label{fig:Magnesium_metalicity_multi}
\end{figure}

Magnesium has 3 stable isotopes: $^{24}$Mg, $^{25}$Mg and $^{26}$Mg. The isotopes of magnesium are primarily formed in carbon and neon burning \citep{woosley2002evolution} and are not produced in SNIa efficiently. $^{24}$Mg is the most abundant isotope of magnesium, and in our models magnesium is primarily ejected as $^{24}$Mg. There is a strong metallicity trend for all isotopes and the relative ratios of these change significantly over the metallicity range investigated in this work. 

$^{24}$Mg is usually a primary isotope, being formed by $\alpha$ captures on $^{20}$Ne, however the observed trend of decreasing $^{24}$Mg abundance above Z = 10$^{-3}$ in these models is due to the reaction $ ^{24}\mathrm{Mg}(n,\gamma){}^{25}\mathrm{Mg} $ with the neutrons produced by the reaction $^{22}$Ne($\alpha$,n)$^{25}$Mg. We may therefore expect the specifics of nucleosynthesis in the cooler outer layers of the WD to be dependent on both the $^{22}$Ne abundance and the rate of the reaction producing neutrons. Below Z = 10$^{-3}$ the abundance of $^{22}$Ne provides an insufficient flux of neutrons to change $^{24}$Mg production. 


Figure \ref{fig:Magnesium_metalicity_multi} presents the isotopic and elemental ejected masses of the three stable isotopes of magnesium. All models show a decrease in the ejected mass of elemental Mg at metallicities in the region of solar. As we reach super-solar metallicities, the elemental abundance of Mg increases again, as the decrease in $^{24}$Mg begins to plateau and the significant increase in both $^{25}$Mg and $^{26}$Mg begins to compensate for the lost mass from $^{24}$Mg. Secondary contributions to the abundances of $^{25}$Mg and $^{26}$Mg begin in the Z=10$^{-4}$ region, increasing abundances of these by over 3 orders of magnitude in all models. This is linear with the increase in $^{22}$Ne for $^{25}$Mg, and with a steeper increase for $^{26}$Mg.


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_MG_24.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_MG_24.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_MG_24.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_MG_24.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_MG_24.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_MG_24.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_MG_24.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_MG_24.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_MG_24.eps} 
    \end{subfigure}
    
    

    \caption{The abundance distributions of $^{24}$Mg are shown, arranged as in figure \ref{fig:o_16_radiogenic}. Radiogenic contributions from $^{24}$Na and $^{24}$Ne are shown, which become significant at Z $\geq$ Z$_{\odot}$}
 \label{fig:mg_24_radiogenic}
\end{sidewaysfigure}


Figure \ref{fig:mg_24_radiogenic} shows the contributions to the production of $^{24}$Mg at different peak temperatures. The decrease with increasing metallicity comes largely from decreased production at low peak temperatures, where we see from figure \ref{fig:mg_24_radiogenic} the peak production in the 2 - 3.5 GK range has fallen from a mass fraction of greater than 10\% to a few percent between models T1.4Z0 and T1.4Z0.1. We see that the radiogenic contribution to $^{24}$Mg increases in all models as the initial metallicity increases, with $^{24}$Na becoming a contributor to the ejecta from lower peak temperature regions at Z=0.1, although it remains negligible. This $^{24}$Na is produced in the series of reactions

$$ ^{22}\mathrm{Ne}(n,\gamma) {}^{23}\mathrm{Ne}(n,\gamma) {}^{24}\mathrm{Ne} (\beta^{-}) {}^{24}\mathrm{Na}  , $$

the neutron flux required is again supplied by the $^{22}$Ne($\alpha$,n)${}^{25}$Mg reaction.

From figure \ref{fig:mg_24_radiogenic} we note that there is no significant contribution from radiogenic sources to the abundance $^{24}$Mg at any metallicity. There is also a small contribution from $^{24}$Na but this is negligible, as seen across all models.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_MG_25.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_MG_25.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_MG_25.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_MG_25.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_MG_25.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_MG_25.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_MG_25.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_MG_25.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_MG_25.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{25}$Mg are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:mg_25_radiogenic}
\end{sidewaysfigure}

In the T1.4Z0 model, we see that there is a significant contribution to the ejected $^{25}$Mg from $^{25}$Al (Figure \ref{fig:mg_25_radiogenic}) in the intermediate peak temperature range. Under these conditions the majority of $^{25}$Mg is produced as $^{25}$Al. As can be seen in the T1.4Z0 panel, this is not the largest contributor to the ejected mass of $^{25}$Mg in this model. This comes from the cooler outer layers of the explosion, where the majority of $^{25}$Mg is synthesised by the $^{22}$Ne($\alpha$,n)$^{25}$Mg reaction. 

%This secondary production is driven by the reaction XXXX (notes here from marco - can I check this somehow though?). 

We observe an interesting trend in the T1.4 models, whereby the intermediate temperature peak region ceases to contribute to the ejected $^{25}$Mg mass as we increase the initial metallicity. This is more than compensated for by the increase in production at lower peak temperatures across the models. We therefore conclude that $^{25}$Mg is produced as both a primary isotope, in the hotter regions, and a secondary one in the cooler outer layers. %This holds true for the production of $^{25}$Al in the T1.4 models.

A similar trend is observed in the S1.0 models, where we observe some production of $^{25}$Al in the intermediate peak temperature layers, here around the 6\,GK range (the hottest peak temperatures for this model). We observe the secondary production of $^{25}$Mg, again directly as $^{25}$Mg for the most part. Figure \ref{fig:mg_25_radiogenic} reveals the relatively small impact these radiogenic contributions have to the overall ejected mass of $^{25}$Mg across all models.

For the M0.8 models, we see that production is concentrated in the outer layers and is strongly dependent on metallicity, as is seen in the other two models. The production peak in the outer layers of M0.8Z0.1 is very similar to that of both T1.4Z0.1 and S1.0Z0.1, with the temperature range over which $^{25}$Mg is produced being more similar to the S1.0 model, as we see a small shift in the tail of production from the T1.4Z0.1 model from 4.5 to 4 GK. Peak production for all models lies at approximately 2.4 GK however, so we can conclude that burning conditions in this region are very similar between the three sets.




\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_MG_26.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_MG_26.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_MG_26.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_MG_26.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_MG_26.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_MG_26.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_MG_26.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_MG_26.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_MG_26.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{26}$Mg are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:mg_26_radiogenic}
\end{sidewaysfigure}


$^{26}$Mg has significant radiogenic contributions to ejected mass in all models at Z=0. We see a broad production of $^{26}$Mg as $^{26}$Si and $^{26}$Al in the T1.4Z0 model - $^{26}$Si in the intermediate peak temperature region (4 GK - 6 GK) and $^{26}$Al in the lower peak temperature region, with a more complicated interplay in the 4 - 5\,GK range, where both Si and Al are produced in similar quantities. We can look at this nucleosynthesis as a superposition of the lower and intermediate peak temperature region nucleosynthesis. Direct production of $^{26}$Mg does occur in the outer regions of the SNIa explosion, however it does not constitute the majority of the total ejected $^{26}$Mg. As the metallicity increases in the T1.4 models, we see a dramatic change in the nucleosynthesis. Intermediate peak temperature production is eliminated, and the outer layers of the explosion dominate, with a large increase in the ejected mass from these trajectories which more than compensates for this as can be seen in figure \ref{fig:Magnesium_metalicity_multi}. We also see a swap to the dominant nucleosynthesis channel being direct synthesis of $^{26}$Mg, with a broad contribution from $^{26}$Al. $^{26}$Si production is eliminated. At super-solar metallicities (T1.4Z0.1) that direct synthesis of $^{26}$Mg dominates, with a decreased contribution from $^{26}$Al. We concluded that $^{26}$Mg is produced directly as a secondary isotope in SNIa explosions in the T1.4 set of models.

In the S1.0Z0 models production of $^{26}$Mg is dominated at all temperatures by radiogenic contributions from $^{26}$Al. As we increase our initial metallicity, direct production of $^{26}$Mg is again boosted by the supply of neutrons from the $^{22}$Ne($\alpha$,n) reaction. Contributions from the $^{22}$Ne($\alpha$,$\gamma$)$^{26}$Mg channel are negligible at the temperatures where $^{26}$Mg is produced in this model, as the cross section for the ($\alpha$,$\gamma$) reaction are three orders of magnitude smaller than for the ($\alpha$,n), due to resonances. We also observe an increase in the amount of $^{26}$Al produced, due to the increased production of $^{25}$Mg and subsequent (p,$\gamma$) reactions. As with the T1.4Z0.1 model, the production of $^{26}$Al decreases again in the S1.0Z0.1 model, and $^{26}$Mg is dominated by direct synthesis.

Similar trends are observed in the M0.8 models, with an increase in the production of radiogenic $^{26}$Al boosting production of $^{26}$Mg in the Z = Z$_{\odot}$ model. This decreases as the metallicity increases to super-solar values. In all models at Z > 0.014, there is no production in the intermediate peak temperature range as identified in the Z = 0 models.


\subsection{Aluminium}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Al_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Al_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Al_brox_yields_.eps} 
    \end{subfigure}

 \caption{
     As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of $^{27}$Al.
 }
 \label{fig:Aluminium_metalicity_multi}
\end{figure}

Aluminium is mono-isotopic, with only $^{27}$Al being stable. the primary production site of aluminium is carbon and neon burning in CCSN \citep{woosley2002evolution} with similar conditions for production to $^{25}$Mg and $^{26}$Mg \citep{pignatari2016nugrid}. Figure \ref{fig:Aluminium_metalicity_multi} shows the dependence of the elemental aluminium production on initial metallicity. Al production does generally increase with increasing metallicity for all models, with a plateau around the solar metallicity region. Production is nearly flat for Z $\leq$ 10$^{-4}$ with a significant radiogenic contribution from $^{27}$Si. This radiogenic contribution decreases with increasing metallicity. We see that there is a significant radiogenic contribution only in the lower metallicity T1.4 models, above Z=10$^{-4}$ almost all material is produced directly as $^{27}$Al. At lower metallicities, particularly in the T1.4Z0 model, the radiogenic contribution is on the order of 50\% of the total ejected mass of $^{27}$Al. The primary radiogenic contribution shifts both in species from $^{27}$Si to $^{27}$Mg and in temperature range, from peak production of radioisotpes in the 2-4 GK range down to a more localised production around 2 GK. This is the odd even effect, observed in a variety of SN scenarios (see, for example \citet{kozyreva2014explosion}) 

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_AL_27.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_AL_27.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_AL_27.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_AL_27.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_AL_27.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_AL_27.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_AL_27.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_AL_27.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_AL_27.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{27}$Al are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:al_27_radiogenic}
\end{sidewaysfigure}


We see from figure \ref{fig:al_27_radiogenic} that there is a significant contribution to the abundance of $^{27}$Al in the T1.4Z0 model from $^{27}$Si over a broad range of temperatures. Production of $^{27}$Si ranges from around 1.5 to 5.5\,GK, over the majority of which this silicon component is comparable to the direct production of $^{27}$Al and is the dominant source of $^{27}$Al over much of this temperature range. In the S1.0Z0 and M0.8Z0 models, while there is a significant contribution from $^{27}$Si, direct synthesis of $^{27}$Al remains the dominant channel for production of Al.

In the models T1.4Z0.014, S1.0Z0.014 and M0.8Z0.014 show a reduction in the production of $^{27}$Al in all channels in the range of 4-5\,GK, as well as a smaller reduction in the higher temperature range of T1.4Z0.014. There is also a boost to direct production of $^{27}$Al at peak temperatures between 2 and 4GK. We see for all solar models that $^{27}$Al is primarily ejected directly, however there is a non-negligible contribution from some radioisotopes, not only at solar metallicities.  There is a reduction in the radiogenic contribution from $^{27}$Si at solar metallicity, similar to other intermediate mass elements discussed previously. This is due to reaction pathways shifting towards more neutron rich species as the flux of neutrons increases due to the $^{22}$Ne($\alpha$,n) reaction. This is also why we see the increase in $^{27}$Mg, as it is a product of neutron captures on the stable $^{26}$Mg. Most $^{27}$Al is ejected directly, although there are major contributions from radiogenic sources such as $^{27}$Si and $^{27}$Mg. There is still a significant proportion of $^{27}$Mg which contributes at the lowest peak temperatures.


\subsection{Silicon}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Si_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Si_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Si_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Si, and its stable isotopes $^{28}$Si, $^{29}$Si and $^{30}$Si.
 }
 \label{fig:Silicon_metalicity_multi}
\end{figure}

Silicon consists of 3 stable isotopes: $^{28}$Si, $^{29}$Si and $^{30}$Si and is mostly made in CCSN. $^{28}$Si is the most abundant naturally occurring stable isotope, and is a product of oxygen fusion through the reaction

$$ ^{16}\mathrm{O}({}^{16}\mathrm{O},\alpha){}^{28}\mathrm{Si} .  $$

Contributions from SNIa events are needed however to fit the observed solar system abundances \citep[see, for example][]{seitenzahl2013three,kobayashi2020origin}.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_SI_28.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_SI_28.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_SI_28.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_SI_28.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_SI_28.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_SI_28.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_SI_28.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_SI_28.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_SI_28.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{28}$Si are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:si_28_radiogenic}
\end{sidewaysfigure}

$^{28}$Si is by far the most abundant isotopic contributor to elemental Si production, as shown in figure \ref{fig:Silicon_metalicity_multi}. In all models, Si is produced in large quantities, with ejected masses above 0.2-0.3 M$_{\odot}$. The largest producers of Si are the M0.8 models, with a factor of around 2 larger ejected mass than compared with the other two classes of model across all metallicities (Figure \ref{fig:si_28_radiogenic}).

$^{28}$Si has no trend with metallicity until we reach super-solar models. After this there is a small dip in production of all classes of model, arising from reduced production of $^{28}$Si at the lowest peak temperatures due to neutron captures. We do see a strong metallicity dependence in $^{29}$Si and $^{30}$Si contributions to elemental silicon, resulting in a flat ejected elemental mass. $^{28}$Si has a broad peak of production in all models, stretching from 1.8 to 6 \,GK (slightly lower in the S1.0 and M0.8 models, due to the lower density of these tracer particles). Production of  $^{28}$Si in the lowest temperature range is dominated by radiogenic contributions, mostly from neutron rich Al although the impact on the integrated abundances is negligible, as can be seen in figure \ref{fig:Silicon_metalicity_multi}.

From figure \ref{fig:si_28_radiogenic} we see that models T1.4Z0, T1.4Z0.014 and T1.4Z0.1 have a higher temperature production peak for $^{28}$Si, which is relatively insensitive to the initial metallicity. This is due to the high density region in the SNIa causing electron capture reactions. For stellar conditions where nuclear reaction rates are approaching NSE, charged particle reaction rates are in equilibrium, and so it is the weak interactions which govern the shift in distribution from normal NSE to a more neutron rih distribution \citep{langanke2000shell}. The density of these hottest particles ensure that the Ye is similar between all T1.4 models in the high temperature region. Despite this, production is negligible compared to trajectories at lower peak temperatures.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_SI_29.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_SI_29.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_SI_29.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_SI_29.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_SI_29.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_SI_29.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_SI_29.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_SI_29.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_SI_29.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{29}$Si are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:si_29_radiogenic}
\end{sidewaysfigure}

$^{29}$Si has a similar trend with metallicity across the three class of models, as does $^{30}$Si. We see that the $^{29}$Si to $^{30}$Si ratio changes dramatically as we move from sub- to super-solar metallicities. $^{29}$Si is produced in a broad range of conditions in T1.4Z0, with production extending above 6\,GK. This small contributor to the ejected $^{29}$Si is lost at higher metallicities, although this is more than compensated for by the boost in secondary production at lower peak temperatures. This same trend is seen in the S1.0 and M0.8 models, with a reduction in the production at intermediate peak temperatures accompanied by a boost in production at lower temperatures. Radiogenic $^{29}$P is a significant contributor to $^{29}$Si in the T1.4Z0, S1.0Z0 and M0.8Z0  models although there is no significant radiogenic contribution at metallicities above 0 from $^{29}$P. At supersolar metallicities, we see a small contribution to the ejected $^{29}$Si mass of the order of a few percent.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_SI_30.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_SI_30.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_SI_30.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_SI_30.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_SI_30.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_SI_30.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_SI_30.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_SI_30.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_SI_30.eps} 
    \end{subfigure}
    
    

    \caption{The abundance distributions of $^{30}$Si are shown, arranged as in figure \ref{fig:o_16_radiogenic}. Note that the contribution from $^{}30$P in S1.0Z0 is very nearly 100\% of the eject4ed $^{30}$S, and is therefore difficult to observe under the decayed abundance line.}
 \label{fig:si_30_radiogenic}
\end{sidewaysfigure}

Production of $^{30}$Si is more complex, especially in the model T1.4Z0. There are broad radiogenic contributions from two isotopes - $^{30}$P is dominant at most peak temperatures, while there is equal production with $^{30}$S at temperatures above 5\,GK. At higher metallicities, the contribution from $^{30}$S becomes negligible, and $^{30}$Si is primarily ejected. $^{30}$P also becomes negligible at higher metallicities. We see this same trend in the S1.0 and M0.8 models, where at metallicity Z = 0 $^{30}$P dominated production of $^{30}$Si, while at higher metallicities $^{30}$Si is mostly ejected. 



\subsection{Phosphorus}

Phosphorus is mono-isotopic and is produced in carbon and neon burning in massive stars \citep{woosley2002evolution}. \citet{pignatari2016nugrid} identify explosive helium burning as a source. $^{31}$P is made in roughly equal proportions in our three types of progenitor (see figure \ref{fig:Phosphorus_metalicity_multi}). Production at lower metallicities in the intermediate mass S1.0 models is a factor of 2 lower than the T1.4 models, and 5 compared to the M0.8 models. Primary production of phosphorus decreases slightly from Z = 10$^{-5}$ to Z = 10$^{-3}$, after which production increases across all classes of model by more than an order of magnitude.


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/P_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/P_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/P_brox_yields_.eps} 
    \end{subfigure}

 \caption{
     As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of $^{31}$P.
 }
 \label{fig:Phosphorus_metalicity_multi}
\end{figure}


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_P__31.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_P__31.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_P__31.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_P__31.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_P__31.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_P__31.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_P__31.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_P__31.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_P__31.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{31}$P are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:p_31_radiogenic}
\end{sidewaysfigure}

At Z = 0, $^{31}$P is ejected mainly as $^{31}$S in the T1.4Z0 model, whilst it is directly made in the S1.0Z0 and M0.8Z0 models. As we move to the Z = 0.014 models, $^{31}$P is directly ejected, with the three models being nearly identical in the lower peak temperature range. Contributions to the ejected mass of $^{31}$P above T$_{9}$ = 4 GK are negligible, we may therefore ignore the high peak temperature tail of production in T1.4Z0.014. At Z = 0.1, we have a trace production of $^{31}$Al, which is shifted between the T1.4Z0.1 and S1.0Z0.1 and M0.8Z0.1 models from a peak around 2.2 \,GK, to a broader peak centered at 3\,GK in the lower mass models.



\subsection{Sulphur}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/S_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/S_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/S_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of S, and its stable isotopes $^{32}$S, $^{33}$S, $^{34}$S and $^{36}$S.
 }
 \label{fig:Sulphur_metalicity_multi}
\end{figure}

Sulphur consists of 4 stable isotopes: $^{32}$S, $^{33}$S, $^{34}$S and $^{36}$S. $^{32}$S is produced in explosive and hydrostatic oxygen burning as is $^{34}$S. $^{33}$S is produced in explosive oxygen or neon burning, all of these occur in CCSN \citep{woosley2002evolution}. $^{36}$S, the least abundant stable isotope, is produced in AGB stars in addition to the contribution from CCSN, in either hydrostatic helium burning or carbon neon burning \citep{pignatari2016nugrid,woosley2002evolution}. 

From figure \ref{fig:Sulphur_metalicity_multi} the trends of each isotope of sulphur are very similar between different sets of model, with similar trends with respect to metallicity. The models differ on the absolute ejected mass of the various S isotopes by about a factor of 2, except for $^{33}$S, which is more strongly produced in the M0.8 models, at some metallicities by nearly an oder of magnitude. 


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_S__32.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_S__32.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_S__32.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_S__32.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_S__32.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_S__32.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_S__32.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_S__32.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_S__32.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{32}$S are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:s_32_radiogenic}
\end{sidewaysfigure}

We see in figure \ref{fig:s_32_radiogenic} that $^{32}$S is ejected directly at zero metallicity for all models, with a similar profile for production below 5\,GK. There is a negligible contribution to the ejected mass of $^{32}$S from a high peak temperature tail in the T1.4Z0 model. At Z = 0.014, we begin to see the secondary production of other isotopes, namely $^{32}$P and $^{32}$Si although these are in trace amounts compared with the direct synthesis of $^{32}$S. The same is again true of the Z = 0.1 models.


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_S__33.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_S__33.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_S__33.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_S__33.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_S__33.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_S__33.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_S__33.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_S__33.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_S__33.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{33}$S are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:s_33_radiogenic}
\end{sidewaysfigure}


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_S__34.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_S__34.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_S__34.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_S__34.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_S__34.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_S__34.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_S__34.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_S__34.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_S__34.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{34}$S are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:s_34_radiogenic}
\end{sidewaysfigure}


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_S__36.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_S__36.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_S__36.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_S__36.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_S__36.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_S__36.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{36}$S are shown, arranged as in figure \ref{fig:o_16_radiogenic}. There is no production of $^{36}$S at Z = 0 and so those plots have been omitted.}
 \label{fig:s_36_radiogenic}
\end{sidewaysfigure}



\subsection{Chlorine}

Chlorine consists of two stable isotopes: $^{35}$Cl and $^{37}$Cl. $^{35}$Cl is produced during explosive oxygen and neon burning, with a small contribution from neutrino interactions \cite{pignatari2016nugrid,woosley2002evolution} during a CCSN. The majority of $^{37}$Cl is made in explosive oxygen or neon burning. SNIa are not expected to contribute significantly to the abundances of chlorine in the galaxy \citep{kobayashi2020origin,woosley2002evolution}.


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Cl_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Cl_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Cl_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Cl, and its stable isotopes $^{35}$Cl and $^{37}$Cl.
 }
 \label{fig:Chlorine_metalicity_multi}
\end{figure}



Figure \ref{fig:Chlorine_metalicity_multi} shows the metallicity dependency of the two chlorine isotopes. The trend with metallicity is similar between all three models, with the ejected mass of elemental chlorine being a factor of 2 higher in the M0.8 models than in the T1.4 and S1.0 models at all metallicities. significant radiogenic contributions are seen for both $^{35}$Cl and $^{37}$Cl at lower metallicities, however this contribution decreases for both isotopes above Z = 10$^{-4}$. Whilst there remains a large radiogenic contribution for $^{37}$Cl up to Z = 0.1, $^{35}$Cl is directly ejected at these higher metallicities.


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CL_35.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CL_35.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CL_35.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CL_35.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CL_35.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CL_35.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CL_35.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CL_35.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CL_35.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{35}$Cl are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:cl_35_radiogenic}
\end{sidewaysfigure}

Figure \ref{fig:cl_35_radiogenic} shows that a significant proportion of $^{35}$Cl in the T1.4Z0 model is ejected as radioactive $^{35}$Ar. This production occurs mainly in the region from 2GK to 5.8\,GK. As seen in model T1.4Z0.014, this contribution decreases with metallicity. Production of $^{35}$Ar is significantly reduced across the whole temperature range. On the other hand, the $^{35}$S radiogenic contribution increases with metallicity. Both of these trends continue in the T1.4Z0.1 model, with $^{35}$S becoming the dominant production pathway in the lower peak temperature trajectories. $^{35}$Cl production is still dominated by its direct production.

We see a similar trend in the S0.8 models, however there is no significant radiogenic contribution to the ejected mass of $^{35}$Cl, even in the S0.8Z0 model. The M0.8 models also follow the 
same trend as the low peak temperature component of the T1.4 models.

We see a double peak in production of $^{35}$Cl in the Z = 0.014 models at lower peak temperatures - one at 2.5\,GK and one at 3.8\,GK. These correspond to the carbon and oxygen burning regions and therefore to distinct reaction pathways producing these two regions of $^{35}$Cl. Production of $^{35}$Cl is suppressed in the lower of these two peaks in the Z = 0.1 model and the higher temperature production peak is boosted. As discussed above, this peak is directly ejected as $^{35}$Cl, where as the peak at lower temperatures is a mixture of $^{35}$Cl and radiogenic $^{35}$S.



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CL_37.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CL_37.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CL_37.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CL_37.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CL_37.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CL_37.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CL_37.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CL_37.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CL_37.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{37}$Cl are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:cl_37_radiogenic}
\end{sidewaysfigure}

In figure \ref{fig:cl_37_radiogenic} $^{37}$Cl is mostly ejected as radiogenic $^{37}$Ar. We see in the T1.4Z0, S1.0Z0 and M0.8Z0 models that there is almost no contribution from direct synthesis of $^{37}$Cl. There is a trace contribution to the ejected mass of $^{37}$Cl in the T1.4Z0 model from $^{37}$K, however this is negligible. In these models again see a double peak of production in the lower temperature range, slightly shifted to higher temperatures, at 3\,GK and 3.8\,GK respectively, compared to $^{35}$Cl. This temperature range corresponds to the onset of oxygen burning-like conditions in the SNIa in the higher temperature regime, and carbon burning like conditions for the lower band.

As we increase the initial metallicity to Z = 0.014, the higher temperature of these two peaks broadens, with production extending to 5\,GK and more. The lower temperature peak is suppressed, as was the case for $^{35}$Cl, and we see an increase in the direct synthesis of $^{37}$Cl although this remains a small contribution at this metallicity. This trend is similar across all of the Z = 0.014 models.

As the metallicity is again increased to Z = 0.1, the lower temperature peak becomes dominated by the direct synthesis of $^{37}$Cl. We see the higher temperature peak broadens again, extending peak production throughout the 4 to 5 \,GK range. We see from comparison with figure \ref{fig:Chlorine_metalicity_multi} that this gives rise to significant increase in the abundance of $^{37}$Cl, similar to the processes discussed for $^{35}$Cl.






\subsection{Argon}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ar_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ar_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ar_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Ar, and its stable isotopes $^{36}$Ar, $^{38}$Ar and $^{40}$Ar.
 }
 \label{fig:Argon_metalicity_multi}
\end{figure}


Argon consists of 3 stable isotopes: $^{36}$Ar, $^{38}$Ar and $^{40}$Ar. $^{36}$Ar and $^{38}$Ar are produced in CCSN during oxygen burning and explosive oxygen burning \citep{woosley2002evolution}. $^{40}$Ar is produced either during explosive helium burning, or carbon or neon burning. \citet{pignatari2016nugrid} note that the solar abundance of $^{40}$Ar is produced by the s-process, with theoretical yields from typical s-process sources matching observations well.

In all three sets of models argon production is seen to be mostly primary, with  a slight reduction in the total ejected mass at super-solar metallicities (\ref{fig:Argon_metalicity_multi}). This is due to the decrease in production of $^{36}$Ar with increasing metallicity which is partially compensated for at the highest metallicities, with the increase in production of $^{38}$Ar. In the case of the M0.8 models, $^{36}$Ar becomes almost as abundant as $^{36}$Ar. Indeed, the ratio of $^{36}$Ar to $^{38}$Ar at super-solar metallicities approaches unity as the mass of the progenitor decreases, whilst there is a factor of 5 difference in the T1.4Z0.1 model. Radiogenic $^{38}$Ar has a primary production up to Z = 10$^{-4}$, direct production becomes the dominant channel above Z = 10$^{-3}$.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_AR_36.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_AR_36.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_AR_36.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_AR_36.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_AR_36.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_AR_36.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_AR_36.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_AR_36.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_AR_36.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{36}$Ar are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ar_36_radiogenic}
\end{sidewaysfigure}


Again with $^{36}$Ar all three classes of model have similar production sites and metallicity trends. Inspection of figure \ref{fig:ar_36_radiogenic} shows that $^{36}$Ar is primarily produced at Z = 0 at temperatures between 4 and 5\,GK. this production is the same for all three classes of model. There is a trace amount of $^{36}$Cl produced at temperatures between 2.5 and 3\,GK, which sits in a secondary peak of production in $^{36}$Ar. At Z = 0.014, production is largely the same as in the Z = 0 case. We see an increased production of radioactive $^{36}$Cl, although this is still negligible compared to the bulk of production.





\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_AR_38.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_AR_38.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_AR_38.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_AR_38.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_AR_38.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_AR_38.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_AR_38.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_AR_38.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_AR_38.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{38}$Ar are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ar_38_radiogenic}
\end{sidewaysfigure}


Figure \ref{fig:ar_38_radiogenic} shows that $^{38}$Ar is mainly made as the radiogenic product of $^{38}$K at low metallicities in the T1.4 class of models. We also see a difference in the nucleosynthetic site of $^{38}$Ar, as there is a large contribution to production in the higher temperature range of 5.5 - 7GK, temperatures which are not reached in the M0.8 models, and only at the lower end (around 6\,GK) in the S1.0 models. $^{38}$Ar has an ejected mass approximately 5x greater in the low metallicity models of T1.4 as compared with S1.0 and M0.8 due to this higher temperature production range. We see two production peaks in the lower temperature region, consistent across the three classes of model.

$^{38}$Ar dominates the higher temperature region noted for the T1.4Z0 model, although this is now a negligible component to the overall ejected mass. The lower temperature region is a superposition of burning in the O and C burning layers, with the oxygen burning zone contributing the greatest proportion of $^{38}$Ar. Explosive oxygen burning produces $^{38}$Ar through the reaction $^{34}$S($\alpha$,$\gamma$)$^{38}$Ar, $^{34}$S being produced through the reaction $^{35}$Cl($\gamma$,p) as discussed in \citet{thielemann1985hydrostatic}.

In the Z = 0.014 models, production is dominated by the oxygen burning region. The double peak production has merged into one broad secondary peak of directly synthesised $^{38}$Ar. In the Z = 0.1 models, production at lower temperatures is dominated by the broad secondary peak of direct nucleosynthesis of $^{38}$Ar. This has increased further, and as such the higher temperature component of the T1.4Z0.1 model has an even smaller relative impact on the ejected mass.




\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
%        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_AR_40.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_AR_40.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_AR_40.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
%        \includegraphics[width=1\textwidth]{figures/Shen_z_0_AR_40.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_AR_40.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_AR_40.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
%        \includegraphics[width=1\textwidth]{figures/Miles_z_0_AR_40.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_AR_40.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_AR_40.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{40}$Ar are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ar_40_radiogenic}
\end{sidewaysfigure}

We see from figure \ref{fig:ar_40_radiogenic} that there is no high temperature component of $^{40}$Ar in SNIa. we also see that $^{40}$Ar production is highly dependent on initial metallicity. No models show production of $^{40}$Ar at Z = 0, and only trace amounts of $^{40}$Ar are synthesised between 2 and 3\,GK in the Z = 0.014 models. We see a sharp rise in the production of $^{40}$Ar at super-solar metallicities. 



\subsection{Potassium}

Potassium consists of 2 stable isotopes: $^{39}$K and $^{41}$K, and a long-lived radioisotope, $^{40}$K with a halflife of 1.28 Gyr. The bulk of solar potassium is $^{39}$K, which is produced in explosive and hydrostatic oxygen burning in CCSN \citep{pignatari2016nugrid,woosley2002evolution}. $^{41}$K is also produced in  explosive oxygen burning in CCSN, with a contribution from AGB stars. Yields of $^{40}$K are around 2 orders of magnitude smaller than total potassium yields. $^{40}$K have contributions from AGB, massive stars and the s-process prior to explosion through explosive helium burning \citep{pignatari2016nugrid}. $^{40}$K  is relevant to the formation and evolution of rocky planets due to the heat generated from its decay \citep{nimmo2020radiogenic}. The predicted theoretical abundance of $^{40}$K in the Milky Way is currently at odds with the observed abundance, with \citet{kobayashi2020origin} identifying it as being underproduced. It may be the case that SNIa contribute significantly to the observed abundances of $^{40}$K, as we see a production factor in excess of one for some of our models starting at solar metallicity in the T1.4 and S1.0 models, and at sub-solar metallicity in the M0.8 model set, within a factor of ten of the production factor of, e.g. $^{28}$Si. Events such as carbon oxygen shell mergers have previously been suggested as a way to boost the abundance of $^{40}$K in \citet{ritter2018nugrid}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/K_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/K_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/K_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of K, and its stable isotopes $^{39}$K, $^{40}$K and $^{41}$K.
 }
 \label{fig:Potasium_metalicity_multi}
\end{figure}

Figure \ref{fig:Potasium_metalicity_multi} shows the metallicity dependence of the stable potassium isotopes. $^{40}$K is only produced at higher metallicities, and only in trace amounts. We also see that $^{39}$K and $^{41}$K have similar trends. The relative ratio of these isotopes changes more dramatically for the S1.0 and M0.8 models than for the T1.4 model. $^{41}$K has a large radiogenic contribution, and a significant proportion of $^{39}$K in the T1.4 models for Z = 10$^{-4}$ is also from radiogenic sources.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_K__39.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_K__39.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_K__39.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_K__39.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_K__39.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_K__39.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_K__39.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_K__39.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_K__39.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{39}$K are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:k_39_radiogenic}
\end{sidewaysfigure}


Nucleosynthesis in the Z = 0 models differs significantly between the classes of models seen in figure \ref{fig:k_39_radiogenic}. While the overall production is similar within a factor of two between T1.4 and M0.8 (around 0.5) and S1.0 (around 1), T1.4Z0 has a relevant radiogenic contribution across the whole range of production from $^{39}$Ca. We also note that the range of temperatures over which $^{39}$K is produced is large, with similar mass fractions from 2\,GK up to 7\,GK (for those models with the appropriate particles to reach the respective peak temperatures). All three models show a production peak between 2 and 3 \,GK, the T1.4Z0 model containing a significant contribution from $^{39}$Ca. A narrow dip in production at around 3.5\,GK then leads to a broad plateau, where production continues up to 7\,GK.

The path of nucleosynthesis in these SNIa is more consistent between models at Z = 0.014 with production almost exclusively through direct synthesis of $^{39}$K. Trace amounts of $^{39}$Ar are produced in the 2-4\,GK range in all classes of model, and there is a trace contribution from $^{39}$Ca in the intermediate to high peak temperature range in model T1.4Z0.014.

As the initial metallicity increases to Z = 0.1, this trace production of $^{39}$Ca is suppressed further in the T1.4Z0.1 model, there is an increase in the production of radio-isotope $^{39}$Ar, and a trace amount of $^{39}$Cl produced in the 2-3\,GK range due to neutron captures in the carbon burning region. Production in the low peak temperature region is consistent between all models.


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
%        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_K__40.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_K__40.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_K__40.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
%        \includegraphics[width=1\textwidth]{figures/Shen_z_0_K__40.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_K__40.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_K__40.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
%        \includegraphics[width=1\textwidth]{figures/Miles_z_0_K__40.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_K__40.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_K__40.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{40}$K are shown, arranged as in figure \ref{fig:o_16_radiogenic}. There are no data for the Z = 0 models, theses panels have therefore been omitted.}
 \label{fig:k_40_radiogenic}
\end{sidewaysfigure}

$^{40}$K shows no production at Z = 0 for any of the three class of models, we therefore show no plots for the Z = 0 column in figure \ref{fig:k_40_radiogenic}. Above Z = 0 $^{40}$K production is very similar for all of the models shown in figure \ref{fig:k_40_radiogenic}. At Z = 0.014, we have a double peak of production - the largest between 2.5 and 3 GK, the second between 3.5 and 4\,GK. We note that the position of the second peak here is slightly shifted between models, with the T1.4Z0.014 peak being at a higher temperature with a broader profile. This peak in the T1.4 model remains sightly broader in the Z = 0.1 models, where it is also boosted by secondary contributions to the nucleosynthesis of $^{40}$K. 

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_K__41.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_K__41.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_K__41.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_K__41.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_K__41.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_K__41.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_K__41.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_K__41.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_K__41.eps} 
    \end{subfigure}
    
    

    \caption{The abundance distributions of $^{41}$K are shown, arranged as in figure \ref{fig:o_16_radiogenic}. Radiogenic contributions from $^{41}$Ca account for nearly 100\% of production at low metallicities, and is therefore obscured by the decayed abundance line.}
 \label{fig:k_41_radiogenic}
\end{sidewaysfigure}

We see the same general trend for $^{41}$K in (figure \ref{fig:k_41_radiogenic}) as was observed in  $^{39}$K. Lower peak temperature production is consistent between all classes of model, here the primary production of nucleosynthesis is $^{41}$Ca, in the Z = 0 models almost 100\% of the $^{41}$K ejected is produced as radiogenic $^{41}$Ca, which is therefore obscured in these plots by the decayed abundance line. We see a double peaked feature in the cooler outer layers of the SNIa explosion, with the T1.4Z0 model having a slight broadening and shifting to higher temperatures as compared with the S1.0Z0 and M0.8Z0 models. A broad high temperature production region is also present in the T1.4Z0 model, which provides a non-negligible contribution to the integrated abundance of $^{41}$K on the order of a few percent.

In the Z = 0.014 models, the second of the low temperature peaks begins to dominate production, with a secondary boost to the production of $^{41}$Ca, under explosive oxygen burning conditions. It is similar between each of the three models, the T1.4Z0.014 peak is at a slightly higher temperature and is broader. The high temperature production in the T1.4Z0.014 model is small in comparison to the production in the explosive oxygen burning layers of the ejecta. We see a trace amount of $^{41}$K produced directly in the outer layers of the WD at peak temperatures between 2 and 4 GK. 

In the Z = 0.1 models, this trace production begins to dominate in the carbon burning conditions. A trace amount of $^{41}$Ar is produced in the very lowest peak temperature conditions, corresponding to the tail of carbon burning.









\subsection{Calcium}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ca_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ca_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ca_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Ca, and its stable isotopes  $^{40}$Ca, $^{42}$Ca, $^{43}$Ca and $^{44}$Ca.
 }
 \label{fig:Calcium_metalicity_multi}
\end{figure}


Calcium consists of 6 stable isotopes: $^{40}$Ca, $^{42}$Ca, $^{43}$Ca and $^{44}$Ca, $^{46}$Ca and $^{48}$Ca. $^{40}$Ca is produced in oxygen burning, and both $^{40}$Ca and $^{42}$Ca are produced in explosive oxygen burning during CCSN events. $^{43}$Ca is produced in carbon and neon burning, and in $\alpha$-rich freezout from NSE \citep{woosley2002evolution}. $^{44}$Ca is predicted to be produced efficiently from SNIa helium detonation or from $\alpha$-rich freezout, where it is formed as $^{44}$Ti \citep{pignatari2016nugrid,magkotsios2010trends}. $^{46}$Ca has a contribution from AGB stars, and is also produced in carbon and neon burning. Finally, $^{48}$Ca is formed in the n-process \citep{pignatari2016nugrid}, or in conditions in a CCSN with high neutron fluxes. \cite{woosley2002evolution} also identify $^{48}$Ca as having a significant contribution from Chandrasekhar mass SNIa events. 

Figure \ref{fig:Calcium_metalicity_multi} shows how similar production is between our three classes of model, with $^{40}$Ca, $^{42}$Ca and $^{44}$Ca having very similar trends with respect to metallicity. $^{43}$Ca also has a similar trend. In the Z = 10$^{-4}$ to 10$^{-2}$ range, production drops significantly for this isotopes in the M0.8 models, as compared with the T1.4 and S1.0 models, it is also produced directly, where as the production in the other models is almost exclusively as radio-isotopes. Only a trace amount of $^{46}$Ca is produced in any model, and only in the M0.8Z0.1 metallicity model. $^{48}$Ca is not produced in any of our post-processed models.



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CA_40.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CA_40.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CA_40.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CA_40.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CA_40.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CA_40.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CA_40.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CA_40.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CA_40.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{40}$Ca are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ca_40_radiogenic}
\end{sidewaysfigure}

In figure \ref{fig:ca_40_radiogenic} we see that production of $^{40}$Ca is fairly simple and consistent throughout the models. A broad production peak is observed in the Z = 0 models in the peak temperature range between 4 and 5.5 GK. As the initial metallicity is increased we see that the mass fraction of $^{40}$Ca in this peak production region also decreases, resulting in the metallicity trend of $^{40}$Ca observed in figure \ref{fig:Calcium_metalicity_multi}. The ejected mass of $^{40}$Ca decreases from 2.27x10$^{-2}$ to 1.29x10$^{-2}$ M$_{\odot}$ for the T1.4 models, 2.43x10$^{-2}$ to 1.21x10$^{-2}$ M$_{\odot}$ in the S1.0 models and 2.71x10$^{-2}$ to 7.55x10$^{-3}$ M$_{\odot}$ in the M0.8 models. The larger effect in the M0.8 model is due to the absence of any production in NSE regions in this class of model.





\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CA_42.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CA_42.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CA_42.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CA_42.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CA_42.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CA_42.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CA_42.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CA_42.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CA_42.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{42}$Ca are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ca_42_radiogenic}
\end{sidewaysfigure}


Production of $^{42}$Ca in T1.4Z0 is dominated by a high temperature peak in the 6-7\,GK range, with smaller peaks between 4 and 4.3\,GK and 8 and 9\,GK. The lowest temperature peak is reproduced in the S1.0Z0 and M0.8Z0 models in the same temperature range. Direct synthesis of $^{42}$Ca is the main path for all three classes of model.

Production of $^{42}$Ca is significantly boosted in the T1.4Z0.014, S1.0Z0.014 and M0.8Z0.1 models, the low temperature peak observed in the Z = 0 models is here increased by several orders of magnitude and covers a peak temperature range from 2 to 4\,GK. This temperature range covers both carbon burning and oxygen burning regions, with the largest contribution being in the 3.5 - 5 GK range, corresponding to oxygen burning. The lower temperature shoulder of production below approximately 3 GK contributes on the order of a few percent to the ejected mass of $^{42}$Ca, in both regions through direct synthesis of $^{42}$Ca. In T1.4Z0.014, these is also a significant boost to the production in the intermediate temperature range peak but due to the rapid growth of production in the outer layers of the SNIa explosion, this contribution is negligible.

We see a further dramatic increase in production in the Z = 0.1 case. T1.4Z0.1 has a small reduction in production in the 6-7\,GK peak. This is compensated for by the increase in the oxygen burning region where $^{42}$Ca is around 0.2\% of the mass fraction of these tracer particles. This is accompanied by a decrease in production in the carbon burning like region below 3 GK. This same trend is seen in models S1.0Z0.1 and M0.8Z0.1, with trace production of $^{42}$K and $^{42}$Ar appearing in the very lowest peak temperature range. The peak at around Z$_{\odot}$ for $^{42}$Ca in the carbon burning region to the decline at higher metallicity is due to the effect of excess neutron captures driving production to more neutron rich isotopes.




\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CA_43.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CA_43.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CA_43.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CA_43.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CA_43.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CA_43.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CA_43.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CA_43.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CA_43.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{43}$Ca are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ca_43_radiogenic}
\end{sidewaysfigure}


Figure \ref{fig:ca_43_radiogenic} shows the production of $^{43}$Ca. Production in the T1.4Z0 is dominated by the 5.5 - 7 GK temperature range, where $^{43}$Ca is produced as $^{43}$Sc with a contribution on the order of 1\% from $^{43}$Ti. The majority of nucleosynthesis in this temperature range is primary as $^{43}$Sc production does not change across metallicities; however, the radiogenic contribution does show some secondary effects. As the metallicity increases (T1.4Z0.014), we see that production below 5 GK shifts to lower peak temperatures. We now see a double peaked structure, which corresponds to the positions of the oxygen and carbon burning regions described in \citet{iliadis2015nuclear} between 2 and 4 GK. In these two regions, $^{43}$Ca is produced directly with a small contribution from $^{43}$Sc. As the initial neon mass fraction is increased further, the carbon and oxygen burning regions become less distinct, and a broad production peak is seen spanning the whole peak temperature range. A small radiogenic contribution from $^{43}$Sc is observed in the 3.5 - 5 GK range, where as $^{43}$Ca is mainly produced as radiogeninc $^{43}$K in the lower temperature carbon burning region. This shows that there is a fundamental difference in the nucleosynthesis of $^{43}$Ca in these two regions and that $^{43}$Ca production may be sensitive to a range of nuclear reaction rates at these lower temperatures.

In the S1.0Z0 model, the maximum peak temperature is approximately 6.2 GK. From around 5.5 to 6.2 GK we see again the production of the radioisotope $^{43}$Sc. The double peaked production region between 2 and 4 GK, which corresponds to the carbon and oxygen-like burning regions is present in the S1.0Z0.014 model. We see that it is similar between to the T1.4Z0.014 case, with direct production of $^{43}$Ca with a small contribution from $^{43}$Sc however the carbon region production is boosted in the S1.0Z0.014 model compared with T1.4Z0.014. S1.0Z0.1 shows the same trend as the T.14 models, where the double peak of production between 2 and 4 GK broadens, with the carbon region producing radiogenic $^{43}$K and the oxygen region producing $^{43}$Ca directly.

The M0.8 models show the same trends in the 2 to 5 GK range as are observed in the T1.4 and S1.0 models, with the higher temperature region being absent. In the M0.8Z0.014 models, the carbon peak production of $^{43}$Ca is closer to the value found in the T1.4Z0.014 model than the S1.0Z0.014 model.

%Production in T1.4Z0.014 is substantially different to the Z = 0 case. $^{43}$Sc still represents the bulk of $^{43}$Ca production but there is now a smaller double peaked contribution from direct synthesis of $^{43}$Ca in the 2.3-2.8 and 3.5-4.2\,GK ranges. $^{43}$Ti continues to contribute at the high temperature end, although it is still a small fraction of the total $^{43}$Ca produced. S1.0Z0.014 has a large contribution to $^{43}$Ca from a small section of the higher temperature peak production, secondary production of $^{43}$Ca is also significant, as described for the T1.4Z0.014 model. We see a somewhat higher peak for the lowest temperature production site in S1.0Z0.014 as compared with the other Z = 0.014 models.



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CA_44.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CA_44.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CA_44.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CA_44.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CA_44.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CA_44.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CA_44.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CA_44.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CA_44.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{44}$Ca are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ca_44_radiogenic}
\end{sidewaysfigure}


$^{44}$Ca is produced primarily as $^{44}$Ti in all of the Z = 0 models. In T1.4Z0, it is produced over a wide range of peak temperatures from 4 to 6.5\,GK, with a negligible contribution from a peak at 2.8\,GK. We see a similar distribution in the S1.0Z0 and M0.8Z0 models, with appropriate upper temperature limits as discussed for in previous sections.

T1.4Z0.014 shows a small drop in the production of $^{44}$Ti at the lower end of this broad range of production, this is partially compensated for by the increased secondary production in the small peak centered at 2.8\,GK. Across the rest of the peak temperature range, we see contributions only from $^{44}$Ca and $^{44}$Ti, in this secondary peak we see production of $^{44}$Sc also, although it is not the most abundant isotope in this temperature window. S1.0Z0.014 shows the same trend, as does M0.8Z0.014.

In the Z = 0.1 models, we see a further suppression of the $^{44}$Ti production at the tail end of the broad production range, the increase in direct synthesis of $^{44}$Ca compensates for this somewhat and leads to a continuation of the production range out to approximately 2.4\,GK



\subsection{Scandium}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Sc_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Sc_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Sc_brox_yields_.eps} 
    \end{subfigure}

 \caption{
     As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of $^{45}$Sc.
 }
 \label{fig:Scandium_metalicity_multi}
\end{figure}


Scandium is mono-isotopic, with $^{45}$Sc being produced in $\alpha$-rich freeze-out, the neutrino process and carbon and neon burning in massive stars \citep{woosley2002evolution}. Current theoretical predictions of the GCE of scandium report it being underproduced relative to observations \citep{kobayashi2020origin,kobayashi2006galactic}, although recent work including the contributions of jet-induced supernovae mitigate this somewhat. Carbon oxygen shell shell mergers also increase the amount of scandium produced in CCSN \citep{ritter2018nugrid} which accounts for some of this discrepancy.

Scandium shows a similar trend across all three classes of model with respect to metallicity. It is mainly produced as a radiogenic $^{45}$Ti, with only M0.8Z0.1 having a direct $^{45}$Sc yield of greater than 10\% synthesised during the explosion.




\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_SC_45.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_SC_45.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_SC_45.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_SC_45.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_SC_45.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_SC_45.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_SC_45.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_SC_45.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_SC_45.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{45}$Sc are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:sc_45_radiogenic}
\end{sidewaysfigure}


$^{45}$Sc is produced over a range of peak temperatures in the T1.4Z0 model, mostly as $^{45}$Ti. There is a peak in production at 4 GK and a broad region between 5 and 8 GK. Production is similar in S1.0Z0 however as the maximum peak temperature in this model is at around 6.2 GK, the broad production region above 5 GK contributes proportionally less to the ejected mass of $^{45}$Sc. The 4 GK peak is shifted slightly to between 3.5 and 4 GK, and is narrower. The small peak at 3 GK, which was negligible in the T1.4Z0.0 model is larger here. Production in M0.8Z0 is similar to the low temperature peak component of S1.0Z0.

In model T1.4Z0.014, production of $^{45}$Sc is boosted significantly across a wide range of temperatures as compared with the Z = 0 case. In figure \ref{fig:sc_45_radiogenic}, we see a secondary component in production of both $^{45}$Sc and $^{45}$Ti which boosts production in the lower temperature burning region significantly. This effect is also seen in S1.0Z0.014 and M0.8Z0.014. At peak temperatures above 3.5 GK, $^{45}$Sc is mostly produced as the radioisotope $^{45}$Ti. At lower temperatures it is directly produced. A The metallicity increases further, a small contribution from $^{45}$K in the 2.5 - 3 GK range is seen. This is also true for the S1.0 and M0.8 models.

As th initial metallicity is increased further, production at the very lowest temperatures is suppressed, with the double peaked production sites evident in the Z = 0 and 0.014 cases becoming a single peak.













\subsection{Titanium}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ti_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ti_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ti_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Ti, and its stable isotopes $^{46}$Ti, $^{47}$Ti, $^{48}$Ti, $^{49}$Ti and $^{50}$Ti.
 }
 \label{fig:Titanium_metalicity_multi}
\end{figure}


Titanium has 5 stable isotopes: $^{46}$Ti, $^{47}$Ti, $^{48}$Ti, $^{49}$Ti and $^{50}$Ti. $^{46}$Ti is produced in explosive oxygen burning and SNIa detonations, $^{47}$Ti is produced in the same as well as in explosive silicon burning. $^{48}$Ti is produced in explosive silicon burning or SNIa detonations, and $^{49}$Ti in explosive silicon burning only. Finally, $^{50}$Ti is produced in Chandrasekhar mass SNIa explosions and the s-process in massive stars \citep{woosley2002evolution}.

Figure \ref{fig:Titanium_metalicity_multi} presents the metallicity dependence of the production of these isotopes. We see that $^{48}$Ti is the most abundant isotope of titanium in all three models for almost all metallicities. Only in the M0.8Z0.1 model does $^{46}$Ti become more abundant than $^{48}$Ti. $^{46}$Ti production is primary at Z < 0.00001 and secondary above this, with the ejected mass of $^{46}$Ti increasing with metallicity. $^{47}$Ti has a strong secondary component in the three classes of model above Z = 0.001, this secondary component is through direct production of $^{47}$Ti. $^{48}$Ti is flat with metallicity in the T1.4 models until Z > 0.05 where a strong secondary contribution is seen, for the S1.0 and M0.8 models, this contribution starts at Z = 0.001. $^{50}$Ti is abundant the T1.4 models only, with only trace amounts produced in the S1.0 and M0.8 models at Z > 0.01. $^{50}$Ti also has a very flat dependency on the metallicity of the progenitor. These properties suggest that the $^{50}$Ti/$^{48}$Ti isotopic ratio may provide a diagnostic for the determination of SNIa progenitor.

The ejected mass of elemental titanium decreases with increasing progenitor metallicity, despite the strong secondary production observed in all isotopes except for $^{48}$Ti.



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_TI_46.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_TI_46.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_TI_46.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_TI_46.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_TI_46.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_TI_46.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_TI_46.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_TI_46.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_TI_46.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{46}$Ti are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ti_46_radiogenic}
\end{sidewaysfigure}


Figure \ref{fig:ti_46_radiogenic} shows that $^{46}$Ti production at Z = 0 is much more active in T1.4Z0 than in either of the other two models. This is due to $^{46}$Ti being synthesised in intermediate to high temperatures, at 6\,GK or above, which do not exist in the S1.0 and M0.8 models. There is a small peak of production at approximately 4\,GK which is negligible.

We see in the Z = 0.014 panels that production of $^{46}$Ti (through direct nucleosynthesis) is highly dependent on the initially metallicity. The small peak at 4\,GK now dominates the production. The high temperature component of the T1.4 models remains unchanged.


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_TI_47.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_TI_47.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_TI_47.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_TI_47.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_TI_47.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_TI_47.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_TI_47.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_TI_47.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_TI_47.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{47}$Ti are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ti_47_radiogenic}
\end{sidewaysfigure}

Figure \ref{fig:ti_47_radiogenic} shows the production of $^{47}$Ti with respect to the peak temperatures experienced in a given tracer particle. $^{47}$Ti is produced over a broad range of peak temperatures in the T1.4 models. At Z = 0, the production of $^{47}$Ti occurs in the temperature range from 4 to 9 GK, this spans the range from explosive oxygen burning through to NSE. There is a peak between 5.5 and 7 GK, which contributes the majority of material. Across the whole temperature range, the radioisotope $^{47}$V contributes the largest proportion of $^{47}$Ti. In the peak temperature range from 8 to 9 GK, there is some contribution from $^{47}$Ti however this is a small fraction of the integrated $^{47}$V contribution. Above 9 GK, there is a region of $^{47}$Sc production but again this is small. Moving to the T1.4Z0.014 model, production extends to lower peak temperatures, with a peak between 2.3 and 4.2 GK being formed. This temperature range corresponds to the carbon burning regions. $^{47}$Ti is produced directly in this region. In T1.4Z0.1 model, we see that production of $^{47}$Ti in the lower peak temperature regions has increased further. $^{47}$Ti now accounts for more than 1\% of the ejected Ti mass, however this is also, in part, due to a decrease in the ejected mass driven by the metallicity dependence of $^{46}$Ti.

In model S1.0Z0, production is between 3.8 and 6.1 GK, with the radioisotope $^{47}$V dominating production. In model S1.0Z0.014, the carbon and oxygen burning regions begin to contribute a significant proportion of the ejected mass of $^{47}$Ti. It is produced directly in this region. At Z = 0.1, almost the whole amount of $^{47}$Ti is produced as radiogenic $^{47}$V, mostly in the carbon and oxygen burning regions.

As with the S1.0 models the production in the M0.8 models is strongly metallicity dependent. As there is no contribution in the M0.8 models from the >6 GK production region, the yields of $^{47}$Ti for M0.8 are very sensitive to the nucleosynthesis in the carbon and oxygen burning regions. The trend is otherwise the same as for the S1.0 model, with production being through the same mechanism.


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_TI_48.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_TI_48.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_TI_48.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_TI_48.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_TI_48.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_TI_48.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_TI_48.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_TI_48.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_TI_48.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{48}$Ti are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ti_48_radiogenic}
\end{sidewaysfigure}


The production of $^{48}$Ti is shown in figure \ref{fig:ti_48_radiogenic}. The trend for the T1.4 models is similar to that observed for $^{47}$Ti. Production is again over a broad rage of temperatures, ranging from oxygen burning at 4 GK, to the high density NSE region at > 9 GK. Above 8.2 GK, the main production pathway of $^{48}$Ti is direct production. Below 8.2 GK and across the whole of the rest of the production sites, $^{48}$Ti is produced as $^{48}$Cr, with a negligible contribution from $^{48}$V. This is similar to the $^{47}$Ti where it is produced mainly as radiogenic $^{47}$V. In T1.4Z0.014, production extends into the carbon burning region between 2.3 and 3.8 GK. Here $^{48}$Ti is produced directly and is strongly metallicity dependent. Production at higher temperatures remains fairly unchanged,although there must be a small decrease in production as the ejected mass of $^{48}$Ti decreases slightly compared with the T1.4Z0 model - from 1.46x10$^{-6}$ M$_{\odot}$ to 1.42x10$^{-6}$ M$_{\odot}$. The increasing production in the cooler outer regions in the Z = 0.1 model more than compensate for the slight reduction in the oxygen burning and NSE regions, where we see an overall increase in the ejected mass of $^{48}$Ti to 1.65x10$^{-6}$ M$_{\odot}$. we see an increase in the contributions from $^{48}$V in the 4 - 6 GK range however its contribution remains small. $^{48}$Ti is directly produced above 8.8 GK and below 4.5 GK, and radiogenic $^{48}$Cr provides the bulk of material in the 4 - 8 GK region.

In the S1.0Z0 model, production of radiogenic $^{48}$Cr dominates the $^{48}$Ti production. Only a trace contribution from $^{48}$V is seen. The 3.5 - 6.1 GK production region is otherwise solely $^{48}$Cr. Similar to the metallicity dependence in the T1.4 models, we see direct production of $^{48}$Ti in the 2.8 - 3.8 GK range as we move to the S1.0Z0.014 model. $^{48}$V production also increases somewhat however the dominant channel is still through $^{48}$Ti. In the S1.0Z0.1 models the carbon burning production has increased further. As we see in figure \ref{fig:Titanium_metalicity_multi} however, in neither T1.4, S1.0 or M0.8 is the increase in direct production enough to compensate for the decrease in the oxygen burning and NSE contributions with increasing metallicity. 

The M0.8 models show a similar behaviour to the S1.0 set, with a proportionally larger contribution from the carbon burning ejecta. 





\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_TI_49.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_TI_49.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_TI_49.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_TI_49.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_TI_49.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_TI_49.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_TI_49.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_TI_49.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_TI_49.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{49}$Ti are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ti_49_radiogenic}
\end{sidewaysfigure}

Figure \ref{fig:ti_49_radiogenic} shows the ejected abundances for $^{49}$Ti in the three sets of models. In T1.4Z0, production ranges from 3.8 GK to > 9GK, with three peaks of production between 3.8 and 6 GK, 7 and 8 GK and above 9 GK respectively. The majority of $^{49}$Ti is produced as $^{49}$Cr, particularly below 8 GK where almost 100\% of the ejecta is radiogenic $^{49}$Cr. Only trace amounts of radiogenic $^{49}$Mn and $^{49}$V are present. between 8 and 9 GK, there is a small region where production is dominated by contributions from radiogenic $^{49}$V, and above 9 GK direct production of $^{49}$Ti is seen. These two regions are small compared to the $^{49}$Cr producing region however. In the T1.4Z0.014 model, we see a significant increase in the 4 - 6 GK region, corresponding to oxygen and silicon burning. Peak production in these particles increases by an order of magnitude between these two models. We also see an increase in the contribution from $^{49}$V, where a low temperature production region in the carbon burning particles is seen between 2.3 and 3.5 GK. In the T1.4Z0.1 model, this low temperature region is depleted, due to increased neutron captures shifting material to more neutron rich isotopes. We see a further increase in the 4.5 - 6 GK region, which drives the increasing ejected mass of $^{49}$Ti with initial metallicity.

the models of S1.0 and M0.8 show a similar trend to the two lower temperature peaks in T1.4. There is an initial, small increase in production in the carbon burning region, along with a larger increase in the 3.5 - 5.8 GK region in these two models. $^{49}$Ti is produced as $^{49}$Cr in the intermediate temperature region, and $^{49}$V in the lower temperature regions. When the initial metallicity is increased further to Z = 0.1, then the carbon burning region is suppressed. This has a larger effect on the trend in the S1.0 and M0.8 models. 





\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_TI_50.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_TI_50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_TI_50.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_TI_50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_TI_50.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps} 
   \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_TI_50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_TI_50.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{50}$Ti are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ti_50_radiogenic}
\end{sidewaysfigure}

Figure \ref{fig:ti_50_radiogenic} shows the production of $^{50}$Ti in our three classes of model. In T1.4Z0, we see that the only contribution to $^{50}$Ti is from the particles with peak temperature T > 8 GK. As such, neither the S1.0 or M0.8 model can produce $^{50}$Ti at Z = 0. As the metallicity is increased, we see a small production of $^{50}$Ti in the oxygen burning region, between 3 and 3.5 GK. This is reproduced in S1.0Z0.014 and M0.8Z0.014, where production is slightly larger than in the T1.4 model. In all cases however, the lower temperature component is small, and has a negligible impact on the abundances of $^{50}$Ti in T1.4. As the metallicity is increased to Z = 0.1, we see a very slight increase in the ejected mass of $^{50}$Ti, from 1.12x10$^{-5}$ M$_{\odot}$ in the Z = 0 case to 1.34x10$^{-5}$ M$_{\odot}$ in the Z = 0.1 case. There is a larger proportional increase in the S1.0 and M0.8 models however the maximum ejected mass of $^{50}$Ti in either of these models is of the order a few x10$^{-8}$ and so it is only ejected as a trace isotope.




















\subsection{Vanadium}

Vanadium has two isotopes which are considered stable (one with a half-life of 10$^{17}$Yrs): $^{50}$V and $^{51}$V. $^{50}$V is made in a variety of conditions in massive stars - carbon and neon burning, and explosive oxygen and neon burning. $^{51}$V is made also in massive stars in explosive oxygen and silicon burning, as well as the neutrino process, $\alpha$-rich freeze-out and SNIa detonation models \citep{woosley2002evolution}. 

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/V_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/V_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/V_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of V, and its stable isotopes $^{50}$V and $^{51}$V.
 }
 \label{fig:Vanadium_metalicity_multi}
\end{figure}

We see in figure \ref{fig:Vanadium_metalicity_multi} that vanadium has a similar trend with metallicity through our three classes of model. There is a factor of ~10 between production between the T1.4 and M0.8, and a dip in production in M0.8 at Z = 10$^{-4}$ which is not observed in the other models, however the broad trend of a strong secondary component is the same across the models. We do see that trace amounts of $^{50}$V are produced at all metallicities in the T1.4 models, with a weak secondary component, where as in the S1.0 and M0.8 models, this secondary component has a much stronger dependency on metallicity.



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_V__50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_V__50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_V__50.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_V__50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_V__50.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_V__50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_V__50.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{50}$V are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:v_50_radiogenic}
\end{sidewaysfigure}

In figure \ref{fig:v_50_radiogenic} we show the production of $^{50}$V. There is no production of $^{50}$V in the lower mass models at zero metallicity, and that a secondary component arises in the 2.5-4\,GK range at solar metallicity. This oxygen burning region shifts to hotter peak temperature particles as metallicity continues to increase. In the T1.4 models, we see that the primary component from the hottest particles (T > 8 GK). This is due to the Ye of these particles being governed by electron captures in the hight density, high temperature regime. This sets a Ye that is independent from the initial electron fraction. A similar secondary production trend as seen in S1.0Z0.014 and S1.0Z0.1 can be seen between T1.4Z0.014 and T1.4Z0.1 in the ejecta of the external layers.






\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_V__51.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_V__51.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_V__51.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_V__51.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_V__51.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_V__51.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_V__51.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_V__51.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_V__51.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{51}$V are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:v_51_radiogenic}
\end{sidewaysfigure}

Production of $^{51}$V is significantly more complex than $^{50}$V, particularly in the T1.4 models. In model T1.4Z0, the highest peak temperature particles (above 9\,GK) have direct synthesis of $^{51}$V. As we move to lower peak temperatures, $^{51}$Cr becomes the largest contributor. This extends only over a narrow temperature range from approximately 7.8 to 8.5\,GK, below which synthesis of $^{51}$V is mostly as $^{51}$Mn. We see a trace contribution from $^{51}$Fe in this model, but it is small in comparison to the other contributing isotopes. As the metallicity increases in model T1.4Z0.014, the high temperature contribution to the isotopic abundance of $^{51}$V remains the same. We see the low temperature contribution from $^{51}$Cr increase, boosting production of $^{51}$V slightly. From comparison with figure \ref{fig:Vanadium_metalicity_multi}, we can see that this increase in radiogenic contribution has a significant impact on the ejected mass of $^{51}$V, and consequently on the ejected mass of elemental vanadium. Secondary production is boosted still further in model T1.4Z0.1, where the low temperature secondary tail begins to dominate the ejecta.

The synthesis of $^{51}$Mn is the main route for production in model S1.0Z0, with a trace contribution from radioactive $^{51}$Cr. This production occurs over a broad range of temperatures, but is much less abundant than in the T1.4 cases. 

In models S1.0Z0.014, the production of $^{51}$Cr at lower temperatures begins to contribute significantly to the overall ejected mass of $^{51}$V. This trend increases as we move to model S1.Z0.1, where the contributions from $^{51}$Mn and $^{51}$Cr become comparable. The contribution from $^{51}$Mn occurs above peak temperatures greater than 4.5\,GK and $^{51}$Cr below this.

Production in the M0.8 models follows a similar trend to the S1.0 models. M0.8Z0.1 shows a much larger $^{51}$Cr to $^{51}$Mn production due to the smaller number of particles at higher peak temperatures, and the lower maximum peak temperature in this model.









\subsection{Chromium}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Cr_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Cr_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Cr_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Cr, and its stable isotopes $^{50}$Cr, $^{52}$Cr, $^{53}$Cr and $^{54}$Cr.
 }
 \label{fig:Chromium_metalicity_multi}
\end{figure}


Chromium has 4 stable isotopes: $^{50}$Cr, which has a half-life of 1.3$\times$ 10$^{18}$ years and which we therefore can treat as stable, $^{52}$Cr, $^{53}$Cr and $^{54}$Cr. $^{52}$Cr is the most abundant Cr isotope in the Sun (83.789$\%$ of the solar Cr), while $^{54}$Cr has the lowest abundance (2.365$\%$ of the solar Cr) \citep{asplund2009chemical,lodders2003solar}.

%[A SENTENCE OR TWO ABOUT PRODUCTION OF CR WITH RESPECT TO SOME PREVIOUS FIGURE WITH ABUNDANCE DISTRIBUTION. FOR INSTANCE, HOW MUCH CR IS MADE WITH RESPECT TO IRON, OR THE MOST ABUNDANT ELEMENT. CAN YOU UPLOAD PLOTS WITH ABUNDANCE DISTRIBUTION, YIELDS AND PRODUCTION FACTORS?]

In Figure~\ref{fig:Chromium_metalicity_multi}, we show the integrated Cr yields for the element and its isotopes, for the T1.4, S1.0 and M0.8 sets. Cr production is dominated by $^{52}$Cr for all metallicities in the T1.4 and S1.0 sets. At metallicities higher than solar, in the M0.8Z0.1 models $^{50}$Cr and $^{53}$Cr production increases enough as the metallicity of the progenitor increases to affect the Cr abundance budget, causing an increase of the total ejected mass. With the exception of this pattern, Cr production appears to be primary in all models, following the $^{52}$Cr behavior. Hear, primary denotes that material which is synthesised directly in the explosion during freeze-out, where as secondary is material which is synthesised from the seeds of other nuclei (ultimately in this work originating with the initial abundance of $^{22}$Ne)

On the other hand, the relative production of different Cr isotopes changes significantly with metallicity and using different model sets.
$^{50}$Cr is the only isotope that is always produced directly. $^{54}$Cr is mostly ejected as itself in T1.4 models, while for other the sets it is mostly radiogenic.  $^{52}$Cr and $^{53}$Cr are produced by radiogenic contribution in the Chandrasekhar mass explosion models, primarily from $^{52}$Fe and $^{53}$Fe respectively. There is a significant contribution from $^{53}$Mn, particularly at higher initial $^{22}$Ne mass fractions, indicating a strong secondary production. Production of $^{52}$Cr is more mixed in the lower mass explosions, with competing contributions from $^{52}$Cr and $^{52}$, along with negligible $^{52}$Mn. $^{53}$Mn becomes a significant contributor to the abundance of $^{53}$Cr at higher metallicities, becoming comparable to the contribution form $^{53}$Fe. Non radiogenic contributions to $^{53}$Cr are negligible
For all sets, the yield of $^{50}$Cr rises with increasing metallicity of the WD progenitor above a threshold value of Z = 10$^{-4}$. $^{53}$Cr shows a much weaker rise. $^{54}$Cr is mostly primary for T1.4 models, while its (much weaker) production is secondary for other sets.


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CR_50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CR_50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CR_50.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CR_50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CR_50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CR_50.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CR_50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CR_50.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CR_50.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{50}$Cr are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:cr_50_radiogenic}
\end{sidewaysfigure}




In the T1.4 set, the $^{50}$Cr yields are dominated by two production peaks, at 7-9 \,GK and 3-5 \,GK temperature, respectively (Figure~\ref{fig:cr_50_radiogenic}). The first peak is primary, while the low temperature peak is secondary, rising with increasing metallicity. Only the T1.4Z0 model shows a relevant radiogenic contribution by $^{50}$Mn at lower temperatures, but the production is dominated by the first peak.
S1.0 and M0.8 sets only carry the secondary peak, explaining their smaller $^{50}$Cr production at low metallicities compared to T1.4. On the other hand, for all sets the strong secondary component in $^{50}$Cr causes this isotope to form up to about 10\% of all Cr ejecta (M0.8Z0.1 model).

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CR_52.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CR_52.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CR_52.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CR_52.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CR_52.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CR_52.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CR_52.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CR_52.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CR_52.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{52}$Cr are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:cr_52_radiogenic}
\end{sidewaysfigure}





The $^{52}$Cr abundance pattern is significantly more complex than $^{50}$Cr, revealing a larger number of production channels (Figure~\ref{fig:cr_52_radiogenic}). For the T1.4 set, primary $^{52}$Cr is directly produced in the hottest ejecta, with SN shock temperatures above 8 \,GK. Two additional peaks, from the eventual decay of $^{52}$Fe occur at around 7\,GK and 5\,GK. These are insensitive to the initial metallicity of the model, and contribute the majority of $^{52}$Cr. Finally, we obtain a secondary production of $^{52}$Cr at about 4\,GK in the T1.4Z0.014 and T1.4Z0.1 models. Small amounts of $^{52}$Mn are also produced in all models.
The Sxx and Mxx models all show the primary $^{52}$Fe production, and the secondary $^{52}$Cr channel at lower temperatures.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CR_53.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CR_53.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CR_53.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CR_53.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CR_53.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CR_53.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CR_53.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CR_53.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CR_53.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{53}$Cr are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:cr_53_radiogenic}
\end{sidewaysfigure}





In Figure~\ref{fig:cr_53_radiogenic}, for the T1.4 set, $^{53}$Cr is produced directly above 9\,GK in the innermost ejecta. For 8-9 \,GK the production is dominated by a primary peak of radiogenic $^{53}$Mn. Two additional $^{53}$Mn channels appear at lower temperatures, with the colder production peak in oxygen burning conditions becoming particularly relevant at super-solar metallicities, again demonstrating that it is a secondary production channel. Two broad primary peaks at 7-8 \,GK and about 5 \,GK are due to the radiogenic contribution from $^{53}$Fe.
$^{53}$Fe continues to be the primary radiogenic source of $^{53}$Cr in the S1.0 and M0.8 sets.
In agreement with T1.4 models, a secondary production of $^{53}$Mn and $^{53}$Cr is obtained at 3-4 \,GK.


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CR_54.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CR_54.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CR_54.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CR_54.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CR_54.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CR_54.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CR_54.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{54}$Cr are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:cr_54_radiogenic}
\end{sidewaysfigure}


 

In Figure~\ref{fig:cr_54_radiogenic}, $^{54}$Cr is produced directly at temperatures above 8 \,GK, while a secondary production peak is present at about 4 \,GK from the radiogenic decay of $^{54}$Mn.


\subsection{Manganese}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Mn_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Mn_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Mn_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of $^{55}$Mn.
 }
 \label{fig:Manganese_metalicity_multi}
\end{figure}


Mn is mono-isotopic, with only $^{55}$Mn being stable. It is formed in explosive silicon burning, the neutrino process and in SNIa \citep{woosley2002evolution}. Most of the solar manganese is produced in SNIa \citep{kobayashi2020origin}, it has also been proposed as a key tracer for differentiating the mass of SNIa progenitor \citep{eitner2020observational}. Figure \ref{fig:Manganese_metalicity_multi} shows the ejected mass of Mn from our three models with respect to metallicity, indicating a large radiogenic contribution across the range of Z investigated.

Figure \ref{fig:mn_55_radiogenic} shows the radiogenic contributions from the different models. In the low metallicity sub Chandrasekhar mass models, most production of Mn is as $^{55}$Co, with a negligible contribution from $^{55}$Fe. This contribution increases as the the secondary $^{55}$Fe component begins to dominate at lower temperatures, between 3 and 4 GK in explosive oxygen burning conditions. Production of $^{55}$Co is also boosted by this secondary component in both the S1.0 and M0.8 models. In the T1.4 models, we see that the production of $^{55}$Fe is again  boosted at higher metallicities, with a small primary secondary peak of $^{55}$Mn contributing at lower temperatures in in these models. This peak has a negligible impact on the total production of Mn. We see that the trace amount of $^{55}$Ni produced at intermediate temperatures in this model is suppressed with increasing initial $^{22}$Ne abundance while $^{55}$Fe production is boosted throughout the model. $^{55}$Cr production is comparable to the radiogenic $^{55}$Fe contribution, in contrast with the lower mass models where it is the dominant radiogenic contribution. Unfortunately, the half-life of $^{55}$Cr is 3.5 minutes, much too short to be able to observe in the expanding ejecta of a Type Ia explosion.


\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_MN_55.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_MN_55.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_MN_55.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_MN_55.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_MN_55.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_MN_55.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_MN_55.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_MN_55.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_MN_55.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{55}$Mn are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:mn_55_radiogenic}
\end{sidewaysfigure}

Manganese production is predicted to be sensitive to the mass of the progenitor model. \citet{truran1967nucleosynthesis} identifies Mn as being mainly produced as $^{55}$Co, consistent with the production presented in figure \ref{fig:mn_55_radiogenic}.  $^{55}$Mn production in the most extreme conditions is dependent on a normal, low $\alpha$, freeze out from NSE  \citep{seitenzahl2013solar,thielemann1986explosive} 

\citet{seitenzahl2013solar} states $^{55}$Co is the largest contributor to manganese yields at densities above 2x10$^{8}$ gcm$^{-3}$. In the T1.4 Chandrasekhar mass models, these densities cover the full range of peak temperatures (although not all of the particles have a density above this threshold density). $^{55}$Co is the dominant source of $^{55}$Mn in the T1.4Z0 model, and remains the largest contributor to ejected $^{55}$Mn mass however the relative contribution from $^{55}$Fe increases with increasing metallicity and at Z = 0.1 contributes on the order of 10\% of the ejected $^{55}$Mn mass. There is also a contribution from direct synthesis of $^{55}$Mn in the highest temperature regions, however this is small - of the order  1\% of total ejected mass of $^{55}$Mn in the T1.4Z0 model.

$^{55}$Co is destroyed at lower densities through the reaction $ ^{55}\mathrm{Co}(p,\gamma)^{56}\mathrm{Ni} $ \citep{seitenzahl2013solar} which we see in the differences (particularly at low metallicities) between M0.8 and the higher mass models. at Z = 0, the T1.4 model ejects 3.72X10$^{-3}$ M$_{\odot}$ of $^{55}$Mn, the S1.0 model 1.19x10$^{-4}$M$_{\odot}$ and the M0.8 model 2.24x10$^{-5}$ M$_{\odot}$.

\citet{kobayashi2020new} identify a positive correlation for the production of Mn with respect to initial metallicity, similar to the results presented here. They, however, see a decrease in the ejected mass of Mn with increasing progenitor mass, at odds with the findings of \citet{seitenzahl2013three} and this work. The reaction $ ^{52}\mathrm{Fe}(\alpha,p)^{55}\mathrm{Co} $ is identified as the main production channel for the bulk of $^{55}$Mn \citep{seitenzahl2013three}. The production of Mn with respect to Fe in SNIa has been extensively studied, and has been the subject of a number of GCE investigations \citep{seitenzahl2013solar,kobayashi2006galactic,eitner2020observational} as both Mn and Fe in the Milky Way are produced primarily in SNIa \citep{matteucci2009effect}. This [Mn/Fe] has been used in many publications to investigate the ration of Chandrasekhar to sub-Chandrasekhar SNIa progenitor.

\citet{eitner2020observational} consider the fraction of sub-Chandrasekhar mass SNIa to be as high as 75\%, due to the large [Mn/Fe] ratios possible in these low mass models. %\citet{eitner2020observational} also draw attention to the fact that even a 0.9M$_{sun}$ model would be too faint to be observed.

% Q. Where is incomplete Si burning in my peak T diagrams?
%
%\citet{bravo2012sensitivity} - sensitivity - reaction rates not so important
%\citet{parikh2013effects} - also sensitivity
%
%\citet{jordan2003nuclear} - NSE physics


\subsection{Iron}
\label{ssec:Iron_yields}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Fe_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Fe_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Fe_brox_yields_.eps} 
    \end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Fe, and its stable isotopes $^{54}$Fe, $^{56}$Fe, $^{57}$Fe and $^{58}$Fe.
 }
 \label{fig:Iron_metalicity_multi}
\end{figure}



Iron has 4 stable isotopes: $^{54}$Fe, $^{56}$Fe, $^{57}$Fe and $^{58}$Fe. $^{54,56,57}$Fe are all produced in explosive silicon burning or in SNIa explosions. $^{58}$Fe is produced in Chandrasekhar mass SNIa explosions in NSE or in the helium burning s-process \citep{woosley2002evolution}. Around 70\% of Fe in the universe is produced in SNIa explosions \citep{matteucci1986relative}. \citet{kobayashi2020new} find that up to 25\% of SNIa progenitors may be sub-Chandrasekhar mass WDs, while \citet{seitenzahl2013solar} find a value close to 50\%.

$^{54}$Fe, in all conditions, is produced directly. In figure \ref{fig:Iron_metalicity_multi} the ejected mass of the stable Fe isotopes is given, along with their radiogenic contributions, as a function of initial metallicity. There is a a small decrease in the abundance of elemental Fe ejected from the T1.4 and S1.0 models due to a reduction in the ejected mass of $^{56}$Fe with increasing initial metallicity. This is compensated for partially by an increase in the abundances of $^{54}$Fe in these two models, which occurs sharply at Z=0.0001 in the S1.0 and M0.8 models, and more gradually at super-solar metallicities in the Chandrasekhar mass model. The increase of over two orders of magnitude in the abundance of $^{54}$Fe is significant, particularly as this only becomes a significant contributor to the overall abundance of Fe in models other than T1.4 at super-solar metallicities. %This therefore may provide a possible tracer of supernova progenitor if the metallicity of the initial WD can be determined.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_FE_54.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_FE_54.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_FE_54.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_FE_54.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_FE_54.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_FE_54.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_FE_54.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_FE_54.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_FE_54.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{54}$Fe are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:fe_54_radiogenic}
\end{sidewaysfigure}



Figure \ref{fig:fe_54_radiogenic} shows the production of $^{56}$Fe in our models with respect to peak temperature. $^{56}$Fe is one of the largest components of the ejecta of all three models. While M0.8 has a smaller contribution than the others,  most metallicities still have mass fractions of $^{56}$Fe above 10\%. In T1.4 we can see that production is dominated by contributions from $^{56}$Ni, with a non-negligible contribution from direct synthesis of $^{56}$Fe at higher metallicities. This is more than offset by the reduction in production at intermediate peak temperatures from the Z = 0.014 and Z = 0.1 metallicity models. We also see this reduction in $^{56}$Fe in the S1.0 and M0.8 models, most clearly illustrated in figure \ref{fig:fe_56_radiogenic}. We see that $^{56}$Fe is produced directly at temperatures above 8\,GK, which is insensitive to metallicity effects. There is a more pronounced effect on the overall abundance of $^{56}$Fe vs metallicity in the 0.8M$_{\odot}$ model, however iron production actually increases for M0.8 at higher metallicities, due to a significant contribution from $^{54}$Fe.



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_FE_56.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_FE_56.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_FE_56.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_FE_56.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_FE_56.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_FE_56.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_FE_56.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_FE_56.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_FE_56.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{56}$Fe are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:fe_56_radiogenic}
\end{sidewaysfigure}



$^{57}$Fe has a large radiogenic contribution across all models. We see that $^{57}$Fe produced directly during the explosion accounts for ~1\% of the mass of $^{57}$Fe in the T1.4 models, where as it contributes almost nothing to the ejected mass in the sub Chandrasekhar models, where almost all production is through radiogenic contributions. These radiogenic contributions come mainly from $^{57}$Ni and $^{57}$Co, particularly in the lower mass models. There is a small contribution to $^{57}$Fe abundance from $^{57}$Mn and $^{57}$Cu in T1.4 which is negligible, and $^{57}$Cu production is still smaller at non-zero metallicity. Primary production of $^{57}$Fe does occur in models at higher metallicity, in the low temperature end. This constitutes a small fraction of the total ejected mass of $^{57}$Fe. $^{57}$Co production is boosted at higher metallicities, driving the increasing trend in all models in figure \ref{fig:Iron_metalicity_multi}.



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_FE_57.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_FE_57.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_FE_57.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_FE_57.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_FE_57.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_FE_57.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_FE_57.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_FE_57.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_FE_57.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{57}$Fe are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:fe_57_radiogenic}
\end{sidewaysfigure}



$^{58}$Fe is an interesting isotope, as only trace abundances of it are ever produced in the sub-Chandrasekhar models, whilst production in T1.4 models is both consistent over a range of metallicities (with a weak increase in production at super-solar) and with an ejected mass in the order of 0.001 M$_{\odot}$. Production at lower temperatures as initial metallicity increases is very similar between our three classes of model, with radiogenic $^{58}$Co contributing to most of$^{58}$Fe ejecta. At the highest temperature peaks in the T1.4 models (>8.5\,GK) direct nucleosynthesis of $^{58}$Fe dominates, below this there is a band of production where $^{58}$Co is the most abundant isotope in this isobar. The relatively simple nucleosynthesis pathways of $^{58}$Fe, where the majority is produced in the most extreme conditions, is a tracer for the progenitors of SNIa explosions.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_FE_58.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_FE_58.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_FE_58.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_FE_58.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_FE_58.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_FE_58.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_FE_58.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{58}$Fe are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:fe_58_radiogenic}
\end{sidewaysfigure}


\citet{timmes2003variations} has investigated the impact of metallicity on Fe production in SNIa. They find a linear dependence on metallicity, with a decrease in production as initial metallicity increases for metallicity close to solar or higher. Between 0.1 and 10x solar metallicity, a variation of 25\% in the production of Fe through it's radioactive progenitor $^{56}$Ni is observed. Models T1.4 and S1.0 have similar trends with metallicity, in agreement with the results of \citet{timmes2003variations}, showing a linear decrease in production over the range of metallicities investigated here. This decrease in the production of Fe is approximately 25\% across this metallicity range. The M0.8 model however does not show the same linear dependence as the higher mass models. We instead see an exponential decrease in the ejected mass of $^{56}$Ni to around 30\% of the initial ejected mass at Z = 0.

In figure \ref{fig:ni_56_vs_met} I compare the results of my models with \citet{timmes2003variations}. S1.0 matches the Chandrasekhar mass SNIa model of \citet{timmes2003variations} most closely. This is because the T1.4 model is 2 dimensional, as discussed in \citet{townsley2016tracer}, which decreases the neutronisation in the innermost 0.2 M$_{\odot}$ of the WD progenitor, resulting in the destruction of this stable iron group material as compared to a 1 dimensional model.


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/met_dependency_ni_yield.eps}


    \caption{Ejected mass of $^{56}$Ni as a function of initial metallicity.}
    \label{fig:ni_56_vs_met}
\end{figure}

\subsection{Cobalt}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Co_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Co_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Co_brox_yields_.eps} 
    \end{subfigure}

 \caption{
     As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of $^{59}$Co.
 }
 \label{fig:Cobalt_metalicity_multi}
\end{figure}











\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CO_59.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CO_59.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CO_59.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CO_59.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CO_59.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CO_59.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_CO_59.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_CO_59.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CO_59.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{59}$Co are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:co_59_radiogenic}
\end{sidewaysfigure}

$^{59}$Co is the only stable isotope of cobalt. It is produced in a variety of stellar environments - the helium burning s-process, $\alpha$-rich freeze-out, the neutrino process and SNIa explosions \citep{woosley2002evolution}.


$^{59}$Co has significant contributions from radiogenic sources across all models (figure \ref{fig:Cobalt_metalicity_multi}). We see that for the case of S1.0 and M0.8, there is a strong secondary effect in both the direct and radiogenic synthesis of $^{59}$Co, starting at Z = 0.001. In the models T1.4, there is no strong dependency on metallicity. The production of cobalt shows an increasing efficiency with an increase in the mass of the SNIa progenitor. M0.8 models show the strongest metallicity dependence, with an increase in production of almost 3 orders of magnitude between the model at Z = 0.001 and the maximum at Z = 0.1.


In figure \ref{fig:co_59_radiogenic}, we show that the radiogenic contribution to $^{59}$Co is dominated from $^{59}$Ni (at peak temperatures between 7.5 and 8.5 GK) and $^{59}$Cu (at intermediate and lower peak temperatures). $^{59}$Cu is produced directly at T > 8.5 GK. This radiogenic production of cobalt is insensitive to metallicity effects at temperatures above 5\,GK. The $^{59}$Ni ejecta is uniform across T1.4 modes at temperatures exceeding 7\,GK, and the increase at around T = 4 GK in models T1.40.014 and T1.4Z0.1 is small compared to contributions from deeper layers. Production of $^{59}$Cu in the intermediate peak temperature range is broadly insensitive to increasing metallicity, and as this contributes a large proportion of the $^{59}$Co production in this model, the production of Co is also therefore insensitive. The trace production of $^{59}$Zn observed in model T1.4Z0 is suppressed at metallicities above Z = 0. Production of $^{59}$Ni is significantly increased in the lower temperature region at higher metallicities, contributing to a slight increase in Co yields with increasing metallicity.

Production in the S1.0 models has two components - a large, narrow peak for T > 5.5 GK, and a broader shallower peak between 3.5 and 5.5 GK. In the S1.0Z0 model, both of these Co peaks are dominated by radiogenic $^{59}$Cu. As initial metallicity rises, the production of $^{59}$Cu is suppressed in the lower temperature peak, and the secondary component of $^{59}$Ni is boosted. In model S1.0Z0.1, production of $^{59}$Ni is boosted to the extent that it is comparable with the total contribution of $^{59}$Cu. 

In the S0.8 models, $^{59}$Co production is severely reduced as compared with the previous sets of models. S0.8Z0 has a small peak between 3.2 and 5\,GK, where the main contributor to ejected cobalt mass is from radioactive $^{59}$Cu. As seen in the S1.0 models, production of $^{59}$Cu is suppressed at higher metallicities, leading to $^{59}$Ni dominating the production, here with a small contributing abundance of $^{59}$Co which is directly made. The direct production of $^{59}$Co is boosted still further moving to higher metallicities; however, the contribution from $^{59}$Co is still small compared to $^{59}$Ni.






\subsection{Nickel}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ni_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ni_shen_yields_.eps} 
    \end{subfigure}


    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ni_brox_yields_.eps} 
    \end{subfigure}

 \caption{
     As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Ni, and its stable isotopes $^{58}$Ni, $^{60}$Ni, $^{61}$Ni, $^{62}$Ni and $^{64}$Ni.
 }
 \label{fig:Nickel_metalicity_multi}
\end{figure}


Nickel is composed of 5 stable isotopes: $^{58}$Ni, $^{60}$Ni, $^{61}$Ni, $^{62}$Ni and $^{64}$Ni. The isotopes $^{(58,60,61,62)}$Ni are produced during $\alpha$-rich freeze-out from NSE \citep{woosley2002evolution}, with the dominant source of $^{(58,60)}$Ni being SNIa \citep{pignatari2016nugrid}. $^{58}$Ni is the largest contributor to ejected elemental nickel from CCSN \citep{jerkstrand2015constraints}. Isotopes $^{(60,61,62,64)}$Ni also have contributions from the s-process during helium burning \citep{woosley2002evolution}. Only $^{61}$Ni is identified as having a large contribution from SNIa events in \citet{woosley2002evolution}, \citep{pignatari2016nugrid} identify $^{(61,62,64)}$Ni as having some contribution from AGB stars. \citet{kobayashi2020origin} find that the evolution of [Ni/Fe] vs [Fe/H] for elemental nickel is reproduced well with only contributions from CCSN and SNIa events, with other sources having a negligible impact.

Figure \ref{fig:Nickel_metalicity_multi} shows the metallicity dependence of the ejected elemental nickel and the stable isotopes, with radiogenic contributions. In the T1.4 models, there is an increase in the ejected mass of elemental nickel at around Z$_{\odot}$ from around 5x10$^{-2}$ M$_{\odot}$ to over 0.1 M$_{\odot}$ at Z = 0.1, driven by an increase in the production of $^{58}$Ni. In S1.0, we see a similar increase from a lower initial mass of approximately 6x10$^{-3}$ M$_{\odot}$ to nearly 0.1 M$_{\odot}$. In these models however the major contributor at low metallicities is $^{60}$Ni, which is suppressed above Z = 10$^{-3}$, although this is compensated for by the increase in production of $^{58}$Ni which becomes the dominant isotope and drives the metallicity dependence of elemental nickel. In M0.8, we see an increase in the abundance of $^{58}$Ni from 2.5x10$^{-5}$ at Z = 0 t0 3.6x10$^{-3}$ at Z = 0.1.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_NI_58.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_NI_58.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_NI_58.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_NI_58.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_NI_58.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_NI_58.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_NI_58.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_NI_58.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_NI_58.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{58}$Ni are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ni_58_radiogenic}
\end{sidewaysfigure}


In all models, we see an increase in the ejected mass of $^{58}$Ni with increasing metallicity, due to contributions from lower temperature regions of the SNIa explosion. Figure \ref{fig:ni_58_radiogenic} shows the mass fraction of $^{58}$Ni with respect to peak temperature in each particle. We see that the NSE regions of the T1.4 models are largely insensitive to the changing metallicity. Although there is a decrease in the radiogenic contributions from $^{58}$Cu, these are negligible at most peak temperatures, except in the T1.4Z0 model where a non-negligible contribution in the 5-6 GK range from $^{58}$Co is seen. Even so, this will have no impact on the total ejected yields. Because of the large contributions from NSE conditions, the proportional change in the abundance of $^{58}$Ni is less in the T1.4 model than for the S1.0 and M0.8 models, where we see a change in the ejected mass of $^{58}$Ni of over an order of magnitude (this is also due to the lower starting abundance). Production of $^{58}$Ni extends to the top of the oxygen burning region at approximately 3.5 GK, it is between 4 and 5 GK at which we see the increase in $^{58}$Ni production at higher metallicities in all models. 

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_NI_60.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_NI_60.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_NI_60.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_NI_60.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_NI_60.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_NI_60.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_NI_60.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_NI_60.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_NI_60.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{60}$Ni are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ni_60_radiogenic}
\end{sidewaysfigure}



Figure \ref{fig:ni_60_radiogenic} shows that the metallicity dependence of $^{60}$Ni production is similar between models T1.4 and S1.0, where the ejected mass of $^{60}$Ni decreases with increasing metallicity above approximately Z = 10$^{-2}$ for the T1.4 models and Z = 2x10$^{-3}$ for the S1.0 models. We see three areas of production in the T1.4Z0 model - one above 8 GK, one between 5 and 7 GK and a smaller peak between 4 and 5 GK, in the 8-9 GK region production is dominated through direct synthesis of $^{60}$Ni, due to the high density conditions in the central region. In the 5-6 GK peak, most $^{60}$Ni is synthesised as $^{60}$Zn. We see that this contribution decreases with increasing metallicity, driving the shallow decline of ejected $^{60}$Ni. In the T1.4Z0.014 model, we see that the low temperature peak has been boosted significantly, with direct production of $^{60}$Ni, this peak also extends further down to around 3.5 GK, corresponding with the lower edge of the oxygen burning region. This trend continues in T1.4Z0.1, where there is a significant boost to the $^{60}$Ni production in the oxygen burning region. In model S1.0, the highest temperature peak is missing, as no particles experience these conditions. We therefore see a much stronger metallicity dependence on the $^{60}$Ni for this model, with the total ejected mass of $^{60}$Ni decreasing as the metallicity increases. This is due to the same effects driving the decrease in the T1.4 models - namely a drop in production of $^{60}$Zn in the intermediate peak temperature region, but as there is not a large contribution from T > 6 GK regions in the S1.0 models, there is proportionally a much larger effect. While the low temperature oxygen burning region does increase significantly, it does not compensate for the lost material in the intermediate region. We see in figure \ref{fig:Nickel_metalicity_multi} that this effect causes $^{58}$Ni to become the dominant isotope in the S1.0 models at metallicities above Z = 4x10$^{-3}$.

In the M0.8 models we initially see the same trend of suppression of $^{60}$Zn production leading to a decrease in the $^{60}$Ni ejected mass however, since both the high temperature and most of the intermediate temperature region are absent in the M0.8 model, the Z = 0 mass of $^{60}$Ni is already low. When production moves to lower temperatures therefore, with $^{60}$Ni being synthesised directly, the ejected abundance of $^{60}$Ni increases compared to the Z = 0 value.

Shifts in the isotopic distribution of the iron group cannot be attributed to any one particular reaction, as the models are in NSE. In the oxygen burning region however, neutron capture reactions with the increased Y$_{e}$ of the system lead to the increase in production of $^{60}$Ni.

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_NI_61.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_NI_61.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_NI_61.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_NI_61.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_NI_61.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_NI_61.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_NI_61.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_NI_61.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_NI_61.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{61}$Ni are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ni_61_radiogenic}
\end{sidewaysfigure}

In figure \ref{fig:ni_61_radiogenic} we see that production of $^{61}$Ni is dominated by the intermediate and high temperature regions. In the T1.4 model sets, the ejected mass of $^{60}$Ni changes from 2.06x10$^{-4}$ M$_{\odot}$ at Z = 0 to 3.89x10$^{-4}$ M$_{\odot}$ at Z = 0.1. This is consistent with the results for other isotopes mainly produced in the high temperature regions, where the changing initial Y$_{e}$ has a marginal impact in the NSE conditions. The increase in production in the peak temperature region between 3.5 and 5 GK may be sufficient to account for the observed increase in ejected mass, however a very small increase in the higher temperature regions cannot be excluded. In the high temperature region, $^{61}$Ni is directly produced, in the intermediate peak temperature region $^{61}$Zn is the major contributor to ejected $^{61}$Ni mass (and this dominates the production overall). In the low temperature region, $^{61}$Ni is produced directly.

Similarly for the S1.0 models, there is a small increase in the ejected mass of $^{61}$Ni between S1.0Z0 (8.81x10$^{-5}$ M$_{\odot}$) and S1.0Z0.1 (1.47x10$^{-4}$ M$_{\odot}$). Production in the intermediate peak temperature region is insensitive to an increase in the initial $^{22}$Ne mass fraction, with $^{61}$Ni being synthesised as $^{61}$Zn, as in the T.14 models. The low temperature region is directly produced as $^{61}$Ni, and contributes only on the order of 0.1-1\% of the ejected mass of $^{61}$Ni in this model. With the high temperature region missing, the total ejected mass of $^{61}$Ni compared with the T1.4 models is a factor of two lower.

In the M0.8 models, both the intermediate and high temperature peaks are missing, so only the relatively small contribution from the oxygen burning region is seen, and only in non-negligible amounts above Z = 2x10$^{-2}$. We see that in the case of $^{61}$Ni, the intermediate peak of production is slightly higher than e.g. $^{56,57}$Fe, leading to there being no contribution from the higher temperature regions of this class of model.



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_NI_62.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_NI_62.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_NI_62.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_NI_62.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_NI_62.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_NI_62.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_NI_62.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_NI_62.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{62}$Ni are shown, arranged as in figure \ref{fig:o_16_radiogenic}. Model M0.8Z0 produces no $^{62}$Ni, and so the subplot for this model is omitted.}
 \label{fig:ni_62_radiogenic}
\end{sidewaysfigure}



Figure \ref{fig:ni_62_radiogenic} shows the production of $^{62}$Ni. The trend in production is very similar to that for $^{61}$Ni, with a large contribution from the high and intermediate peak temperature regions. In the T1.4 models, we see that production of $^{62}$Ni in the 8-9 GK region is larger than the production of $^{61}$Ni in that same region. This is due to the increased density which causes production to shift to more neutron rich isotopes in the central region. Production is through direct synthesis of $^{62}$Ni. 

The intermediate peak temperature region from around 5 to 7 GK is very similar to the $^{61}$Ni production region in the T1.4 models, with the mass fraction of $^{62}$Ni being around 0.1\%. $^{62}$Zn is the major contributor to abundances in this region as direct production ceases at 8 GK. Production in this region is sensitive to the initial metallicity, increasing from the initial approximately 0.2\% by mass fraction in T1.4Z0 to around 3\% in model T1.4Z0.1. We also see a small contribution in the oxygen burning region through direct production of $^{62}$Ni, although this has a negligible effect on the ejected mass. 

In the S1.0 series of models, we again see an increase in the production at intermediate peak temperatures. As the highest temperatures in this model are at approximately 6 GK, we see only the lower end of this production region, which significantly reduces the ejected mass of $^{62}$Ni from these models. There is again a small contribution at around 3.5 GK but this is negligible.

In the models M0.8, there is no production at Z = 0, and only a marginal production at Z = Z$_{\odot}$. The 6 GK region is completely absent from this model and so the production through formation of $^{62}$Zn is not possible. We therefore only have the small secondary contribution in the lower temperature region, as seen for the T1.4 and S1.0 models. 

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_NI_64.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_NI_64.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_NI_64.eps} 
    \end{subfigure}
    

 \caption{The abundance distributions of $^{64}$Ni. Only models T1.4Z0,T1.4Z0.014 and T1.4Z0.1 produce $^{64}$Ni. Only the T1.4 models show production of $^{64}$Ni, as such the other models have been omitted.}
 \label{fig:ni_64_radiogenic}
\end{sidewaysfigure}

Figure \ref{fig:ni_64_radiogenic} shows the production of $^{64}$Ni in the T1.4 models. Production is confined to the high peak temperature region above 8 GK, and as such the effect of initial metallicity is suppressed, as weak interactions in the core of the WD change the Y$_{e}$ of the interior. There is a very mild dependence on initial metallicity however, with the ejected mass of $^{64}$Ni changing from 8.89x10$^{-7}$ M$_{\odot}$ at Z = 0 to 1.05x10$^{-6}$ M$_{\odot}$ at Z = 0.1. $^{64}$Ni is directly produced in this region, with no radiogenic component.






\subsection{Copper}

Copper has two stable isotopes: $^{63}$Cu and $^{65}$Cu.  $^{63}$Cu is produced in the helium burning s-process, carbon, and neon burning in massive stars and $^{65}$Cu is mainly produced in the s-process in massive stars \citep{woosley2002evolution}. SNIa do not produce copper efficiently. 

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Cu_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Cu_shen_yields_.eps} 
    \end{subfigure}


    %\begin{subfigure}[t]{0.65\textwidth}
    %    \centering
    %    \includegraphics[width=\textwidth]{figures/Cu_brox_yields_.eps} 
    %\end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Cu, and its stable isotopes $^{63}$Cu and $^{65}$Cu. The M0.8 models are excluded as copper is not produced efficiently in these low.
 }
 \label{fig:Copper_metalicity_multi}
\end{figure}


In figure \ref{fig:Copper_metalicity_multi} both $^{63}$Cu and $^{65}$Cu show a large radiogenic contributions to their abundances in both the T1.4 and S1.0 models. These models also have a similar distribution with respect to metallicity. At approximately Z = 2$x$10$^{-3}$ and 10$^{-3}$ for T1.4 and S1.0 respectively, the production of $^{63}$Cu is reduced dramatically. At super-solar metallicities, $^{63}$Cu production increases again for the region around Z = Z$_{\odot}$ we see that $^{65}$Cu becomes the most abundant copper isotope in the ejecta. 





\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CU_63.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CU_63.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CU_63.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CU_63.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CU_63.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CU_63.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_CU_63.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{63}$Cu are shown, arranged as in figure \ref{fig:o_16_radiogenic}. The models M0.8Z0 and M0.8Z0.014 do not produce $^{63}$Cu and are therefore omitted.}
 \label{fig:cu_63_radiogenic}
\end{sidewaysfigure}


Figure \ref{fig:cu_63_radiogenic} illustrates the complicated nucleosynthesis of $^{63}$Cu, particularly in the T1.4 models. In T1.4Z0, there is a contribution from $^{63}$Ni at the most extreme temperature peaks, which becomes negligible for T < 8.5 GK. In this region, we next see the direct synthesis of $^{63}$Cu. This is quickly replaced, from T = 8 GK to the coolest temperature at which $^{63}$Cu is produced at around 5.2 GK by radiogenic contributions from $^{63}$Ga and $^{63}$Zn. The change in production between $^{63}$Ga and $^{63}$Zn is more ordered in the T1.4Z0.014 model: the lower temperature production below 6.5 GK is dominated by $^{63}$Ga, between 6.5 and 8 GK $^{63}$Zn has the largest radiogenic contribution. In T1.4Z0.1, production of $^{63}$Zn is boosted across the whole temperature range from 5.2 to 8\,GK, $^{63}$Ga production is reduced in this same range. The innermost ejecta stays consistent with lower metallicities.

Production in the S1.0 models follows a similar, non-linear trend with metallicity, whereby $^{63}$Ga and $^{63}$Zn exchange positions as the most abundant isotope. In model S1.0Z0, $^{63}$Ga is the most abundant. In the S1.0Z0.014 model, there is a reduction in the overall ejected mass of $^{63}$Cu, as the reduction in $^{63}$Ga is not fully compensated for by the increase in the abundance of $^{63}$Zn. Total ejected mass is then similar again in S1.0Z0.1, as $^{63}$Zn continues to increase with metallicity.





\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_CU_65.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_CU_65.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_CU_65.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_CU_65.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_CU_65.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_CU_65.eps} 
    \end{subfigure}
    
   
    

 \caption{The abundance distributions of $^{65}$Cu are shown, arranged as in figure \ref{fig:o_16_radiogenic}. There is no production of $^{65}$Cu in the M0.8 models, these are therefore omitted.}
 \label{fig:cu_65_radiogenic}
\end{sidewaysfigure}


Figure \ref{fig:cu_65_radiogenic} shows the production of $^{65}$Cu in the T1.4 and S1.0 models. There is no low temperature contribution to the ejected mass of $^{65}$Cu at any metallicity. Production in the T1.4Z0 model is largely in the temperature range 5.2 - 7.8 GK, where $^{65}$Cu is produced as the radioisotope $^{65}$Ge. In the high temperature peak above 8 GK, $^{65}$Cu is produced directly. There is a shallow trend with respect to metallicity in the ejected mass of $^{65}$Cu in the T1.4 models, from 1.47 to 2.99x10$^{-6}$ M$_{\odot}$. Production becomes more tightly centered around 6 GK but with a larger contribution from this narrower range of temperatures, especially at the higher end of the intermediate peak temperature range.

Because this peak temperature range is missing in the S1.0 models, we see that the $^{65}$Cu production peaks at around solar metallicity. As the increase in the temperature in the lower end of the intermediate production region becomes larger, the slight increase in production at those temperatures is not enough to compensate for the loss of production sites. In all three models shown for S1.0, $^{65}$Cu is produced as a combination of $^{65}$Ge and $^{65}$Ga. 


\subsection{Zinc}



\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Zn_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Zn_shen_yields_.eps} 
    \end{subfigure}


    %\begin{subfigure}[t]{0.65\textwidth}
    %    \centering
    %    \includegraphics[width=\textwidth]{figures/Zn_brox_yields_.eps} 
    %\end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Zn, and its stable isotopes $^{64}$Zn, $^{66}$Zn, $^{67}$Zn and $^{68}$Zn. There is no production of zinc in the M0.8 models and therefore the plot is omitted.
 }
 \label{fig:Zinc_metalicity_multi}
\end{figure}


Zinc has 5 stable isotopes: $^{64}$Zn, $^{66}$Zn, $^{67}$Zn, $^{68}$Zn and $^{70}$Zn. None of the models investigated here produce $^{70}$Zn, as such, we will not discuss this isotope further. $^{64}$Zn is produced in neutrino driven winds \citep{woosley2002evolution} - where neutrino interactions in dense stellar environments with large neutrino fluxes cause neutrino captures. It is also formed in the helium burning s-process in massive stars, and $\alpha$-rich freeze-out from NSE. $^{66}$Zn is likewise produced in the helium burning s-process and $\alpha$-rich freeze-out, however \citet{woosley2002evolution} also identify $^{66}$Zn as having a significant contribution from Chandrasekhar mass SNIa explosions. $^{68}$Zn is produced only in massive stars through the helium burning s-process \citep{woosley2002evolution}. 

Zinc production in the models T1.4 and S1.0 is very similar (figure \ref{fig:Zinc_metalicity_multi}, with similar trends for all of the isotopes produced aside from a scaling factor between models for these isotopes. The elemental trend of Zn production decreases at around Z = 0.001 by approximately a factor of 5, following the trend of $^{64}$Zn. At the same time $^{66}$Zn production increases becoming the most abundant isotope at higher metallicities. 

\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_ZN_64.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_ZN_64.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_ZN_64.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_ZN_64.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_ZN_64.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_ZN_64.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_ZN_64.eps} 
    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{64}$Zn are shown, arranged as in figure \ref{fig:o_16_radiogenic}. from the M0.8 models, only M0.8Z0.1 has even a trace production of $^{64}$Zn. Because of this, we omitted the M0.8 plots at lower metallicities.}
 \label{fig:zn_64_radiogenic}
\end{sidewaysfigure}

Production of $^{64}$Zn in fig \ref{fig:zn_64_radiogenic} shows that production in all T1.4 models is dominated by the radio-isotope $^{64}$Ge. The contribution of $^{64}$Ga to the ejected abundance is never large, although it increases at higher metallicities as the intermediate peak temperature range production of $^{64}$Ge shrinks.

We see that production in the S1.0 models is also primarily through synthesis of $^{64}$Ge. We clearly see the decrease in the overall production of $^{64}$Zn with the reduction in $^{64}$Ge and $^{64}$Ga produced at between peak temperatures of 5.5-6 GK. We also observe the rise in direct production of $^{64}$Zn, although the absolute abundance is only on the order of 5\% in the S1.0Z0.1 model. 




\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_ZN_66.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_ZN_66.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_ZN_66.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_ZN_66.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_ZN_66.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_ZN_66.eps} 
    \end{subfigure}
    
   
    

 \caption{The abundance distributions of $^{66}$Zn are shown, arranged as in figure \ref{fig:o_16_radiogenic}. M0.8 models do not produce $^{66}$Zn and are therefore omitted.}
 \label{fig:zn_66_radiogenic}
\end{sidewaysfigure}


The production of $^{66}$Zn is largely centered in the intermediate peak temperature range starting at approximately 5.2\,GK and continuing to 8\,GK. $^{66}$Zn is produced as $^{66}$Ge in the T1.4Z0 model, with trace amounts of other isotopes. Production is nearly identical in the T1.4Z0.014 model, with only a slight increase in the production of $^{66}$Ga (already with very low abundance). The range of peak temperatures suitable for production is less broad in the T1.4Z0.1 model, with production at the upper limit of the production region becoming less efficient.

Production in all three S1.0 models is very similar, with a slight increase in the amount of $^{66}$Zn ejected caused by an increase in the radiogenic contribution of $^{66}$Ge. Trace amounts of $^{66}$Ga do not affect the overall yields.








\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_ZN_67.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_ZN_67.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_ZN_67.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_ZN_67.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_ZN_67.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_ZN_67.eps} 
    \end{subfigure}
    
   
    

 \caption{The abundance distributions of $^{67}$Zn are shown, arranged as in figure \ref{fig:o_16_radiogenic}. The M0.8 models do not produce $^{67}$Zn and are therefore omitted.}
 \label{fig:zn_67_radiogenic}
\end{sidewaysfigure}


$^{67}$Zn has a similar trend as for $^{66}$Zn (figure \ref{fig:zn_67_radiogenic}). In model T1.4Z0 we see a comparable contribution to the ejected mass of $^{67}$Zn from both $^{67}$Ge and $^{67}$As. As the initial metallicity increases, both of these contributions become secondary to the increased production of $^{67}$Ge, culminating in T1.4Z0.1, where only trace amounts of $^{67}$Ge and $^{67}$Cu contribute to the abundance of $^{67}$Zn.








\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_ZN_68.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_ZN_68.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_ZN_68.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_ZN_68.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_ZN_68.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_ZN_68.eps} 
    \end{subfigure}
    
   

    \caption{The abundance distributions of $^{68}$Zn are shown, arranged as in figure \ref{fig:o_16_radiogenic}. The M0.8 models do not produce $^{67}$Zn and are therefore omitted.}
 \label{fig:zn_68_radiogenic}
\end{sidewaysfigure}


Production of $^{68}$Zn, again occurs mainly at intermediate peak temperatures from 5.2 to 7\,GK. In the model T1.4Z0, we see that there is a small contribution to $^{68}$Zn from $^{68}$As, with the bulk of material being synthesised as $^{68}$Se. $^{68}$Se production is reduced as the metallicity increases, leading to an overall decrease in the ejected mass of $^{68}$Zn and and increase in the $^{68}$Ge to $^{68}$Se ratio. In model T1.4Z0.1, $^{68}$Se is no longer the most abundant isotope, $^{68}$Ge has become more favorable to produce.

In the S1.0 models, we again note that the nucleosynthesis is similar, with $^{68}$Se being the most abundant isotope in the S1.0Z0 models, a decrease in the production of $^{68}$Se as the initial metallicity increases, and then production becoming more reliant on $^{68}$Ge, with $^{68}$Se as a trace isotope only at Z = 0.1.


\subsection{Germanium}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ge_dean_yields_.eps} 
    \end{subfigure}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Ge_shen_yields_.eps} 
    \end{subfigure}


    %\begin{subfigure}[t]{0.65\textwidth}
    %    \centering
    %    \includegraphics[width=\textwidth]{figures/Ge_brox_yields_.eps} 
    %\end{subfigure}

 \caption{
    As in Figure \ref{fig:Oxygen_metalicity_multi} but for ejected mass of Ge, and its stable isotopes  $^{70}$Ge and $^{72}$Ge. The M0.8 models do not produce Ge and so that figure has been omitted.
 }
 \label{fig:Germanium_metalicity_multi}
\end{figure}

Germanium consists of five stable isotopes - $^{70}$Ge, $^{72}$Ge, $^{73}$Ge, $^{74}$Ge and $^{76}$Ge. Only $^{70}$Ge and $^{72}$Ge are produced in any of our models and so we will restrict our discussion to these isotopes. $^{70}$Ge is and s only species, produced in the pre-explosive massive stars of CCSN \citep{pignatari2016nugrid}.

Figure \ref{fig:Germanium_metalicity_multi} shows the production of germanium in the various categories of model with respect to metallicity. While the M0.8 models do not produce Ge, both the T1.4 and S1.0 models do produce trace amounts. $^{72}$Ge contributes less than 1\% to elemental germanium in the T1.4 models, and less still to the S1.0 models. It is also not overproduced with respect to solar abundances and as such we will not discuss $^{72}$Ge further. We see that $^{70}$Ge has a fairly strong secondary component, with an increase in ejected mass of over an order of magnitude. This trend continues smoothly for the T1.4 models, however for the S1.0 models at Z = 0.1 we see a decrease in the total ejected mass.






\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_GE_70.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_GE_70.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_GE_70.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_GE_70.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_GE_70.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_GE_70.eps} 
    \end{subfigure}
    
%    \begin{subfigure}[text]{0.28\textwidth}
%        \centering
%        \includegraphics[width=1\textwidth]{figures/Miles_z_0_GE_70.eps}
%    \end{subfigure}%
%    \begin{subfigure}[text]{0.28\textwidth}
%        \centering
%        \includegraphics[width=1\textwidth]{figures/Miles_z_0_014_GE_70.eps} 
%    \end{subfigure}%
%    \begin{subfigure}[text]{0.28\textwidth}
%        \centering
%        \includegraphics[width=1\textwidth]{figures/Miles_z_0_1_GE_70.eps} 
%    \end{subfigure}
    
    

 \caption{The abundance distributions of $^{70}$Ge are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:ge_70_radiogenic}
\end{sidewaysfigure}

In figure \ref{fig:ge_70_radiogenic}, the production of $^{70}$Ge in the T1.4 models is broadly consistent through all metallicities, with a slight increase in production at temperatures close to 6\,GK as the initial metallicity increases. We see that production in the S1.0 models is similar, for the peak temperatures it shares with T1.4. 









\subsection{Selenium}

Although only produced in trace amounts in high metallicity Chandrasekhar mass models, these models do show an overproduction of $^{74}$Se.


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Se_dean_yields_.eps} 
    \end{subfigure}

%    \begin{subfigure}[t]{0.65\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/Se_shen_yields_.eps} 
%    \end{subfigure}
%
%
%    \begin{subfigure}[t]{0.65\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/Se_brox_yields_.eps} 
%    \end{subfigure}

 \caption{
 The ejected mass for the element Se and its stable isotopes is shown for the model set T1.4 The elemental yields take into account the radiogenic contribution. For isotopes, decayed and undecayed abundances are shown (continuous lines with crosses and dot-dashed lines with empty circles, respectively). There is no production in either of the other two categories of model. 
 }
 \label{fig:Selenium_metalicity_multi}
\end{figure}



\begin{sidewaysfigure}
    \centering
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_SE_74.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_014_SE_74.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Townsley_z_0_1_SE_74.eps} 
    \end{subfigure}
    
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/blank_plot.eps}
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_014_SE_74.eps} 
    \end{subfigure}%
    \begin{subfigure}[text]{0.28\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Shen_z_0_1_SE_74.eps} 
    \end{subfigure}
    
   

 \caption{The abundance distributions of $^{74}$Se are shown, arranged as in figure \ref{fig:o_16_radiogenic}.}
 \label{fig:se_74_radiogenic}
\end{sidewaysfigure}


As we can see in figure \ref{fig:se_74_radiogenic}, production of $^{74}$Se is limited in Type Ia SN. It is almost completely absent in sub-Chandrasekhar mass models, and at low metallicities the contribution to the ejecta is negligible. Even in models T1.40.014 and T1.40.01, the abundance of $^{74}$Se is small however the increase in production between these models does mean that there is an overproduction of $^{74}$Se in Chandrasekhar mass Type IaSN at high initial metallicity.

\subsection{All Yields Comparison}

Finaly, figure \ref{fig:type_Ia_sectrum} shows the log$_{10}$ of the ejected mass of each isotope in each of the three SNIa models. Metallicity is given on the y-axis, with the T1.4, S1.0 and M0.8 models shown in the top, middle and bottom panels respectively. It can be seen that production is broadly consistent between these three classes of model, with $\alpha$-chain ind iron group isotopes contributing the largest fraction of the ejected mass. We also see clearly the effect of initiall metallicity in, for example $^{54}$Cr and $^{58}$Fe. Production of $^{64}$Ni is exclusive to the T1.4 model.

\begin{sidewaysfigure}
    \centering
       \includegraphics[width=1\textwidth]{Chapters/ejecta_spectra.eps} 
    
 \caption{This plot shows the ejected mass of each stable isotope for all three models, at all metallicities. Stable isotopes with significant metallicity trends are easily identified.}
 \label{fig:type_Ia_sectrum}
\end{sidewaysfigure}










==> Chapters/shen_table_production_factors.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
  Element & A & $^{22}$Ne = 0  & 1e-7 & 1e-6 & 1e-5 & 1e-4 & 1e-3 & 2e-3 & 5e-3 & 1e-2 & 1.4e-2 & 2e-2 & 5e-2 & 1e-1 \\ 
\hline
C  & 12 & 3.62e-01 & 3.62e-01 & 3.62e-01 & 3.62e-01 & 3.61e-01 & 3.59e-01 & 3.58e-01 & 3.54e-01 & 3.51e-01 & 3.50e-01 & 3.48e-01 & 3.41e-01 & 3.31e-01  \\
C  & 13 & 2.01e-05 & 2.01e-05 & 2.03e-05 & 1.99e-05 & 2.01e-05 & 4.03e-05 & 8.18e-05 & 2.83e-04 & 6.85e-04 & 1.03e-03 & 1.57e-03 & 4.22e-03 & 8.07e-03  \\
N  & 14 & 1.75e-05 & 1.75e-05 & 1.75e-05 & 1.74e-05 & 2.35e-05 & 1.26e-04 & 2.15e-04 & 4.14e-04 & 6.31e-04 & 7.41e-04 & 8.64e-04 & 1.34e-03 & 1.93e-03  \\
N  & 15 & 3.74e-01 & 3.74e-01 & 3.72e-01 & 3.53e-01 & 1.71e-01 & 6.17e-03 & 2.26e-03 & 8.22e-04 & 5.57e-04 & 5.22e-04 & 5.69e-04 & 2.68e-03 & 1.13e-02  \\
O  & 16 & 7.91e+00 & 7.91e+00 & 7.91e+00 & 7.92e+00 & 7.98e+00 & 8.19e+00 & 8.30e+00 & 8.55e+00 & 8.80e+00 & 8.91e+00 & 9.01e+00 & 9.01e+00 & 8.42e+00  \\
O  & 17 & 1.37e-04 & 1.37e-04 & 1.39e-04 & 1.61e-04 & 5.67e-04 & 9.53e-03 & 1.74e-02 & 2.90e-02 & 3.53e-02 & 3.78e-02 & 4.07e-02 & 4.32e-02 & 3.91e-02  \\
O  & 18 & 3.65e-07 & 3.66e-07 & 3.70e-07 & 4.12e-07 & 1.01e-06 & 8.53e-06 & 1.39e-05 & 2.66e-05 & 4.54e-05 & 5.80e-05 & 8.16e-05 & 5.38e-04 & 2.27e-03  \\
F  & 19 & 2.80e-04 & 2.80e-04 & 2.78e-04 & 2.64e-04 & 1.78e-04 & 5.22e-05 & 6.47e-05 & 1.30e-04 & 2.05e-04 & 2.67e-04 & 4.03e-04 & 8.94e-04 & 9.81e-04  \\
Ne & 20 & 4.24e-01 & 4.24e-01 & 4.24e-01 & 4.24e-01 & 4.24e-01 & 4.18e-01 & 4.12e-01 & 3.99e-01 & 3.82e-01 & 3.71e-01 & 3.57e-01 & 3.12e-01 & 2.67e-01  \\
Ne & 21 & 1.16e-03 & 1.16e-03 & 1.16e-03 & 1.19e-03 & 1.55e-03 & 1.48e-02 & 4.15e-02 & 1.15e-01 & 1.99e-01 & 2.72e-01 & 4.38e-01 & 1.50e+00 & 3.43e+00  \\
Ne & 22 & 6.23e-05 & 6.23e-05 & 6.24e-05 & 6.27e-05 & 9.00e-05 & 1.31e-03 & 3.46e-03 & 1.31e-02 & 3.57e-02 & 5.69e-02 & 9.32e-02 & 3.50e-01 & 9.76e-01  \\
Na & 23 & 8.94e-02 & 8.94e-02 & 8.93e-02 & 8.91e-02 & 8.63e-02 & 7.59e-02 & 7.65e-02 & 9.21e-02 & 1.25e-01 & 1.56e-01 & 2.18e-01 & 5.64e-01 & 1.43e+00  \\
Mg & 24 & 1.27e+01 & 1.27e+01 & 1.27e+01 & 1.27e+01 & 1.28e+01 & 1.19e+01 & 1.07e+01 & 7.81e+00 & 5.14e+00 & 3.95e+00 & 2.92e+00 & 1.54e+00 & 2.04e+00  \\
Mg & 25 & 1.03e-03 & 1.03e-03 & 1.04e-03 & 1.05e-03 & 1.45e-03 & 1.63e-02 & 2.59e-02 & 5.77e-02 & 1.19e-01 & 1.77e-01 & 2.74e-01 & 9.18e-01 & 2.88e+00  \\
Mg & 26 & 3.68e-03 & 3.68e-03 & 3.68e-03 & 3.74e-03 & 4.43e-03 & 1.17e-02 & 1.90e-02 & 3.90e-02 & 7.09e-02 & 9.57e-02 & 1.33e-01 & 3.86e-01 & 1.49e+00  \\
Al & 27 & 2.95e-01 & 2.95e-01 & 2.94e-01 & 2.92e-01 & 2.71e-01 & 7.11e-01 & 1.21e+00 & 2.02e+00 & 2.51e+00 & 2.64e+00 & 2.69e+00 & 3.02e+00 & 5.09e+00  \\
Si & 28 & 2.91e+02 & 2.91e+02 & 2.91e+02 & 2.91e+02 & 2.92e+02 & 2.96e+02 & 2.98e+02 & 3.00e+02 & 2.99e+02 & 2.99e+02 & 2.98e+02 & 2.94e+02 & 2.85e+02  \\
Si & 29 & 7.44e-01 & 7.44e-01 & 7.43e-01 & 7.37e-01 & 7.67e-01 & 2.75e+00 & 3.50e+00 & 4.69e+00 & 5.80e+00 & 6.53e+00 & 7.67e+00 & 1.73e+01 & 6.93e+01  \\
Si & 30 & 5.67e-01 & 5.67e-01 & 5.63e-01 & 5.21e-01 & 2.34e-01 & 4.98e-01 & 1.64e+00 & 5.86e+00 & 1.29e+01 & 1.81e+01 & 2.59e+01 & 7.82e+01 & 2.47e+02  \\
P  & 31 & 4.71e+00 & 4.71e+00 & 4.69e+00 & 4.53e+00 & 3.19e+00 & 3.72e+00 & 5.77e+00 & 1.12e+01 & 1.84e+01 & 2.32e+01 & 2.96e+01 & 5.71e+01 & 8.64e+01  \\
S  & 32 & 3.52e+02 & 3.52e+02 & 3.52e+02 & 3.52e+02 & 3.51e+02 & 3.45e+02 & 3.43e+02 & 3.42e+02 & 3.39e+02 & 3.35e+02 & 3.29e+02 & 2.91e+02 & 2.29e+02  \\
S  & 33 & 6.15e+00 & 6.15e+00 & 6.17e+00 & 6.30e+00 & 7.58e+00 & 1.30e+01 & 1.68e+01 & 2.65e+01 & 3.86e+01 & 4.63e+01 & 5.60e+01 & 8.94e+01 & 1.04e+02  \\
S  & 34 & 1.36e-01 & 1.36e-01 & 1.34e-01 & 1.23e-01 & 4.78e-02 & 2.39e+00 & 7.00e+00 & 2.22e+01 & 4.94e+01 & 7.20e+01 & 1.06e+02 & 2.80e+02 & 5.11e+02  \\
S  & 36 & 9.28e-08 & 9.28e-08 & 9.32e-08 & 9.75e-08 & 1.78e-07 & 5.42e-04 & 3.23e-03 & 2.55e-02 & 1.07e-01 & 2.30e-01 & 5.37e-01 & 8.02e+00 & 7.19e+01  \\
Cl & 35 & 8.07e-01 & 8.07e-01 & 8.04e-01 & 7.74e-01 & 5.74e-01 & 1.03e+00 & 1.67e+00 & 3.35e+00 & 5.85e+00 & 7.71e+00 & 1.02e+01 & 1.77e+01 & 1.97e+01  \\
Cl & 37 & 6.07e-01 & 6.07e-01 & 6.09e-01 & 6.29e-01 & 8.00e-01 & 1.50e+00 & 2.01e+00 & 3.26e+00 & 4.87e+00 & 5.96e+00 & 7.33e+00 & 1.18e+01 & 1.35e+01  \\
Ar & 36 & 3.99e+02 & 3.99e+02 & 3.99e+02 & 3.99e+02 & 3.96e+02 & 3.83e+02 & 3.76e+02 & 3.66e+02 & 3.55e+02 & 3.47e+02 & 3.35e+02 & 2.77e+02 & 2.06e+02  \\
Ar & 38 & 4.87e-02 & 4.92e-02 & 4.95e-02 & 4.70e-02 & 4.10e-02 & 1.58e+00 & 4.09e+00 & 1.30e+01 & 3.06e+01 & 4.63e+01 & 7.09e+01 & 1.88e+02 & 3.13e+02  \\
Ar & 40 & 9.23e-09 & 9.23e-09 & 9.27e-09 & 9.64e-09 & 1.46e-08 & 2.85e-05 & 1.47e-04 & 1.03e-03 & 5.09e-03 & 1.24e-02 & 3.50e-02 & 5.66e-01 & 3.30e+00  \\
K  & 39 & 5.51e-01 & 5.52e-01 & 5.51e-01 & 5.37e-01 & 4.77e-01 & 1.89e+00 & 3.31e+00 & 6.64e+00 & 1.11e+01 & 1.42e+01 & 1.81e+01 & 2.96e+01 & 2.93e+01  \\
K  & 40 & 9.10e-05 & 9.10e-05 & 9.14e-05 & 9.49e-05 & 1.67e-04 & 4.73e-02 & 1.08e-01 & 3.51e-01 & 1.00e+00 & 1.73e+00 & 3.02e+00 & 6.90e+00 & 5.46e+00  \\
K  & 41 & 8.71e-01 & 8.71e-01 & 8.75e-01 & 9.16e-01 & 1.30e+00 & 2.70e+00 & 3.78e+00 & 6.39e+00 & 9.73e+00 & 1.19e+01 & 1.45e+01 & 2.10e+01 & 1.90e+01  \\
Ca & 40 & 3.68e+02 & 3.68e+02 & 3.68e+02 & 3.68e+02 & 3.65e+02 & 3.50e+02 & 3.42e+02 & 3.30e+02 & 3.16e+02 & 3.06e+02 & 2.93e+02 & 2.41e+02 & 1.83e+02  \\
Ca & 42 & 9.93e-03 & 9.94e-03 & 9.94e-03 & 9.64e-03 & 5.63e-03 & 6.98e-01 & 2.01e+00 & 7.19e+00 & 1.82e+01 & 2.82e+01 & 4.42e+01 & 1.12e+02 & 1.52e+02  \\
Ca & 43 & 7.27e-01 & 7.26e-01 & 7.16e-01 & 6.96e-01 & 5.03e-01 & 8.55e-01 & 1.90e+00 & 3.30e+00 & 3.62e+00 & 3.50e+00 & 3.35e+00 & 2.35e+00 & 1.62e+00  \\
Ca & 44 & 1.58e+01 & 1.56e+01 & 1.57e+01 & 1.59e+01 & 1.57e+01 & 1.53e+01 & 1.50e+01 & 1.41e+01 & 1.32e+01 & 1.26e+01 & 1.18e+01 & 8.76e+00 & 5.86e+00  \\
Ca & 46 & 2.02e-13 & 2.02e-13 & 2.05e-13 & 2.34e-13 & 9.31e-13 & 9.10e-09 & 1.55e-07 & 5.43e-06 & 8.34e-05 & 3.37e-04 & 1.47e-03 & 3.01e-02 & 1.98e-01  \\
Ca & 48 & 3.81e-23 & 3.82e-23 & 3.92e-23 & 5.04e-23 & 5.05e-22 & 1.15e-16 & 7.93e-15 & 7.06e-13 & 2.48e-11 & 2.04e-10 & 1.19e-09 & 3.13e-07 & 3.03e-05  \\
Sc & 45 & 3.23e-01 & 3.22e-01 & 3.24e-01 & 3.44e-01 & 5.68e-01 & 1.16e+00 & 1.37e+00 & 1.87e+00 & 2.45e+00 & 2.81e+00 & 3.22e+00 & 4.00e+00 & 3.96e+00  \\
Ti & 46 & 5.63e-01 & 5.72e-01 & 5.77e-01 & 5.43e-01 & 5.01e-01 & 6.17e-01 & 1.65e+00 & 6.44e+00 & 1.66e+01 & 2.54e+01 & 3.87e+01 & 9.41e+01 & 1.31e+02  \\
Ti & 47 & 1.10e+00 & 1.11e+00 & 1.11e+00 & 1.06e+00 & 9.63e-01 & 5.31e-01 & 7.65e-01 & 1.37e+00 & 1.93e+00 & 2.24e+00 & 2.66e+00 & 4.03e+00 & 5.87e+00  \\
Ti & 48 & 2.15e+02 & 2.15e+02 & 2.15e+02 & 2.15e+02 & 2.15e+02 & 2.12e+02 & 2.10e+02 & 2.03e+02 & 1.93e+02 & 1.85e+02 & 1.76e+02 & 1.38e+02 & 9.77e+01  \\
Ti & 49 & 1.66e+01 & 1.66e+01 & 1.67e+01 & 1.75e+01 & 3.03e+01 & 6.10e+01 & 6.80e+01 & 8.75e+01 & 1.13e+02 & 1.28e+02 & 1.45e+02 & 1.82e+02 & 1.97e+02  \\
Ti & 50 & 2.35e-13 & 2.35e-13 & 2.38e-13 & 2.66e-13 & 7.41e-13 & 1.24e-07 & 1.99e-06 & 5.20e-05 & 4.53e-04 & 1.07e-03 & 2.11e-03 & 6.03e-03 & 3.74e-02  \\
V  & 50 & 1.57e-07 & 1.57e-07 & 1.60e-07 & 1.71e-07 & 3.92e-07 & 1.51e-03 & 9.55e-03 & 1.19e-01 & 7.39e-01 & 1.47e+00 & 2.38e+00 & 7.72e+00 & 4.64e+01  \\
V  & 51 & 2.35e+01 & 2.36e+01 & 2.36e+01 & 2.31e+01 & 1.83e+01 & 3.17e+01 & 5.14e+01 & 9.49e+01 & 1.46e+02 & 1.78e+02 & 2.18e+02 & 3.43e+02 & 5.19e+02  \\
Cr & 50 & 2.92e+00 & 2.95e+00 & 3.00e+00 & 2.88e+00 & 3.13e+00 & 9.22e+00 & 2.15e+01 & 6.47e+01 & 1.45e+02 & 2.13e+02 & 3.21e+02 & 9.18e+02 & 1.73e+03  \\
Cr & 52 & 7.69e+02 & 7.69e+02 & 7.69e+02 & 7.70e+02 & 7.68e+02 & 7.59e+02 & 7.50e+02 & 7.27e+02 & 6.95e+02 & 6.72e+02 & 6.43e+02 & 5.44e+02 & 5.17e+02  \\
Cr & 53 & 1.19e+02 & 1.19e+02 & 1.19e+02 & 1.22e+02 & 1.48e+02 & 1.89e+02 & 2.10e+02 & 2.71e+02 & 3.51e+02 & 4.01e+02 & 4.61e+02 & 6.59e+02 & 9.21e+02  \\
Cr & 54 & 9.15e-09 & 9.18e-09 & 9.47e-09 & 1.02e-08 & 4.59e-08 & 9.17e-05 & 4.74e-04 & 3.97e-03 & 1.81e-02 & 3.77e-02 & 8.36e-02 & 8.76e-01 & 6.41e+00  \\
Mn & 55 & 1.04e+01 & 1.04e+01 & 1.04e+01 & 1.04e+01 & 1.15e+01 & 5.80e+01 & 9.13e+01 & 1.63e+02 & 2.49e+02 & 3.02e+02 & 3.70e+02 & 6.06e+02 & 8.91e+02  \\
Fe & 54 & 5.86e-01 & 5.87e-01 & 5.93e-01 & 6.02e-01 & 7.65e-01 & 1.07e+01 & 2.40e+01 & 6.64e+01 & 1.40e+02 & 2.00e+02 & 2.91e+02 & 7.27e+02 & 1.35e+03  \\
Fe & 56 & 4.49e+02 & 4.49e+02 & 4.49e+02 & 4.49e+02 & 4.49e+02 & 4.47e+02 & 4.46e+02 & 4.41e+02 & 4.33e+02 & 4.28e+02 & 4.19e+02 & 3.81e+02 & 3.24e+02  \\
Fe & 57 & 1.56e+02 & 1.56e+02 & 1.55e+02 & 1.57e+02 & 1.59e+02 & 1.87e+02 & 2.07e+02 & 2.33e+02 & 2.73e+02 & 3.02e+02 & 3.40e+02 & 4.81e+02 & 6.16e+02  \\
Fe & 58 & 7.20e-09 & 7.22e-09 & 7.29e-09 & 7.86e-09 & 2.59e-08 & 4.90e-06 & 2.07e-05 & 1.47e-04 & 6.21e-04 & 1.26e-03 & 2.67e-03 & 2.10e-02 & 9.70e-02  \\
Co & 59 & 6.40e+01 & 6.43e+01 & 6.49e+01 & 6.26e+01 & 5.81e+01 & 1.75e+01 & 1.83e+01 & 3.49e+01 & 5.07e+01 & 5.99e+01 & 7.07e+01 & 9.89e+01 & 1.07e+02  \\
Ni & 58 & 1.40e+01 & 1.40e+01 & 1.42e+01 & 1.38e+01 & 1.37e+01 & 9.50e+00 & 1.28e+01 & 5.65e+01 & 1.31e+02 & 1.92e+02 & 2.84e+02 & 7.67e+02 & 1.61e+03  \\
Ni & 60 & 2.94e+02 & 2.93e+02 & 2.94e+02 & 2.94e+02 & 2.95e+02 & 2.99e+02 & 2.99e+02 & 2.81e+02 & 2.63e+02 & 2.51e+02 & 2.36e+02 & 1.70e+02 & 9.16e+01  \\
Ni & 61 & 9.87e+01 & 9.83e+01 & 9.81e+01 & 9.91e+01 & 1.01e+02 & 1.22e+02 & 1.37e+02 & 1.45e+02 & 1.58e+02 & 1.66e+02 & 1.77e+02 & 1.95e+02 & 1.64e+02  \\
Ni & 62 & 1.54e+01 & 1.55e+01 & 1.40e+01 & 1.56e+01 & 1.53e+01 & 4.79e+01 & 8.64e+01 & 1.59e+02 & 2.75e+02 & 3.64e+02 & 4.92e+02 & 9.76e+02 & 1.24e+03  \\
Ni & 64 & 4.81e-17 & 4.77e-17 & 4.86e-17 & 4.85e-17 & 5.14e-17 & 1.07e-13 & 2.20e-12 & 2.96e-11 & 3.36e-11 & 3.62e-11 & 4.40e-11 & 3.32e-10 & 6.04e-09  \\
Cu & 63 & 9.72e+00 & 9.73e+00 & 9.33e+00 & 9.76e+00 & 9.87e+00 & 1.30e+01 & 1.34e+00 & 5.96e-01 & 6.19e-01 & 7.16e-01 & 9.39e-01 & 2.47e+00 & 4.55e+00  \\
Cu & 65 & 2.73e+00 & 2.71e+00 & 2.75e+00 & 2.74e+00 & 2.80e+00 & 2.71e+00 & 2.48e+00 & 2.60e+00 & 2.99e+00 & 3.24e+00 & 3.60e+00 & 3.77e+00 & 2.07e+00  \\
Zn & 64 & 1.72e+02 & 1.71e+02 & 1.76e+02 & 1.72e+02 & 1.76e+02 & 1.05e+02 & 4.14e+01 & 2.10e+01 & 1.52e+01 & 1.32e+01 & 1.15e+01 & 6.43e+00 & 2.37e+00  \\
Zn & 66 & 4.60e+00 & 4.55e+00 & 4.56e+00 & 4.64e+00 & 4.80e+00 & 6.59e+00 & 8.26e+00 & 1.33e+01 & 2.16e+01 & 2.76e+01 & 3.61e+01 & 5.90e+01 & 5.04e+01  \\
Zn & 67 & 2.92e-01 & 2.90e-01 & 2.99e-01 & 2.91e-01 & 2.94e-01 & 1.37e-01 & 1.16e-02 & 2.28e-02 & 5.37e-02 & 8.05e-02 & 1.24e-01 & 2.95e-01 & 3.32e-01  \\
Zn & 68 & 1.55e+00 & 1.56e+00 & 1.59e+00 & 1.51e+00 & 1.44e+00 & 3.82e-01 & 1.07e-01 & 4.59e-02 & 3.14e-02 & 2.69e-02 & 2.40e-02 & 2.64e-02 & 6.53e-02  \\
Zn & 70 & 1.14e-22 & 1.14e-22 & 1.14e-22 & 1.19e-22 & 1.97e-22 & 4.45e-19 & 9.13e-18 & 2.00e-16 & 1.57e-15 & 4.55e-15 & 7.58e-15 & 7.46e-17 & 4.20e-18  \\
Ga & 69 & 7.39e-02 & 7.38e-02 & 7.48e-02 & 7.33e-02 & 7.28e-02 & 5.85e-02 & 5.65e-02 & 5.53e-02 & 5.59e-02 & 5.53e-02 & 5.56e-02 & 4.18e-02 & 2.21e-02  \\
Ga & 71 & 2.43e-04 & 2.42e-04 & 2.50e-04 & 2.41e-04 & 2.41e-04 & 2.02e-04 & 5.22e-04 & 1.63e-03 & 3.47e-03 & 4.80e-03 & 6.91e-03 & 1.07e-02 & 6.22e-03  \\
Ge & 70 & 2.76e-01 & 2.73e-01 & 2.76e-01 & 2.77e-01 & 2.84e-01 & 3.42e-01 & 4.10e-01 & 6.17e-01 & 9.66e-01 & 1.21e+00 & 1.56e+00 & 2.35e+00 & 1.69e+00  \\
Ge & 72 & 6.08e-03 & 6.18e-03 & 6.27e-03 & 5.88e-03 & 5.48e-03 & 1.04e-03 & 1.76e-04 & 9.75e-05 & 2.17e-04 & 4.04e-04 & 8.54e-04 & 5.43e-03 & 1.11e-02  \\
Ge & 73 & 8.00e-04 & 7.96e-04 & 8.07e-04 & 7.97e-04 & 8.07e-04 & 7.68e-04 & 5.73e-04 & 3.65e-04 & 3.19e-04 & 2.95e-04 & 2.85e-04 & 1.79e-04 & 8.14e-05  \\
Ge & 74 & 5.78e-20 & 5.78e-20 & 5.77e-20 & 6.44e-20 & 1.72e-19 & 2.06e-17 & 1.06e-16 & 1.55e-15 & 1.45e-14 & 2.73e-14 & 2.21e-14 & 1.33e-17 & 1.21e-19  \\
Ge & 76 & 9.89e-27 & 9.72e-27 & 9.06e-27 & 1.02e-26 & 1.03e-26 & 9.87e-27 & 9.58e-22 & 3.63e-20 & 3.23e-18 & 1.35e-17 & 1.93e-17 & 2.86e-20 & 1.76e-23  \\
As & 75 & 2.95e-05 & 2.94e-05 & 3.06e-05 & 2.91e-05 & 2.92e-05 & 1.45e-05 & 2.07e-05 & 5.09e-05 & 8.97e-05 & 1.18e-04 & 1.64e-04 & 2.79e-04 & 1.82e-04  \\ \hline
\end{tabular}%
}


==> Chapters/townsley_table_production_factors.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
  Element & A & $^{22}$Ne = 0  & 1e-7 & 1e-6 & 1e-5 & 1e-4 & 1e-3 & 2e-3 & 5e-3 & 1e-2 & 1.4e-2 & 2e-2 & 5e-2 & 1e-1 \\ 
\hline
C  & 12 & 6.55e-01 & 6.55e-01 & 6.55e-01 & 6.55e-01 & 6.55e-01 & 6.53e-01 & 6.51e-01 & 6.47e-01 & 6.42e-01 & 6.39e-01 & 6.35e-01 & 6.21e-01 & 6.01e-01  \\
C  & 13 & 2.12e-05 & 2.12e-05 & 2.11e-05 & 2.09e-05 & 2.04e-05 & 2.89e-05 & 4.80e-05 & 1.34e-04 & 2.92e-04 & 4.28e-04 & 6.49e-04 & 2.05e-03 & 5.31e-03  \\
N  & 14 & 3.44e-05 & 3.44e-05 & 3.44e-05 & 3.42e-05 & 3.88e-05 & 1.90e-04 & 3.83e-04 & 9.01e-04 & 1.63e-03 & 2.14e-03 & 2.81e-03 & 5.29e-03 & 7.69e-03  \\
N  & 15 & 5.94e-01 & 5.94e-01 & 5.92e-01 & 5.74e-01 & 3.98e-01 & 2.97e-02 & 1.13e-02 & 3.60e-03 & 2.22e-03 & 2.02e-03 & 2.07e-03 & 4.02e-03 & 1.44e-02  \\
O  & 16 & 8.84e+00 & 8.84e+00 & 8.84e+00 & 8.85e+00 & 8.86e+00 & 8.94e+00 & 9.02e+00 & 9.21e+00 & 9.43e+00 & 9.54e+00 & 9.67e+00 & 9.80e+00 & 9.35e+00  \\
O  & 17 & 2.36e-04 & 2.36e-04 & 2.38e-04 & 2.58e-04 & 5.23e-04 & 1.08e-02 & 2.66e-02 & 6.61e-02 & 1.08e-01 & 1.31e-01 & 1.56e-01 & 1.99e-01 & 1.98e-01  \\
O  & 18 & 4.19e-07 & 4.19e-07 & 4.21e-07 & 4.43e-07 & 7.37e-07 & 1.22e-05 & 3.03e-05 & 8.16e-05 & 1.60e-04 & 2.19e-04 & 3.07e-04 & 8.38e-04 & 3.02e-03  \\
F  & 19 & 1.70e-03 & 1.70e-03 & 1.69e-03 & 1.62e-03 & 1.19e-03 & 3.59e-04 & 2.47e-04 & 2.67e-04 & 4.52e-04 & 6.34e-04 & 9.34e-04 & 2.49e-03 & 4.18e-03  \\
Ne & 20 & 1.31e+00 & 1.31e+00 & 1.31e+00 & 1.31e+00 & 1.31e+00 & 1.30e+00 & 1.29e+00 & 1.27e+00 & 1.23e+00 & 1.20e+00 & 1.15e+00 & 9.96e-01 & 8.55e-01  \\
Ne & 21 & 3.50e-03 & 3.50e-03 & 3.50e-03 & 3.55e-03 & 4.13e-03 & 2.13e-02 & 5.44e-02 & 1.74e-01 & 3.87e-01 & 5.75e-01 & 8.85e-01 & 2.94e+00 & 8.38e+00  \\
Ne & 22 & 1.99e-04 & 1.99e-04 & 2.01e-04 & 2.23e-04 & 4.83e-04 & 3.71e-03 & 8.01e-03 & 2.42e-02 & 5.94e-02 & 9.34e-02 & 1.53e-01 & 5.73e-01 & 1.72e+00  \\
Na & 23 & 2.14e-01 & 2.14e-01 & 2.14e-01 & 2.13e-01 & 2.09e-01 & 1.92e-01 & 1.94e-01 & 2.17e-01 & 2.82e-01 & 3.45e-01 & 4.49e-01 & 1.16e+00 & 3.36e+00  \\
Mg & 24 & 2.54e+01 & 2.54e+01 & 2.54e+01 & 2.54e+01 & 2.55e+01 & 2.46e+01 & 2.32e+01 & 1.98e+01 & 1.58e+01 & 1.35e+01 & 1.11e+01 & 6.26e+00 & 6.04e+00  \\
Mg & 25 & 2.33e-03 & 2.33e-03 & 2.34e-03 & 2.37e-03 & 2.90e-03 & 3.61e-02 & 5.86e-02 & 1.34e-01 & 2.84e-01 & 4.25e-01 & 6.67e-01 & 2.47e+00 & 8.92e+00  \\
Mg & 26 & 9.78e-03 & 9.78e-03 & 9.79e-03 & 9.90e-03 & 1.12e-02 & 2.75e-02 & 4.50e-02 & 9.65e-02 & 1.81e-01 & 2.49e-01 & 3.56e-01 & 1.08e+00 & 5.70e+00  \\
Al & 27 & 6.69e-01 & 6.69e-01 & 6.69e-01 & 6.67e-01 & 6.57e-01 & 1.51e+00 & 2.72e+00 & 5.07e+00 & 7.13e+00 & 8.03e+00 & 8.78e+00 & 1.02e+01 & 1.53e+01  \\
Si & 28 & 2.54e+02 & 2.54e+02 & 2.54e+02 & 2.54e+02 & 2.55e+02 & 2.58e+02 & 2.60e+02 & 2.61e+02 & 2.61e+02 & 2.60e+02 & 2.59e+02 & 2.53e+02 & 2.41e+02  \\
Si & 29 & 8.34e-01 & 8.34e-01 & 8.34e-01 & 8.31e-01 & 8.66e-01 & 2.99e+00 & 3.91e+00 & 5.83e+00 & 8.29e+00 & 1.02e+01 & 1.32e+01 & 3.96e+01 & 1.46e+02  \\
Si & 30 & 6.98e-01 & 6.97e-01 & 6.94e-01 & 6.63e-01 & 4.45e-01 & 6.31e-01 & 2.15e+00 & 8.91e+00 & 2.22e+01 & 3.30e+01 & 4.92e+01 & 1.35e+02 & 2.89e+02  \\
P  & 31 & 7.11e+00 & 7.11e+00 & 7.09e+00 & 6.91e+00 & 5.30e+00 & 4.06e+00 & 6.24e+00 & 1.28e+01 & 2.27e+01 & 2.98e+01 & 3.94e+01 & 7.60e+01 & 8.70e+01  \\
S  & 32 & 3.03e+02 & 3.03e+02 & 3.02e+02 & 3.02e+02 & 3.02e+02 & 2.99e+02 & 2.98e+02 & 2.96e+02 & 2.94e+02 & 2.92e+02 & 2.88e+02 & 2.60e+02 & 2.07e+02  \\
S  & 33 & 1.30e+01 & 1.30e+01 & 1.30e+01 & 1.31e+01 & 1.38e+01 & 1.38e+01 & 1.53e+01 & 2.32e+01 & 3.42e+01 & 4.11e+01 & 4.94e+01 & 7.07e+01 & 7.42e+01  \\
S  & 34 & 1.88e-01 & 1.88e-01 & 1.87e-01 & 1.77e-01 & 1.05e-01 & 1.20e+00 & 3.70e+00 & 1.21e+01 & 2.80e+01 & 4.19e+01 & 6.42e+01 & 1.74e+02 & 2.89e+02  \\
S  & 36 & 5.32e-05 & 5.32e-05 & 5.32e-05 & 5.32e-05 & 5.33e-05 & 6.43e-04 & 4.58e-03 & 4.34e-02 & 2.06e-01 & 4.35e-01 & 1.01e+00 & 1.57e+01 & 1.45e+02  \\
Cl & 35 & 1.10e+00 & 1.10e+00 & 1.09e+00 & 1.06e+00 & 8.20e-01 & 7.03e-01 & 9.89e-01 & 2.00e+00 & 3.67e+00 & 5.01e+00 & 6.89e+00 & 1.20e+01 & 1.24e+01  \\
Cl & 37 & 8.48e-01 & 8.48e-01 & 8.49e-01 & 8.51e-01 & 8.77e-01 & 9.76e-01 & 1.17e+00 & 1.76e+00 & 2.59e+00 & 3.15e+00 & 3.89e+00 & 7.08e+00 & 9.53e+00  \\
Ar & 36 & 3.55e+02 & 3.55e+02 & 3.55e+02 & 3.55e+02 & 3.54e+02 & 3.46e+02 & 3.43e+02 & 3.36e+02 & 3.29e+02 & 3.23e+02 & 3.14e+02 & 2.69e+02 & 2.07e+02  \\
Ar & 38 & 2.15e-01 & 2.15e-01 & 2.12e-01 & 2.14e-01 & 1.97e-01 & 7.09e-01 & 1.69e+00 & 5.44e+00 & 1.29e+01 & 1.96e+01 & 3.04e+01 & 8.77e+01 & 1.60e+02  \\
Ar & 40 & 5.04e-05 & 5.04e-05 & 5.04e-05 & 5.04e-05 & 5.05e-05 & 6.78e-05 & 1.58e-04 & 9.86e-04 & 5.13e-03 & 1.29e-02 & 3.83e-02 & 7.90e-01 & 3.86e+00  \\
K  & 39 & 9.18e-01 & 9.18e-01 & 9.12e-01 & 9.12e-01 & 8.52e-01 & 1.07e+00 & 1.63e+00 & 3.62e+00 & 5.71e+00 & 7.09e+00 & 8.88e+00 & 1.58e+01 & 1.80e+01  \\
K  & 40 & 3.21e-04 & 3.20e-04 & 3.21e-04 & 3.24e-04 & 3.87e-04 & 2.20e-02 & 5.36e-02 & 1.95e-01 & 6.57e-01 & 1.26e+00 & 2.47e+00 & 6.23e+00 & 2.92e+00  \\
K  & 41 & 4.89e-01 & 4.89e-01 & 4.91e-01 & 5.10e-01 & 6.92e-01 & 1.38e+00 & 1.88e+00 & 3.14e+00 & 4.87e+00 & 6.00e+00 & 7.42e+00 & 1.23e+01 & 1.30e+01  \\
Ca & 40 & 3.44e+02 & 3.44e+02 & 3.44e+02 & 3.44e+02 & 3.42e+02 & 3.35e+02 & 3.30e+02 & 3.22e+02 & 3.13e+02 & 3.06e+02 & 2.96e+02 & 2.52e+02 & 1.96e+02  \\
Ca & 42 & 5.96e-02 & 5.95e-02 & 5.95e-02 & 5.95e-02 & 5.89e-02 & 3.30e-01 & 8.68e-01 & 3.33e+00 & 8.14e+00 & 1.23e+01 & 1.89e+01 & 5.05e+01 & 7.42e+01  \\
Ca & 43 & 2.77e+00 & 2.77e+00 & 2.76e+00 & 2.76e+00 & 2.65e+00 & 2.86e+00 & 4.57e+00 & 1.16e+01 & 1.39e+01 & 1.41e+01 & 1.37e+01 & 1.06e+01 & 6.62e+00  \\
Ca & 44 & 2.63e+01 & 2.63e+01 & 2.63e+01 & 2.63e+01 & 2.63e+01 & 2.68e+01 & 2.69e+01 & 2.64e+01 & 2.52e+01 & 2.44e+01 & 2.32e+01 & 1.81e+01 & 1.22e+01  \\
Ca & 46 & 1.35e-02 & 1.35e-02 & 1.35e-02 & 1.35e-02 & 1.35e-02 & 1.35e-02 & 1.36e-02 & 1.36e-02 & 1.39e-02 & 1.42e-02 & 1.53e-02 & 4.43e-02 & 1.62e-01  \\
Ca & 48 & 1.05e-05 & 1.05e-05 & 1.05e-05 & 1.05e-05 & 1.05e-05 & 1.06e-05 & 1.06e-05 & 1.07e-05 & 1.08e-05 & 1.10e-05 & 1.12e-05 & 1.26e-05 & 4.55e-05  \\
SC & 45 & 2.79e-01 & 2.79e-01 & 2.80e-01 & 2.92e-01 & 4.16e-01 & 9.32e-01 & 1.06e+00 & 1.41e+00 & 1.94e+00 & 2.29e+00 & 2.73e+00 & 3.90e+00 & 4.26e+00  \\
Ti & 46 & 4.02e+00 & 4.02e+00 & 3.99e+00 & 4.02e+00 & 3.70e+00 & 1.64e+00 & 1.10e+00 & 3.02e+00 & 7.49e+00 & 1.14e+01 & 1.76e+01 & 4.97e+01 & 8.40e+01  \\
Ti & 47 & 6.02e+00 & 6.02e+00 & 5.96e+00 & 6.02e+00 & 5.58e+00 & 2.84e+00 & 2.16e+00 & 3.95e+00 & 5.31e+00 & 5.86e+00 & 6.31e+00 & 6.80e+00 & 6.80e+00  \\
Ti & 48 & 2.65e+02 & 2.64e+02 & 2.64e+02 & 2.65e+02 & 2.65e+02 & 2.65e+02 & 2.65e+02 & 2.58e+02 & 2.46e+02 & 2.37e+02 & 2.25e+02 & 1.78e+02 & 1.25e+02  \\
Ti & 49 & 2.70e+01 & 2.70e+01 & 2.70e+01 & 2.78e+01 & 3.96e+01 & 7.76e+01 & 8.59e+01 & 1.09e+02 & 1.39e+02 & 1.58e+02 & 1.78e+02 & 2.25e+02 & 2.42e+02  \\
Ti & 50 & 6.22e+01 & 6.22e+01 & 6.22e+01 & 6.22e+01 & 6.22e+01 & 6.23e+01 & 6.24e+01 & 6.27e+01 & 6.33e+01 & 6.37e+01 & 6.44e+01 & 6.79e+01 & 7.47e+01  \\
V  & 50 & 1.24e+01 & 1.24e+01 & 1.24e+01 & 1.24e+01 & 1.24e+01 & 1.24e+01 & 1.24e+01 & 1.25e+01 & 1.28e+01 & 1.31e+01 & 1.36e+01 & 1.74e+01 & 4.74e+01  \\
V  & 51 & 1.03e+02 & 1.03e+02 & 1.03e+02 & 1.03e+02 & 9.75e+01 & 9.86e+01 & 1.13e+02 & 1.63e+02 & 2.23e+02 & 2.61e+02 & 3.07e+02 & 4.52e+02 & 6.28e+02  \\
Cr & 50 & 7.39e+01 & 7.39e+01 & 7.38e+01 & 7.40e+01 & 7.37e+01 & 7.52e+01 & 8.36e+01 & 1.25e+02 & 2.01e+02 & 2.66e+02 & 3.68e+02 & 9.25e+02 & 1.74e+03  \\
Cr & 52 & 1.03e+03 & 1.03e+03 & 1.03e+03 & 1.03e+03 & 1.03e+03 & 1.02e+03 & 1.01e+03 & 9.82e+02 & 9.45e+02 & 9.20e+02 & 8.87e+02 & 7.69e+02 & 6.95e+02  \\
Cr & 53 & 2.98e+02 & 2.98e+02 & 2.98e+02 & 3.01e+02 & 3.25e+02 & 3.85e+02 & 4.09e+02 & 4.78e+02 & 5.72e+02 & 6.32e+02 & 7.04e+02 & 9.35e+02 & 1.20e+03  \\
Cr & 54 & 4.14e+02 & 4.14e+02 & 4.14e+02 & 4.14e+02 & 4.14e+02 & 4.15e+02 & 4.15e+02 & 4.17e+02 & 4.20e+02 & 4.22e+02 & 4.26e+02 & 4.46e+02 & 4.88e+02  \\
Mn & 55 & 3.24e+02 & 3.24e+02 & 3.24e+02 & 3.24e+02 & 3.25e+02 & 3.72e+02 & 4.11e+02 & 4.94e+02 & 5.95e+02 & 6.61e+02 & 7.47e+02 & 1.07e+03 & 1.47e+03  \\
Fe & 54 & 4.49e+02 & 4.49e+02 & 4.49e+02 & 4.49e+02 & 4.49e+02 & 4.60e+02 & 4.74e+02 & 5.20e+02 & 6.00e+02 & 6.66e+02 & 7.66e+02 & 1.27e+03 & 2.07e+03  \\
Fe & 56 & 6.83e+02 & 6.83e+02 & 6.83e+02 & 6.83e+02 & 6.82e+02 & 6.80e+02 & 6.78e+02 & 6.72e+02 & 6.62e+02 & 6.54e+02 & 6.42e+02 & 5.86e+02 & 4.98e+02  \\
Fe & 57 & 4.43e+02 & 4.43e+02 & 4.43e+02 & 4.43e+02 & 4.47e+02 & 4.82e+02 & 5.14e+02 & 5.56e+02 & 6.11e+02 & 6.50e+02 & 7.04e+02 & 9.02e+02 & 1.08e+03  \\
Fe & 58 & 2.36e+02 & 2.36e+02 & 2.36e+02 & 2.36e+02 & 2.37e+02 & 2.37e+02 & 2.37e+02 & 2.38e+02 & 2.40e+02 & 2.41e+02 & 2.43e+02 & 2.53e+02 & 2.71e+02  \\
Co & 59 & 2.01e+02 & 2.01e+02 & 2.01e+02 & 2.01e+02 & 1.94e+02 & 1.36e+02 & 1.15e+02 & 1.44e+02 & 1.71e+02 & 1.86e+02 & 2.03e+02 & 2.52e+02 & 2.82e+02  \\
Ni & 58 & 6.64e+02 & 6.64e+02 & 6.64e+02 & 6.64e+02 & 6.65e+02 & 6.66e+02 & 6.71e+02 & 7.34e+02 & 8.55e+02 & 9.52e+02 & 1.10e+03 & 1.84e+03 & 3.08e+03  \\
Ni & 60 & 7.26e+02 & 7.26e+02 & 7.25e+02 & 7.26e+02 & 7.26e+02 & 7.28e+02 & 7.31e+02 & 7.09e+02 & 6.79e+02 & 6.59e+02 & 6.33e+02 & 5.33e+02 & 4.21e+02  \\
Ni & 61 & 2.30e+02 & 2.30e+02 & 2.30e+02 & 2.30e+02 & 2.33e+02 & 2.65e+02 & 2.98e+02 & 3.26e+02 & 3.49e+02 & 3.65e+02 & 3.85e+02 & 4.39e+02 & 4.34e+02  \\
Ni & 62 & 3.02e+02 & 3.02e+02 & 3.02e+02 & 3.02e+02 & 3.03e+02 & 3.28e+02 & 3.93e+02 & 5.45e+02 & 7.52e+02 & 9.11e+02 & 1.14e+03 & 2.13e+03 & 3.21e+03  \\
Ni & 64 & 1.16e+00 & 1.16e+00 & 1.16e+00 & 1.16e+00 & 1.16e+00 & 1.17e+00 & 1.17e+00 & 1.17e+00 & 1.18e+00 & 1.19e+00 & 1.20e+00 & 1.26e+00 & 1.37e+00  \\
Cu & 63 & 1.57e+01 & 1.57e+01 & 1.57e+01 & 1.57e+01 & 1.56e+01 & 1.93e+01 & 1.70e+01 & 3.53e+00 & 3.44e+00 & 3.58e+00 & 3.93e+00 & 7.45e+00 & 1.52e+01  \\
Cu & 65 & 6.11e+00 & 6.11e+00 & 6.10e+00 & 6.13e+00 & 6.22e+00 & 6.96e+00 & 6.99e+00 & 7.13e+00 & 8.24e+00 & 9.16e+00 & 1.04e+01 & 1.37e+01 & 1.24e+01  \\
Zn & 64 & 3.13e+02 & 3.13e+02 & 3.12e+02 & 3.14e+02 & 3.16e+02 & 3.00e+02 & 1.78e+02 & 5.93e+01 & 4.05e+01 & 3.55e+01 & 3.11e+01 & 2.06e+01 & 1.20e+01  \\
Zn & 66 & 1.30e+01 & 1.30e+01 & 1.30e+01 & 1.30e+01 & 1.35e+01 & 1.79e+01 & 2.25e+01 & 3.43e+01 & 5.38e+01 & 6.91e+01 & 9.06e+01 & 1.73e+02 & 2.33e+02  \\
Zn & 67 & 6.59e-01 & 6.58e-01 & 6.57e-01 & 6.61e-01 & 6.66e-01 & 5.97e-01 & 2.79e-01 & 8.68e-02 & 1.79e-01 & 2.69e-01 & 4.18e-01 & 1.22e+00 & 2.21e+00  \\
Zn & 68 & 6.33e+00 & 6.32e+00 & 6.28e+00 & 6.33e+00 & 6.04e+00 & 3.11e+00 & 9.89e-01 & 1.99e-01 & 1.27e-01 & 1.11e-01 & 9.97e-02 & 1.03e-01 & 2.52e-01  \\
Zn & 70 & 7.06e-06 & 7.06e-06 & 7.06e-06 & 7.06e-06 & 7.06e-06 & 7.07e-06 & 7.08e-06 & 7.12e-06 & 7.19e-06 & 7.24e-06 & 7.30e-06 & 7.75e-06 & 8.59e-06  \\
Ga & 69 & 2.64e-01 & 2.63e-01 & 2.62e-01 & 2.64e-01 & 2.59e-01 & 2.21e-01 & 2.02e-01 & 2.14e-01 & 2.34e-01 & 2.49e-01 & 2.63e-01 & 2.66e-01 & 2.16e-01  \\
Ga & 71 & 2.11e-03 & 2.10e-03 & 2.10e-03 & 2.11e-03 & 2.15e-03 & 2.21e-03 & 2.70e-03 & 1.09e-02 & 2.71e-02 & 4.16e-02 & 6.39e-02 & 1.59e-01 & 2.24e-01  \\
Ge & 70 & 1.02e+00 & 1.02e+00 & 1.02e+00 & 1.03e+00 & 1.04e+00 & 1.24e+00 & 1.45e+00 & 2.10e+00 & 3.23e+00 & 4.13e+00 & 5.40e+00 & 1.04e+01 & 1.40e+01  \\
Ge & 72 & 4.60e-02 & 4.59e-02 & 4.54e-02 & 4.59e-02 & 4.27e-02 & 1.80e-02 & 4.65e-03 & 9.42e-04 & 1.21e-03 & 1.77e-03 & 3.15e-03 & 2.14e-02 & 8.99e-02  \\
Ge & 73 & 4.27e-03 & 4.27e-03 & 4.24e-03 & 4.28e-03 & 4.26e-03 & 4.40e-03 & 4.92e-03 & 4.11e-03 & 3.83e-03 & 3.92e-03 & 3.97e-03 & 3.47e-03 & 2.43e-03  \\
Ge & 74 & 1.10e-07 & 1.10e-07 & 1.10e-07 & 1.10e-07 & 1.10e-07 & 1.10e-07 & 1.10e-07 & 1.11e-07 & 1.12e-07 & 1.12e-07 & 1.13e-07 & 1.21e-07 & 1.32e-07  \\
Ge & 76 & 1.19e-10 & 1.19e-10 & 1.19e-10 & 1.19e-10 & 1.20e-10 & 1.20e-10 & 1.20e-10 & 1.21e-10 & 1.22e-10 & 1.23e-10 & 1.25e-10 & 1.35e-10 & 1.54e-10  \\ 
As & 75 & 1.96e-04 & 1.95e-04 & 1.94e-04 & 1.96e-04 & 1.94e-04 & 1.59e-04 & 1.15e-04 & 2.74e-04 & 5.37e-04 & 7.52e-04 & 1.09e-03 & 2.73e-03 & 4.37e-03  \\ \hline
\end{tabular}%
}


==> decayed_brox_yields_new_latex_table.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
  Element & Z & A & $^{22}$Ne = 0  & 1e-7 & 1e-6 & 1e-5 & 1e-4 & 1e-3 & 2e-3 & 5e-3 & 1e-2 & 1.4e-2 & 2e-2 & 5e-2 & 1e-1 \\
\hline


O  & 8  & 16   & 0.1785    & 0.1785    & 0.1785    & 0.1786    & 0.1790    & 0.1805    & 0.1819    & 0.1865    & 0.1920    & 0.1948    & 0.1977    & 0.2004    & 0.1912    \\
O  & 8  & 17   & 1.87E-09  & 1.87E-09  & 1.88E-09  & 2.01E-09  & 3.81E-09  & 7.45E-08  & 1.74E-07  & 4.16E-07  & 6.86E-07  & 8.36E-07  & 1.00E-06  & 1.32E-06  & 1.31E-06  \\
O  & 8  & 18   & 1.82E-11  & 1.82E-11  & 1.83E-11  & 1.92E-11  & 3.23E-11  & 4.94E-10  & 1.13E-09  & 2.94E-09  & 5.93E-09  & 8.37E-09  & 1.22E-08  & 3.79E-08  & 1.46E-07  \\
F  & 9  & 19   & 2.63E-09  & 2.63E-09  & 2.61E-09  & 2.49E-09  & 1.77E-09  & 5.07E-10  & 3.53E-10  & 4.22E-10  & 8.10E-10  & 1.18E-09  & 1.78E-09  & 5.03E-09  & 8.28E-09  \\
Ne & 10 & 20   & 0.0064    & 0.0064    & 0.0064    & 0.0064    & 0.0064    & 0.0063    & 0.0063    & 0.0061    & 0.0059    & 0.0058    & 0.0055    & 0.0048    & 0.0041    \\
Ne & 10 & 21   & 3.63E-08  & 3.63E-08  & 3.64E-08  & 3.70E-08  & 4.39E-08  & 2.18E-07  & 5.46E-07  & 1.78E-06  & 4.21E-06  & 6.38E-06  & 1.00E-05  & 3.53E-05  & 0.0001    \\
Ne & 10 & 22   & 6.82E-08  & 6.86E-08  & 7.13E-08  & 9.91E-08  & 3.80E-07  & 3.36E-06  & 6.90E-06  & 1.86E-05  & 4.06E-05  & 6.02E-05  & 9.24E-05  & 0.0002    & 0.0008    \\
Na & 11 & 23   & 2.72E-05  & 2.72E-05  & 2.72E-05  & 2.71E-05  & 2.66E-05  & 2.46E-05  & 2.47E-05  & 2.69E-05  & 3.39E-05  & 4.11E-05  & 5.35E-05  & 0.0001    & 0.0004    \\
Mg & 12 & 24   & 0.0378    & 0.0378    & 0.0378    & 0.0378    & 0.0378    & 0.0364    & 0.0342    & 0.0282    & 0.0215    & 0.0179    & 0.0143    & 0.0079    & 0.0075    \\
Mg & 12 & 25   & 5.16E-07  & 5.16E-07  & 5.17E-07  & 5.28E-07  & 6.80E-07  & 6.98E-06  & 1.26E-05  & 3.30E-05  & 7.65E-05  & 0.0001    & 0.0001    & 0.0007    & 0.0025    \\
Mg & 12 & 26   & 3.47E-06  & 3.47E-06  & 3.47E-06  & 3.51E-06  & 3.97E-06  & 9.35E-06  & 1.49E-05  & 3.06E-05  & 5.73E-05  & 8.02E-05  & 0.0001    & 0.0003    & 0.0015    \\
Al & 13 & 27   & 0.0001    & 0.0001    & 0.0001    & 0.0001    & 0.0001    & 0.0002    & 0.0004    & 0.0008    & 0.0011    & 0.0012    & 0.0013    & 0.0016    & 0.0024    \\
Si & 14 & 28   & 0.3036    & 0.3036    & 0.3037    & 0.3037    & 0.3046    & 0.3107    & 0.3143    & 0.3187    & 0.3206    & 0.3209    & 0.3205    & 0.3161    & 0.3052    \\
Si & 14 & 29   & 6.04E-05  & 6.04E-05  & 6.05E-05  & 6.11E-05  & 7.48E-05  & 0.0002    & 0.0003    & 0.0005    & 0.0007    & 0.0009    & 0.0012    & 0.0035    & 0.0135    \\
Si & 14 & 30   & 2.96E-05  & 2.96E-05  & 2.94E-05  & 2.84E-05  & 2.24E-05  & 4.34E-05  & 0.0001    & 0.0005    & 0.0013    & 0.0020    & 0.0030    & 0.0084    & 0.0198    \\
P  & 15 & 31   & 8.92E-05  & 8.91E-05  & 8.88E-05  & 8.57E-05  & 5.93E-05  & 6.00E-05  & 0.0001    & 0.0002    & 0.0004    & 0.0005    & 0.0007    & 0.0014    & 0.0016    \\
S  & 16 & 32   & 0.1561    & 0.1561    & 0.1561    & 0.1561    & 0.1554    & 0.1527    & 0.1518    & 0.1508    & 0.1498    & 0.1485    & 0.1461    & 0.1280    & 0.0952    \\
S  & 16 & 33   & 9.39E-05  & 9.39E-05  & 9.40E-05  & 9.47E-05  & 0.0001    & 0.0001    & 0.0001    & 0.0002    & 0.0002    & 0.0003    & 0.0004    & 0.0005    & 0.0005    \\
S  & 16 & 34   & 4.32E-06  & 4.32E-06  & 4.30E-06  & 4.07E-06  & 2.54E-06  & 7.79E-05  & 0.0002    & 0.0007    & 0.0016    & 0.0023    & 0.0035    & 0.0093    & 0.0146    \\
S  & 16 & 36   & 3.74E-14  & 3.74E-14  & 3.76E-14  & 3.91E-14  & 6.20E-14  & 1.50E-10  & 1.00E-09  & 8.64E-09  & 3.97E-08  & 8.58E-08  & 2.14E-07  & 3.87E-06  & 3.53E-05  \\
Cl & 17 & 35   & 1.03E-05  & 1.02E-05  & 1.02E-05  & 9.71E-06  & 6.19E-06  & 1.27E-05  & 2.14E-05  & 4.52E-05  & 8.64E-05  & 0.0001    & 0.0001    & 0.0002    & 0.0002    \\
Cl & 17 & 37   & 5.91E-06  & 5.92E-06  & 5.92E-06  & 5.98E-06  & 6.51E-06  & 7.39E-06  & 8.99E-06  & 1.37E-05  & 2.02E-05  & 2.46E-05  & 3.02E-05  & 4.81E-05  & 5.73E-05  \\
Ar & 18 & 36   & 0.0302    & 0.0302    & 0.0302    & 0.0302    & 0.0299    & 0.0285    & 0.0277    & 0.0263    & 0.0249    & 0.0240    & 0.0227    & 0.0172    & 0.0114    \\
Ar & 18 & 38   & 3.98E-07  & 3.97E-07  & 3.96E-07  & 3.87E-07  & 2.84E-07  & 3.69E-05  & 9.57E-05  & 0.0002    & 0.0006    & 0.0010    & 0.0016    & 0.0042    & 0.0069    \\
Ar & 18 & 40   & 6.21E-16  & 6.21E-16  & 6.23E-16  & 6.46E-16  & 9.46E-16  & 1.65E-12  & 9.21E-12  & 6.81E-11  & 3.47E-10  & 8.83E-10  & 2.72E-09  & 5.99E-08  & 3.21E-07  \\
K  & 19 & 39   & 1.33E-06  & 1.33E-06  & 1.33E-06  & 1.27E-06  & 1.03E-06  & 1.00E-05  & 1.73E-05  & 3.47E-05  & 5.97E-05  & 7.76E-05  & 0.0001    & 0.0001    & 0.0001    \\
K  & 19 & 40   & 1.53E-12  & 1.53E-12  & 1.54E-12  & 1.58E-12  & 2.30E-12  & 5.19E-10  & 1.13E-09  & 3.64E-09  & 1.20E-08  & 2.29E-08  & 4.48E-08  & 1.11E-07  & 4.28E-08  \\
K  & 19 & 41   & 3.73E-07  & 3.73E-07  & 3.75E-07  & 3.93E-07  & 5.68E-07  & 1.18E-06  & 1.58E-06  & 2.57E-06  & 3.88E-06  & 4.75E-06  & 5.82E-06  & 8.41E-06  & 7.34E-06  \\
Ca & 20 & 40   & 0.0271    & 0.0271    & 0.0270    & 0.0270    & 0.0267    & 0.0248    & 0.0236    & 0.0215    & 0.0195    & 0.0183    & 0.0169    & 0.0119    & 0.0075    \\
Ca & 20 & 42   & 4.74E-09  & 4.73E-09  & 4.70E-09  & 4.33E-09  & 6.84E-10  & 6.64E-07  & 1.89E-06  & 6.65E-06  & 1.70E-05  & 2.66E-05  & 4.21E-05  & 0.0001    & 0.0001    \\
Ca & 20 & 43   & 2.37E-08  & 2.37E-08  & 2.33E-08  & 1.94E-08  & 1.66E-10  & 7.06E-10  & 1.98E-09  & 8.61E-09  & 2.68E-08  & 4.52E-08  & 7.44E-08  & 1.75E-07  & 2.35E-07  \\
Ca & 20 & 44   & 1.24E-05  & 1.24E-05  & 1.24E-05  & 1.24E-05  & 1.22E-05  & 1.10E-05  & 1.03E-05  & 9.08E-06  & 8.01E-06  & 7.42E-06  & 6.75E-06  & 4.71E-06  & 3.14E-06  \\
Ca & 20 & 46   & 2.39E-21  & 2.40E-21  & 2.43E-21  & 2.75E-21  & 9.64E-21  & 1.81E-16  & 2.97E-15  & 9.00E-14  & 1.15E-12  & 4.30E-12  & 1.82E-11  & 4.47E-10  & 2.55E-09  \\
Ca & 20 & 48   & 4.90E-27  & 4.94E-27  & 5.30E-27  & 8.82E-27  & 3.06E-26  & 3.55E-23  & 1.97E-21  & 2.08E-19  & 7.61E-18  & 5.25E-17  & 5.08E-16  & 2.32E-13  & 2.31E-11  \\
Sc & 21 & 45   & 2.23E-08  & 2.23E-08  & 2.26E-08  & 2.53E-08  & 4.86E-08  & 7.72E-08  & 9.39E-08  & 1.27E-07  & 1.66E-07  & 1.89E-07  & 2.18E-07  & 2.49E-07  & 2.06E-07  \\
Ti & 22 & 46   & 1.59E-09  & 1.60E-09  & 1.61E-09  & 1.66E-09  & 3.55E-09  & 2.77E-07  & 8.22E-07  & 3.18E-06  & 8.31E-06  & 1.29E-05  & 1.98E-05  & 4.83E-05  & 6.26E-05  \\
Ti & 22 & 47   & 1.98E-08  & 1.98E-08  & 1.96E-08  & 1.81E-08  & 4.36E-09  & 1.86E-08  & 3.34E-08  & 7.99E-08  & 1.77E-07  & 2.67E-07  & 4.10E-07  & 1.12E-06  & 2.05E-06  \\
Ti & 22 & 48   & 0.0002    & 0.0002    & 0.0002    & 0.0002    & 0.0002    & 0.0002    & 0.0002    & 0.0001    & 0.0001    & 0.0001    & 0.0001    & 7.70E-05  & 4.86E-05  \\
Ti & 22 & 49   & 4.21E-07  & 4.22E-07  & 4.32E-07  & 5.44E-07  & 4.25E-06  & 5.80E-06  & 6.75E-06  & 8.91E-06  & 1.11E-05  & 1.21E-05  & 1.29E-05  & 1.25E-05  & 1.22E-05  \\
Ti & 22 & 50   & 9.89E-20  & 9.90E-20  & 1.00E-19  & 1.14E-19  & 3.64E-19  & 4.40E-14  & 7.78E-13  & 2.48E-11  & 2.53E-10  & 6.11E-10  & 1.17E-09  & 2.92E-09  & 1.17E-08  \\
V  & 23 & 50   & 1.03E-16  & 1.03E-16  & 1.04E-16  & 1.15E-16  & 4.39E-16  & 2.96E-12  & 1.85E-11  & 2.50E-10  & 1.67E-09  & 3.27E-09  & 4.92E-09  & 1.02E-08  & 5.06E-08  \\
V  & 23 & 51   & 2.93E-06  & 2.93E-06  & 2.93E-06  & 2.89E-06  & 4.98E-07  & 6.29E-06  & 1.02E-05  & 1.82E-05  & 2.72E-05  & 3.26E-05  & 3.88E-05  & 5.65E-05  & 0.0001    \\
Cr & 24 & 50   & 1.99E-07  & 1.99E-07  & 2.02E-07  & 2.30E-07  & 3.17E-07  & 7.46E-06  & 1.77E-05  & 5.29E-05  & 0.0001    & 0.0001    & 0.0002    & 0.0008    & 0.0014    \\
Cr & 24 & 52   & 0.0031    & 0.0031    & 0.0031    & 0.0031    & 0.0031    & 0.0030    & 0.0029    & 0.0026    & 0.0023    & 0.0021    & 0.0019    & 0.0015    & 0.0036    \\
Cr & 24 & 53   & 4.69E-05  & 4.70E-05  & 4.73E-05  & 5.07E-05  & 8.62E-05  & 0.0001    & 0.0001    & 0.0001    & 0.0002    & 0.0002    & 0.0002    & 0.0004    & 0.0008    \\
Cr & 24 & 54   & 3.51E-16  & 3.52E-16  & 3.63E-16  & 4.98E-16  & 1.75E-14  & 6.46E-11  & 3.13E-10  & 2.55E-09  & 1.13E-08  & 2.32E-08  & 5.15E-08  & 5.42E-07  & 3.90E-06  \\
Mn & 25 & 55   & 2.25E-05  & 2.25E-05  & 2.23E-05  & 2.03E-05  & 2.25E-05  & 0.0002    & 0.0004    & 0.0007    & 0.0010    & 0.0011    & 0.0013    & 0.0020    & 0.0033    \\
Fe & 26 & 54   & 1.29E-05  & 1.29E-05  & 1.29E-05  & 1.29E-05  & 1.52E-05  & 0.0007    & 0.0016    & 0.0043    & 0.0090    & 0.0127    & 0.0182    & 0.0427    & 0.0680    \\
Fe & 26 & 56   & 0.0486    & 0.0486    & 0.0486    & 0.0486    & 0.0485    & 0.0470    & 0.0455    & 0.0420    & 0.0378    & 0.0352    & 0.0321    & 0.0241    & 0.0232    \\
Fe & 26 & 57   & 0.0001    & 0.0001    & 0.0001    & 0.0001    & 0.0001    & 0.0002    & 0.0002    & 0.0003    & 0.0004    & 0.0004    & 0.0005    & 0.0006    & 0.0007    \\
Fe & 26 & 58   & 2.64E-14  & 2.64E-14  & 2.69E-14  & 3.19E-14  & 1.96E-13  & 4.31E-11  & 1.46E-10  & 9.14E-10  & 3.70E-09  & 7.43E-09  & 1.57E-08  & 1.22E-07  & 5.50E-07  \\
Co & 27 & 59   & 2.64E-07  & 2.64E-07  & 2.62E-07  & 2.41E-07  & 1.86E-08  & 2.06E-08  & 4.91E-08  & 1.94E-07  & 5.82E-07  & 9.98E-07  & 1.78E-06  & 8.46E-06  & 1.86E-05  \\
Ni & 28 & 58   & 2.46E-05  & 2.47E-05  & 2.47E-05  & 2.55E-05  & 3.20E-05  & 8.12E-05  & 0.0001    & 0.0003    & 0.0006    & 0.0008    & 0.0011    & 0.0024    & 0.0035    \\
Ni & 28 & 60   & 3.76E-07  & 3.75E-07  & 3.69E-07  & 3.11E-07  & 5.88E-09  & 7.91E-09  & 2.97E-08  & 2.18E-07  & 1.01E-06  & 2.14E-06  & 4.70E-06  & 3.64E-05  & 0.0001    \\
Ni & 28 & 61   & 6.87E-10  & 6.86E-10  & 6.77E-10  & 5.90E-10  & 3.60E-11  & 6.52E-12  & 1.46E-11  & 6.66E-11  & 2.57E-10  & 5.33E-10  & 1.19E-09  & 9.71E-09  & 4.84E-08  \\
Ni & 28 & 62   & 5.76E-12  & 5.76E-12  & 5.78E-12  & 5.97E-12  & 7.72E-12  & 1.42E-11  & 2.79E-11  & 8.07E-11  & 1.84E-10  & 3.05E-10  & 5.80E-10  & 4.91E-09  & 3.65E-08  \\
Ni & 28 & 64   & 2.94E-26  & 2.95E-26  & 2.98E-26  & 3.37E-26  & 1.43E-25  & 4.28E-19  & 6.16E-18  & 6.62E-17  & 5.89E-17  & 5.81E-17  & 6.72E-17  & 2.85E-16  & 5.13E-15  \\
Cu & 29 & 63   & 7.49E-15  & 7.50E-15  & 7.61E-15  & 8.87E-15  & 3.62E-14  & 2.36E-14  & 5.45E-14  & 2.54E-13  & 1.16E-12  & 2.75E-12  & 6.94E-12  & 7.07E-11  & 3.37E-10  \\
Cu & 29 & 65   & 3.87E-17  & 3.86E-17  & 3.80E-17  & 3.20E-17  & 3.55E-18  & 8.11E-17  & 1.77E-16  & 5.52E-16  & 1.30E-15  & 2.82E-15  & 6.78E-15  & 5.94E-14  & 2.38E-13  \\
Zn & 30 & 64   & 2.28E-15  & 2.28E-15  & 2.29E-15  & 2.32E-15  & 6.07E-15  & 4.58E-14  & 1.21E-13  & 7.19E-13  & 3.29E-12  & 6.91E-12  & 1.49E-11  & 9.45E-11  & 2.60E-10  \\
Zn & 30 & 66   & 3.70E-18  & 3.70E-18  & 3.66E-18  & 3.31E-18  & 1.56E-18  & 1.10E-15  & 6.38E-15  & 2.18E-14  & 9.51E-15  & 9.05E-15  & 1.60E-14  & 2.08E-13  & 1.29E-12  \\
Zn & 30 & 67   & 1.47E-19  & 1.47E-19  & 1.47E-19  & 1.52E-19  & 1.78E-19  & 4.46E-19  & 1.30E-18  & 2.80E-18  & 1.78E-18  & 2.84E-18  & 6.43E-18  & 5.84E-17  & 2.11E-16  \\
Zn & 30 & 68   & 1.36E-18  & 1.36E-18  & 1.37E-18  & 1.45E-18  & 2.27E-18  & 1.46E-18  & 5.03E-18  & 1.36E-17  & 9.31E-18  & 1.01E-17  & 1.03E-17  & 2.27E-17  & 4.99E-17  \\
Zn & 30 & 70   & 3.18E-32  & 3.06E-32  & 3.14E-32  & 3.31E-32  & 1.08E-31  & 1.39E-26  & 1.57E-25  & 9.29E-25  & 3.22E-24  & 1.19E-23  & 2.91E-23  & 6.82E-25  & 3.63E-26  \\
Ga & 31 & 69   & 3.36E-21  & 3.36E-21  & 3.38E-21  & 3.64E-21  & 6.65E-21  & 1.53E-19  & 6.13E-19  & 9.71E-19  & 4.54E-19  & 3.96E-19  & 2.63E-19  & 1.08E-19  & 6.44E-19  \\
Ga & 31 & 71   & 3.24E-22  & 3.24E-22  & 3.27E-22  & 3.60E-22  & 9.02E-22  & 1.92E-21  & 8.19E-21  & 1.73E-20  & 9.33E-21  & 8.15E-21  & 5.76E-21  & 1.01E-22  & 4.89E-22  \\
Ge & 32 & 70   & 2.40E-20  & 2.41E-20  & 2.44E-20  & 2.85E-20  & 1.39E-19  & 8.74E-18  & 3.37E-17  & 5.68E-17  & 2.41E-17  & 1.67E-17  & 7.31E-18  & 1.45E-18  & 6.70E-18  \\
Ge & 32 & 72   & 4.32E-20  & 4.32E-20  & 4.35E-20  & 4.58E-20  & 6.66E-20  & 9.42E-19  & 3.20E-18  & 5.14E-18  & 3.77E-18  & 3.51E-18  & 1.91E-18  & 1.01E-21  & 2.30E-21  \\
Ge & 32 & 73   & 2.86E-22  & 2.86E-22  & 2.89E-22  & 3.12E-22  & 6.26E-22  & 8.15E-21  & 1.27E-20  & 1.01E-20  & 4.87E-21  & 3.75E-21  & 1.68E-21  & 1.65E-24  & 6.70E-24  \\
Ge & 32 & 74   & 9.23E-28  & 9.25E-28  & 9.43E-28  & 1.14E-27  & 8.43E-27  & 2.36E-23  & 1.24E-22  & 4.18E-22  & 1.34E-21  & 2.81E-21  & 2.67E-21  & 1.71E-24  & 7.21E-27  \\






\hline

\end{tabular}}


==> decayed_dean_yields_new_latex_table.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
  Symbol & Z & A & $^{22}$Ne = 0  & 1e-7 & 1e-6 & 1e-5 & 1e-4 & 1e-3 & 2e-3 & 5e-3 & 1e-2 & 1.4e-2 & 2e-2 & 5e-2 & 1e-1 \\
\hline


O  & 8  & 16   & 0.0537   & 0.0537   & 0.0537   & 0.0537   & 0.0538   & 0.0543   & 0.0548   & 0.0559   & 0.0572   & 0.0579   & 0.0587   & 0.0595   & 0.0568   \\
O  & 8  & 17   & 5.78E-10 & 5.79E-10 & 5.84E-10 & 6.32E-10 & 1.28E-09 & 2.65E-08 & 6.52E-08 & 1.62E-07 & 2.66E-07 & 3.22E-07 & 3.82E-07 & 4.89E-07 & 4.85E-07 \\
O  & 8  & 18   & 5.74E-12 & 5.75E-12 & 5.78E-12 & 6.08E-12 & 1.01E-11 & 1.67E-10 & 4.15E-10 & 1.12E-09 & 2.19E-09 & 3.00E-09 & 4.21E-09 & 1.15E-08 & 4.14E-08 \\
F  & 9  & 19   & 9.12E-10 & 9.11E-10 & 9.07E-10 & 8.67E-10 & 6.37E-10 & 1.92E-10 & 1.32E-10 & 1.43E-10 & 2.42E-10 & 3.40E-10 & 5.01E-10 & 1.34E-09 & 2.24E-09 \\
Ne & 10 & 20   & 0.0016   & 0.0016   & 0.0016   & 0.0016   & 0.0016   & 0.0015   & 0.0015   & 0.0015   & 0.0015   & 0.0014   & 0.0014   & 0.0012   & 0.0010   \\
Ne & 10 & 21   & 1.11E-08 & 1.11E-08 & 1.11E-08 & 1.13E-08 & 1.31E-08 & 6.64E-08 & 1.69E-07 & 5.39E-07 & 1.20E-06 & 1.78E-06 & 2.74E-06 & 9.09E-06 & 2.59E-05 \\
Ne & 10 & 22   & 2.04E-08 & 2.05E-08 & 2.07E-08 & 2.29E-08 & 4.87E-08 & 3.70E-07 & 7.98E-07 & 2.41E-06 & 5.91E-06 & 9.29E-06 & 1.52E-05 & 5.70E-05 & 0.0001   \\
Na & 11 & 23   & 6.64E-06 & 6.64E-06 & 6.64E-06 & 6.63E-06 & 6.50E-06 & 5.96E-06 & 6.03E-06 & 6.75E-06 & 8.76E-06 & 1.07E-05 & 1.39E-05 & 3.60E-05 & 0.0001   \\
Mg & 12 & 24   & 0.0148   & 0.0148   & 0.0148   & 0.0148   & 0.0149   & 0.0144   & 0.0135   & 0.0115   & 0.0092   & 0.0079   & 0.0064   & 0.0036   & 0.0035   \\
Mg & 12 & 25   & 2.09E-07 & 2.09E-07 & 2.09E-07 & 2.12E-07 & 2.52E-07 & 2.82E-06 & 4.56E-06 & 1.03E-05 & 2.19E-05 & 3.28E-05 & 5.16E-05 & 0.0001   & 0.0006   \\
Mg & 12 & 26   & 8.80E-07 & 8.80E-07 & 8.81E-07 & 8.91E-07 & 1.01E-06 & 2.44E-06 & 3.99E-06 & 8.55E-06 & 1.60E-05 & 2.21E-05 & 3.16E-05 & 9.61E-05 & 0.0005   \\
Al & 13 & 27   & 3.95E-05 & 3.95E-05 & 3.95E-05 & 3.95E-05 & 3.89E-05 & 8.91E-05 & 0.0001   & 0.0002   & 0.0004   & 0.0004   & 0.0005   & 0.0006   & 0.0009   \\
Si & 14 & 28   & 0.1649   & 0.1649   & 0.1650   & 0.1650   & 0.1654   & 0.1676   & 0.1685   & 0.1694   & 0.1694   & 0.1690   & 0.1683   & 0.1644   & 0.1564   \\
Si & 14 & 29   & 2.90E-05 & 2.90E-05 & 2.89E-05 & 2.88E-05 & 2.99E-05 & 0.0001   & 0.0001   & 0.0001   & 0.0002   & 0.0003   & 0.0004   & 0.0013   & 0.0049   \\
Si & 14 & 30   & 1.76E-05 & 1.76E-05 & 1.75E-05 & 1.67E-05 & 1.13E-05 & 1.55E-05 & 5.05E-05 & 0.0002   & 0.0005   & 0.0007   & 0.0011   & 0.0031   & 0.0067   \\
P  & 15 & 31   & 4.43E-05 & 4.43E-05 & 4.42E-05 & 4.31E-05 & 3.31E-05 & 2.53E-05 & 3.87E-05 & 7.95E-05 & 0.0001   & 0.0001   & 0.0002   & 0.0004   & 0.0005   \\
S  & 16 & 32   & 0.0941   & 0.0941   & 0.0941   & 0.0941   & 0.0939   & 0.0930   & 0.0927   & 0.0922   & 0.0915   & 0.0908   & 0.0896   & 0.0810   & 0.0645   \\
S  & 16 & 33   & 3.34E-05 & 3.35E-05 & 3.35E-05 & 3.37E-05 & 3.56E-05 & 3.57E-05 & 3.94E-05 & 5.97E-05 & 8.80E-05 & 0.0001   & 0.0001   & 0.0001   & 0.0001   \\
S  & 16 & 34   & 2.92E-06 & 2.92E-06 & 2.90E-06 & 2.74E-06 & 1.58E-06 & 1.79E-05 & 5.51E-05 & 0.0001   & 0.0004   & 0.0006   & 0.0009   & 0.0025   & 0.0043   \\
S  & 16 & 36   & 2.54E-12 & 2.54E-12 & 2.54E-12 & 2.55E-12 & 2.55E-12 & 4.61E-11 & 3.36E-10 & 3.20E-09 & 1.52E-08 & 3.21E-08 & 7.48E-08 & 1.16E-06 & 1.07E-05 \\
Cl & 17 & 35   & 7.20E-06 & 7.20E-06 & 7.18E-06 & 6.98E-06 & 5.39E-06 & 4.58E-06 & 6.27E-06 & 1.30E-05 & 2.40E-05 & 3.27E-05 & 4.50E-05 & 7.83E-05 & 8.10E-05 \\
Cl & 17 & 37   & 1.86E-06 & 1.86E-06 & 1.87E-06 & 1.87E-06 & 1.93E-06 & 2.15E-06 & 2.58E-06 & 3.87E-06 & 5.70E-06 & 6.94E-06 & 8.58E-06 & 1.56E-05 & 2.10E-05 \\
Ar & 18 & 36   & 0.0211   & 0.0211   & 0.0211   & 0.0211   & 0.0210   & 0.0206   & 0.0203   & 0.0200   & 0.0195   & 0.0192   & 0.0186   & 0.0159   & 0.0123   \\
Ar & 18 & 38   & 4.62E-06 & 4.61E-06 & 4.57E-06 & 4.56E-06 & 4.36E-06 & 9.74E-06 & 1.99E-05 & 6.19E-05 & 0.0001   & 0.0002   & 0.0003   & 0.0010   & 0.0018   \\
Ar & 18 & 40   & 6.72E-13 & 6.72E-13 & 6.72E-13 & 6.73E-13 & 6.73E-13 & 1.00E-12 & 2.72E-12 & 1.86E-11 & 9.81E-11 & 2.46E-10 & 7.36E-10 & 1.52E-08 & 7.42E-08 \\
K  & 19 & 39   & 3.80E-06 & 3.79E-06 & 3.78E-06 & 3.76E-06 & 3.56E-06 & 3.86E-06 & 4.67E-06 & 1.06E-05 & 1.72E-05 & 2.15E-05 & 2.69E-05 & 4.79E-05 & 5.43E-05 \\
K  & 19 & 40   & 9.65E-13 & 9.65E-13 & 9.67E-13 & 9.80E-13 & 1.26E-12 & 1.07E-10 & 2.61E-10 & 9.51E-10 & 3.21E-09 & 6.16E-09 & 1.21E-08 & 3.05E-08 & 1.43E-08 \\
K  & 19 & 41   & 1.07E-07 & 1.07E-07 & 1.08E-07 & 1.12E-07 & 1.54E-07 & 3.14E-07 & 4.28E-07 & 7.12E-07 & 1.11E-06 & 1.37E-06 & 1.70E-06 & 2.82E-06 & 2.98E-06 \\
Ca & 20 & 40   & 0.0226   & 0.0226   & 0.0226   & 0.0226   & 0.0225   & 0.0220   & 0.0218   & 0.0212   & 0.0206   & 0.0201   & 0.0195   & 0.0166   & 0.0129   \\
Ca & 20 & 42   & 1.56E-08 & 1.56E-08 & 1.56E-08 & 1.55E-08 & 1.46E-08 & 1.35E-07 & 3.70E-07 & 1.45E-06 & 3.71E-06 & 5.66E-06 & 8.73E-06 & 2.33E-05 & 3.43E-05 \\
Ca & 20 & 43   & 2.83E-07 & 2.82E-07 & 2.80E-07 & 2.79E-07 & 2.64E-07 & 2.14E-07 & 2.29E-07 & 9.72E-07 & 1.35E-06 & 1.39E-06 & 1.36E-06 & 1.05E-06 & 6.59E-07 \\
Ca & 20 & 44   & 3.85E-05 & 3.83E-05 & 3.85E-05 & 3.84E-05 & 3.86E-05 & 4.03E-05 & 4.16E-05 & 4.14E-05 & 3.97E-05 & 3.84E-05 & 3.64E-05 & 2.84E-05 & 1.91E-05 \\
Ca & 20 & 46   & 3.22E-11 & 3.22E-11 & 3.22E-11 & 3.22E-11 & 3.22E-11 & 3.23E-11 & 3.24E-11 & 3.26E-11 & 3.32E-11 & 3.41E-11 & 3.74E-11 & 1.28E-10 & 4.94E-10 \\
Ca & 20 & 48   & 1.21E-12 & 1.21E-12 & 1.21E-12 & 1.21E-12 & 1.21E-12 & 1.22E-12 & 1.22E-12 & 1.23E-12 & 1.25E-12 & 1.26E-12 & 1.29E-12 & 1.46E-12 & 6.41E-12 \\
Sc & 21 & 45   & 1.33E-08 & 1.32E-08 & 1.39E-08 & 1.39E-08 & 1.97E-08 & 4.68E-08 & 5.32E-08 & 6.90E-08 & 9.47E-08 & 1.12E-07 & 1.34E-07 & 1.92E-07 & 2.10E-07 \\
Ti & 22 & 46   & 2.27E-06 & 2.27E-06 & 2.26E-06 & 2.25E-06 & 2.14E-06 & 1.20E-06 & 5.82E-07 & 7.91E-07 & 1.97E-06 & 3.00E-06 & 4.62E-06 & 1.31E-05 & 2.21E-05 \\
Ti & 22 & 47   & 2.98E-06 & 2.98E-06 & 2.96E-06 & 2.95E-06 & 2.80E-06 & 1.52E-06 & 6.89E-07 & 8.23E-07 & 1.24E-06 & 1.40E-06 & 1.52E-06 & 1.65E-06 & 1.65E-06 \\
Ti & 22 & 48   & 0.0006   & 0.0006   & 0.0006   & 0.0006   & 0.0006   & 0.0006   & 0.0006   & 0.0006   & 0.0006   & 0.0005   & 0.0005   & 0.0004   & 0.0003   \\
Ti & 22 & 49   & 3.64E-06 & 3.64E-06 & 3.66E-06 & 3.77E-06 & 5.84E-06 & 1.42E-05 & 1.57E-05 & 1.99E-05 & 2.55E-05 & 2.89E-05 & 3.27E-05 & 4.13E-05 & 4.45E-05 \\
Ti & 22 & 50   & 9.41E-06 & 9.41E-06 & 9.41E-06 & 9.41E-06 & 9.41E-06 & 9.43E-06 & 9.44E-06 & 9.49E-06 & 9.57E-06 & 9.64E-06 & 9.75E-06 & 1.03E-05 & 1.13E-05 \\
V  & 23 & 50   & 9.03E-09 & 9.03E-09 & 9.03E-09 & 9.03E-09 & 9.04E-09 & 9.04E-09 & 9.05E-09 & 9.11E-09 & 9.38E-09 & 9.66E-09 & 1.00E-08 & 1.32E-08 & 3.79E-08 \\
V  & 23 & 51   & 4.07E-05 & 4.07E-05 & 4.05E-05 & 4.05E-05 & 3.89E-05 & 3.79E-05 & 3.92E-05 & 5.28E-05 & 7.32E-05 & 8.59E-05 & 0.0001   & 0.0001   & 0.0002   \\
Cr & 24 & 50   & 5.72E-05 & 5.72E-05 & 5.71E-05 & 5.71E-05 & 5.72E-05 & 5.91E-05 & 6.28E-05 & 8.97E-05 & 0.0001   & 0.0001   & 0.0002   & 0.0006   & 0.0012   \\
Cr & 24 & 52   & 0.0150   & 0.0151   & 0.0150   & 0.0150   & 0.0150   & 0.0149   & 0.0147   & 0.0144   & 0.0138   & 0.0134   & 0.0129   & 0.0112   & 0.0101   \\
Cr & 24 & 53   & 0.0004   & 0.0004   & 0.0004   & 0.0004   & 0.0005   & 0.0006   & 0.0006   & 0.0007   & 0.0009   & 0.0010   & 0.0011   & 0.0015   & 0.0020   \\
Cr & 24 & 54   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   \\
Mn & 25 & 55   & 0.0034   & 0.0034   & 0.0034   & 0.0034   & 0.0034   & 0.0039   & 0.0044   & 0.0054   & 0.0065   & 0.0073   & 0.0082   & 0.0119   & 0.0166   \\
Fe & 26 & 54   & 0.0332   & 0.0332   & 0.0332   & 0.0332   & 0.0332   & 0.0340   & 0.0351   & 0.0386   & 0.0447   & 0.0497   & 0.0573   & 0.0959   & 0.1581   \\
Fe & 26 & 56   & 0.8683   & 0.8684   & 0.8683   & 0.8683   & 0.8680   & 0.8655   & 0.8629   & 0.8552   & 0.8425   & 0.8324   & 0.8177   & 0.7465   & 0.6349   \\
Fe & 26 & 57   & 0.0114   & 0.0114   & 0.0114   & 0.0114   & 0.0115   & 0.0126   & 0.0138   & 0.0157   & 0.0174   & 0.0187   & 0.0203   & 0.0265   & 0.0320   \\
Fe & 26 & 58   & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0010   & 0.0010   \\
Co & 27 & 59   & 0.0013   & 0.0013   & 0.0013   & 0.0013   & 0.0012   & 0.0009   & 0.0006   & 0.0006   & 0.0007   & 0.0008   & 0.0009   & 0.0011   & 0.0012   \\
Ni & 28 & 58   & 0.0304   & 0.0304   & 0.0304   & 0.0304   & 0.0304   & 0.0306   & 0.0307   & 0.0329   & 0.0391   & 0.0441   & 0.0518   & 0.0902   & 0.1536   \\
Ni & 28 & 60   & 0.0150   & 0.0150   & 0.0150   & 0.0150   & 0.0150   & 0.0150   & 0.0150   & 0.0148   & 0.0140   & 0.0136   & 0.0131   & 0.0109   & 0.0086   \\
Ni & 28 & 61   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0002   & 0.0002   & 0.0002   & 0.0003   & 0.0003   & 0.0003   & 0.0003   & 0.0003   \\
Ni & 28 & 62   & 0.0008   & 0.0008   & 0.0008   & 0.0008   & 0.0008   & 0.0008   & 0.0009   & 0.0014   & 0.0020   & 0.0025   & 0.0032   & 0.0060   & 0.0092   \\
Ni & 28 & 64   & 9.48E-07 & 9.48E-07 & 9.48E-07 & 9.48E-07 & 9.49E-07 & 9.50E-07 & 9.51E-07 & 9.56E-07 & 9.63E-07 & 9.69E-07 & 9.78E-07 & 1.03E-06 & 1.12E-06 \\
Cu & 29 & 63   & 1.12E-05 & 1.12E-05 & 1.12E-05 & 1.12E-05 & 1.09E-05 & 8.35E-06 & 9.78E-06 & 2.12E-06 & 1.82E-06 & 1.87E-06 & 2.04E-06 & 3.83E-06 & 7.89E-06 \\
Cu & 29 & 65   & 1.17E-06 & 1.17E-06 & 1.17E-06 & 1.18E-06 & 1.20E-06 & 1.45E-06 & 1.69E-06 & 1.67E-06 & 1.92E-06 & 2.14E-06 & 2.44E-06 & 3.28E-06 & 3.00E-06 \\
Zn & 30 & 64   & 0.0002   & 0.0002   & 0.0002   & 0.0002   & 0.0002   & 0.0002   & 0.0002   & 6.40E-05 & 3.77E-05 & 3.23E-05 & 2.79E-05 & 1.82E-05 & 1.05E-05 \\
Zn & 30 & 66   & 3.77E-06 & 3.77E-06 & 3.77E-06 & 3.78E-06 & 3.91E-06 & 5.76E-06 & 8.47E-06 & 1.50E-05 & 2.52E-05 & 3.32E-05 & 4.45E-05 & 8.82E-05 & 0.0001   \\
Zn & 30 & 67   & 4.10E-08 & 4.10E-08 & 4.09E-08 & 4.11E-08 & 4.21E-08 & 5.30E-08 & 5.04E-08 & 5.35E-09 & 1.15E-08 & 1.82E-08 & 2.95E-08 & 9.18E-08 & 1.70E-07 \\
Zn & 30 & 68   & 3.21E-06 & 3.20E-06 & 3.18E-06 & 3.19E-06 & 3.16E-06 & 2.47E-06 & 1.21E-06 & 9.29E-08 & 4.83E-08 & 4.10E-08 & 3.61E-08 & 3.59E-08 & 8.78E-08 \\
Zn & 30 & 70   & 9.92E-14 & 9.92E-14 & 9.92E-14 & 9.92E-14 & 9.92E-14 & 9.94E-14 & 9.96E-14 & 1.00E-13 & 1.01E-13 & 1.02E-13 & 1.03E-13 & 1.09E-13 & 1.20E-13 \\
Ga & 31 & 69   & 1.06E-08 & 1.06E-08 & 1.05E-08 & 1.05E-08 & 1.05E-08 & 9.50E-09 & 7.86E-09 & 7.32E-09 & 8.09E-09 & 8.62E-09 & 9.14E-09 & 9.41E-09 & 7.67E-09 \\
Ga & 31 & 71   & 3.34E-11 & 3.34E-11 & 3.32E-11 & 3.33E-11 & 3.33E-11 & 3.35E-11 & 3.24E-11 & 1.57E-10 & 5.38E-10 & 8.78E-10 & 1.41E-09 & 3.76E-09 & 5.42E-09 \\
Ge & 32 & 70   & 3.63E-08 & 3.63E-08 & 3.61E-08 & 3.62E-08 & 3.71E-08 & 4.67E-08 & 5.81E-08 & 9.06E-08 & 1.47E-07 & 1.93E-07 & 2.58E-07 & 5.13E-07 & 7.06E-07 \\
Ge & 32 & 72   & 5.96E-09 & 5.95E-09 & 5.88E-09 & 5.88E-09 & 5.67E-09 & 3.39E-09 & 1.31E-09 & 6.64E-11 & 6.68E-11 & 9.94E-11 & 1.84E-10 & 1.37E-09 & 6.04E-09 \\
Ge & 32 & 73   & 8.98E-11 & 8.96E-11 & 8.85E-11 & 8.88E-11 & 8.83E-11 & 8.26E-11 & 8.55E-11 & 8.67E-11 & 7.50E-11 & 7.60E-11 & 7.68E-11 & 6.87E-11 & 4.83E-11 \\
Ge & 32 & 74   & 1.27E-14 & 1.27E-14 & 1.27E-14 & 1.27E-14 & 1.27E-14 & 1.27E-14 & 1.27E-14 & 1.28E-14 & 1.29E-14 & 1.30E-14 & 1.31E-14 & 1.38E-14 & 1.52E-14 \\





\hline

\end{tabular}}


==> decayed_shen_yields_new_latex_table.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
  Symbol & Z & A & $^{22}$Ne = 0  & 1e-7 & 1e-6 & 1e-5 & 1e-4 & 1e-3 & 2e-3 & 5e-3 & 1e-2 & 1.4e-2 & 2e-2 & 5e-2 & 1e-1 \\
\hline




O  & 8  & 16  & 0.0480   & 0.0480   & 0.0480   & 0.0481   & 0.0484   & 0.0497   & 0.0504   & 0.0519   & 0.0534   & 0.0541   & 0.0547   & 0.0547   & 0.0511   \\
O  & 8  & 17  & 3.35E-10 & 3.36E-10 & 3.42E-10 & 3.96E-10 & 1.39E-09 & 2.34E-08 & 4.26E-08 & 7.10E-08 & 8.66E-08 & 9.27E-08 & 9.97E-08 & 1.06E-07 & 9.60E-08 \\
O  & 8  & 18  & 5.01E-12 & 5.01E-12 & 5.07E-12 & 5.65E-12 & 1.39E-11 & 1.17E-10 & 1.91E-10 & 3.65E-10 & 6.22E-10 & 7.95E-10 & 1.12E-09 & 7.37E-09 & 3.11E-08 \\
F  & 9  & 19  & 1.50E-10 & 1.50E-10 & 1.49E-10 & 1.41E-10 & 9.52E-11 & 2.80E-11 & 3.47E-11 & 6.99E-11 & 1.10E-10 & 1.43E-10 & 2.16E-10 & 4.80E-10 & 5.26E-10 \\
Ne & 10 & 20  & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0004   & 0.0004   & 0.0004   & 0.0004   & 0.0003   & 0.0003   \\
Ne & 10 & 21  & 3.69E-09 & 3.69E-09 & 3.70E-09 & 3.79E-09 & 4.92E-09 & 4.63E-08 & 1.29E-07 & 3.55E-07 & 6.17E-07 & 8.42E-07 & 1.36E-06 & 4.63E-06 & 1.06E-05 \\
Ne & 10 & 22  & 6.62E-09 & 6.62E-09 & 6.62E-09 & 6.66E-09 & 9.37E-09 & 1.30E-07 & 3.44E-07 & 1.30E-06 & 3.55E-06 & 5.66E-06 & 9.27E-06 & 3.48E-05 & 9.71E-05 \\
Na & 11 & 23  & 2.78E-06 & 2.78E-06 & 2.78E-06 & 2.77E-06 & 2.68E-06 & 2.36E-06 & 2.38E-06 & 2.86E-06 & 3.88E-06 & 4.86E-06 & 6.78E-06 & 1.75E-05 & 4.45E-05 \\
Mg & 12 & 24  & 0.0074   & 0.0074   & 0.0074   & 0.0074   & 0.0074   & 0.0069   & 0.0062   & 0.0045   & 0.0030   & 0.0023   & 0.0017   & 0.0009   & 0.0011   \\
Mg & 12 & 25  & 9.76E-08 & 9.75E-08 & 9.78E-08 & 9.96E-08 & 1.29E-07 & 1.28E-06 & 2.01E-06 & 4.46E-06 & 9.19E-06 & 1.37E-05 & 2.12E-05 & 7.10E-05 & 0.0002   \\
Mg & 12 & 26  & 3.32E-07 & 3.33E-07 & 3.33E-07 & 3.38E-07 & 3.99E-07 & 1.04E-06 & 1.68E-06 & 3.46E-06 & 6.28E-06 & 8.48E-06 & 1.18E-05 & 3.42E-05 & 0.0001   \\
Al & 13 & 27  & 1.74E-05 & 1.74E-05 & 1.74E-05 & 1.73E-05 & 1.61E-05 & 4.20E-05 & 7.16E-05 & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0003   \\
Si & 14 & 28  & 0.1887   & 0.1887   & 0.1888   & 0.1888   & 0.1893   & 0.1923   & 0.1936   & 0.1946   & 0.1943   & 0.1939   & 0.1933   & 0.1911   & 0.1851   \\
Si & 14 & 29  & 2.55E-05 & 2.55E-05 & 2.55E-05 & 2.53E-05 & 2.62E-05 & 9.41E-05 & 0.0001   & 0.0001   & 0.0001   & 0.0002   & 0.0002   & 0.0005   & 0.0023   \\
Si & 14 & 30  & 1.36E-05 & 1.36E-05 & 1.35E-05 & 1.25E-05 & 5.82E-06 & 1.19E-05 & 3.82E-05 & 0.0001   & 0.0002   & 0.0004   & 0.0006   & 0.0018   & 0.0057   \\
P  & 15 & 31  & 2.93E-05 & 2.93E-05 & 2.91E-05 & 2.81E-05 & 1.98E-05 & 2.31E-05 & 3.57E-05 & 6.91E-05 & 0.0001   & 0.0001   & 0.0001   & 0.0003   & 0.0005   \\
S  & 16 & 32  & 0.1095   & 0.1095   & 0.1095   & 0.1095   & 0.1091   & 0.1074   & 0.1069   & 0.1063   & 0.1053   & 0.1043   & 0.1025   & 0.0905   & 0.0714   \\
S  & 16 & 33  & 1.59E-05 & 1.59E-05 & 1.59E-05 & 1.62E-05 & 1.95E-05 & 3.35E-05 & 4.31E-05 & 6.81E-05 & 9.91E-05 & 0.0001   & 0.0001   & 0.0002   & 0.0002   \\
S  & 16 & 34  & 2.04E-06 & 2.03E-06 & 2.02E-06 & 1.85E-06 & 7.16E-07 & 3.58E-05 & 0.0001   & 0.0003   & 0.0007   & 0.0010   & 0.0015   & 0.0041   & 0.0076   \\
S  & 16 & 36  & 6.84E-15 & 6.85E-15 & 6.88E-15 & 7.19E-15 & 1.31E-14 & 4.00E-11 & 2.38E-10 & 1.88E-09 & 7.90E-09 & 1.70E-08 & 3.96E-08 & 5.92E-07 & 5.30E-06 \\
Cl & 17 & 35  & 5.30E-06 & 5.30E-06 & 5.28E-06 & 5.08E-06 & 3.78E-06 & 6.70E-06 & 1.07E-05 & 2.18E-05 & 3.81E-05 & 5.03E-05 & 6.65E-05 & 0.0001   & 0.0001   \\
Cl & 17 & 37  & 1.33E-06 & 1.34E-06 & 1.34E-06 & 1.38E-06 & 1.76E-06 & 3.30E-06 & 4.43E-06 & 7.17E-06 & 1.07E-05 & 1.31E-05 & 1.62E-05 & 2.60E-05 & 2.96E-05 \\
Ar & 18 & 36  & 0.0237   & 0.0237   & 0.0237   & 0.0237   & 0.0235   & 0.0227   & 0.0223   & 0.0217   & 0.0211   & 0.0206   & 0.0199   & 0.0164   & 0.0122   \\
Ar & 18 & 38  & 1.21E-06 & 1.21E-06 & 1.22E-06 & 1.23E-06 & 1.12E-06 & 1.83E-05 & 4.67E-05 & 0.0001   & 0.0003   & 0.0005   & 0.0008   & 0.0021   & 0.0035   \\
Ar & 18 & 40  & 1.77E-16 & 1.77E-16 & 1.78E-16 & 1.85E-16 & 2.81E-16 & 5.47E-13 & 2.81E-12 & 1.97E-11 & 9.77E-11 & 2.39E-10 & 6.73E-10 & 1.09E-08 & 6.34E-08 \\
K  & 19 & 39  & 2.06E-06 & 2.06E-06 & 2.06E-06 & 2.04E-06 & 1.84E-06 & 5.80E-06 & 9.63E-06 & 2.00E-05 & 3.35E-05 & 4.28E-05 & 5.48E-05 & 8.94E-05 & 8.87E-05 \\
K  & 19 & 40  & 4.45E-13 & 4.46E-13 & 4.47E-13 & 4.65E-13 & 8.19E-13 & 2.31E-10 & 5.28E-10 & 1.72E-09 & 4.90E-09 & 8.45E-09 & 1.48E-08 & 3.38E-08 & 2.67E-08 \\
K  & 19 & 41  & 1.99E-07 & 2.00E-07 & 2.00E-07 & 2.09E-07 & 2.98E-07 & 6.20E-07 & 8.66E-07 & 1.46E-06 & 2.23E-06 & 2.73E-06 & 3.33E-06 & 4.82E-06 & 4.37E-06 \\
Ca & 20 & 40  & 0.0242   & 0.0242   & 0.0242   & 0.0242   & 0.0240   & 0.0231   & 0.0225   & 0.0217   & 0.0208   & 0.0202   & 0.0193   & 0.0158   & 0.0120   \\
Ca & 20 & 42  & 5.48E-09 & 5.48E-09 & 5.48E-09 & 5.38E-09 & 3.44E-09 & 3.21E-07 & 9.14E-07 & 3.31E-06 & 8.39E-06 & 1.30E-05 & 2.04E-05 & 5.18E-05 & 7.03E-05 \\
Ca & 20 & 43  & 7.69E-08 & 7.68E-08 & 7.68E-08 & 7.48E-08 & 5.40E-08 & 4.17E-08 & 7.78E-08 & 3.04E-07 & 3.57E-07 & 3.54E-07 & 3.36E-07 & 2.40E-07 & 1.62E-07 \\
Ca & 20 & 44  & 2.41E-05 & 2.43E-05 & 2.40E-05 & 2.41E-05 & 2.40E-05 & 2.39E-05 & 2.36E-05 & 2.21E-05 & 2.07E-05 & 1.98E-05 & 1.86E-05 & 1.38E-05 & 9.18E-06 \\
Ca & 20 & 46  & 6.31E-22 & 6.32E-22 & 6.40E-22 & 7.33E-22 & 2.91E-21 & 2.85E-17 & 4.86E-16 & 1.70E-14 & 2.61E-13 & 1.06E-12 & 4.61E-12 & 9.42E-11 & 6.21E-10 \\
Ca & 20 & 48  & 5.82E-30 & 5.84E-30 & 5.98E-30 & 7.69E-30 & 7.71E-29 & 1.75E-23 & 1.21E-21 & 1.08E-19 & 3.78E-18 & 3.11E-17 & 1.81E-16 & 4.78E-14 & 4.63E-12 \\
Sc & 21 & 45  & 1.63E-08 & 1.66E-08 & 1.61E-08 & 1.72E-08 & 2.88E-08 & 5.77E-08 & 6.80E-08 & 9.23E-08 & 1.21E-07 & 1.39E-07 & 1.59E-07 & 1.98E-07 & 1.96E-07 \\
Ti & 22 & 46  & 4.41E-07 & 4.39E-07 & 4.42E-07 & 4.49E-07 & 4.16E-07 & 2.80E-07 & 4.46E-07 & 1.69E-06 & 4.36E-06 & 6.68E-06 & 1.02E-05 & 2.47E-05 & 3.44E-05 \\
Ti & 22 & 47  & 6.67E-07 & 6.65E-07 & 6.70E-07 & 6.78E-07 & 6.19E-07 & 2.46E-07 & 1.36E-07 & 3.08E-07 & 4.61E-07 & 5.44E-07 & 6.44E-07 & 9.85E-07 & 1.42E-06 \\
Ti & 22 & 48  & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0004   & 0.0004   & 0.0004   & 0.0004   & 0.0003   & 0.0002   \\
Ti & 22 & 49  & 2.41E-06 & 2.42E-06 & 2.43E-06 & 2.62E-06 & 5.31E-06 & 1.12E-05 & 1.25E-05 & 1.60E-05 & 2.07E-05 & 2.35E-05 & 2.66E-05 & 3.34E-05 & 3.63E-05 \\
Ti & 22 & 50  & 4.21E-20 & 4.22E-20 & 4.27E-20 & 4.77E-20 & 1.33E-19 & 2.22E-14 & 3.58E-13 & 9.33E-12 & 8.13E-11 & 1.93E-10 & 3.78E-10 & 1.08E-09 & 6.71E-09 \\
V  & 23 & 50  & 6.22E-17 & 6.24E-17 & 6.29E-17 & 6.86E-17 & 2.07E-16 & 1.25E-12 & 7.90E-12 & 9.85E-11 & 6.11E-10 & 1.22E-09 & 1.97E-09 & 6.39E-09 & 3.84E-08 \\
V  & 23 & 51  & 1.09E-05 & 1.09E-05 & 1.09E-05 & 1.08E-05 & 8.85E-06 & 1.20E-05 & 1.72E-05 & 3.18E-05 & 4.91E-05 & 5.99E-05 & 7.32E-05 & 0.0001   & 0.0001   \\
Cr & 24 & 50  & 4.13E-06 & 4.11E-06 & 4.14E-06 & 4.20E-06 & 4.27E-06 & 8.04E-06 & 1.59E-05 & 4.76E-05 & 0.0001   & 0.0001   & 0.0002   & 0.0006   & 0.0012   \\
Cr & 24 & 52  & 0.0113   & 0.0113   & 0.0113   & 0.0113   & 0.0113   & 0.0112   & 0.0111   & 0.0107   & 0.0102   & 0.0099   & 0.0095   & 0.0080   & 0.0076   \\
Cr & 24 & 53  & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0002   & 0.0003   & 0.0003   & 0.0004   & 0.0005   & 0.0006   & 0.0007   & 0.0011   & 0.0015   \\
Cr & 24 & 54  & 4.79E-16 & 4.94E-16 & 5.05E-16 & 6.69E-16 & 1.44E-14 & 3.97E-11 & 2.05E-10 & 1.72E-09 & 7.84E-09 & 1.64E-08 & 3.62E-08 & 3.80E-07 & 2.78E-06 \\
Mn & 25 & 55  & 7.70E-05 & 7.73E-05 & 7.70E-05 & 7.62E-05 & 8.74E-05 & 0.0006   & 0.0010   & 0.0018   & 0.0028   & 0.0034   & 0.0042   & 0.0069   & 0.0102   \\
Fe & 26 & 54  & 3.20E-05 & 3.21E-05 & 3.21E-05 & 3.19E-05 & 3.65E-05 & 0.0007   & 0.0018   & 0.0051   & 0.0108   & 0.0154   & 0.0225   & 0.0563   & 0.1050   \\
Fe & 26 & 56  & 0.5678   & 0.5678   & 0.5678   & 0.5677   & 0.5675   & 0.5653   & 0.5632   & 0.5572   & 0.5479   & 0.5407   & 0.5303   & 0.4822   & 0.4099   \\
Fe & 26 & 57  & 0.0038   & 0.0038   & 0.0038   & 0.0038   & 0.0039   & 0.0048   & 0.0057   & 0.0067   & 0.0079   & 0.0088   & 0.0099   & 0.0142   & 0.0182   \\
Fe & 26 & 58  & 1.83E-14 & 1.83E-14 & 1.85E-14 & 2.09E-14 & 9.46E-14 & 1.97E-11 & 8.31E-11 & 5.90E-10 & 2.50E-09 & 5.07E-09 & 1.07E-08 & 8.44E-08 & 3.90E-07 \\
Co & 27 & 59  & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0005   & 0.0002   & 4.39E-05 & 0.0001   & 0.0002   & 0.0002   & 0.0003   & 0.0004   & 0.0004   \\
Ni & 28 & 58  & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0009   & 0.0007   & 0.0005   & 0.0023   & 0.0061   & 0.0092   & 0.0138   & 0.0384   & 0.0813   \\
Ni & 28 & 60  & 0.0059   & 0.0059   & 0.0059   & 0.0059   & 0.0059   & 0.0059   & 0.0061   & 0.0057   & 0.0053   & 0.0051   & 0.0048   & 0.0035   & 0.0018   \\
Ni & 28 & 61  & 7.03E-05 & 7.02E-05 & 7.03E-05 & 7.07E-05 & 7.21E-05 & 8.88E-05 & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   \\
Ni & 28 & 62  & 3.43E-05 & 3.42E-05 & 3.43E-05 & 3.45E-05 & 3.40E-05 & 3.78E-05 & 0.0001   & 0.0003   & 0.0007   & 0.0009   & 0.0013   & 0.0028   & 0.0035   \\
Ni & 28 & 64  & 2.60E-23 & 2.60E-23 & 2.60E-23 & 2.63E-23 & 2.82E-23 & 8.17E-20 & 1.68E-18 & 2.26E-17 & 2.58E-17 & 2.77E-17 & 3.36E-17 & 2.53E-16 & 4.62E-15 \\
Cu & 29 & 63  & 5.19E-06 & 5.18E-06 & 5.19E-06 & 5.21E-06 & 5.01E-06 & 4.56E-06 & 8.11E-06 & 3.31E-07 & 3.16E-07 & 3.64E-07 & 4.73E-07 & 1.28E-06 & 2.37E-06 \\
Cu & 29 & 65  & 5.16E-07 & 5.15E-07 & 5.16E-07 & 5.21E-07 & 5.34E-07 & 6.70E-07 & 6.53E-07 & 6.10E-07 & 7.02E-07 & 7.72E-07 & 8.56E-07 & 9.28E-07 & 5.09E-07 \\
Zn & 30 & 64  & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 0.0001   & 8.38E-05 & 2.09E-05 & 1.39E-05 & 1.20E-05 & 1.03E-05 & 5.83E-06 & 2.12E-06 \\
Zn & 30 & 66  & 1.29E-06 & 1.29E-06 & 1.29E-06 & 1.31E-06 & 1.39E-06 & 2.38E-06 & 3.45E-06 & 6.05E-06 & 1.04E-05 & 1.37E-05 & 1.81E-05 & 3.09E-05 & 2.65E-05 \\
Zn & 30 & 67  & 2.12E-08 & 2.12E-08 & 2.12E-08 & 2.14E-08 & 2.20E-08 & 2.35E-08 & 1.02E-08 & 1.37E-09 & 3.66E-09 & 5.75E-09 & 9.03E-09 & 2.30E-08 & 2.59E-08 \\
Zn & 30 & 68  & 1.08E-06 & 1.08E-06 & 1.09E-06 & 1.10E-06 & 1.06E-06 & 5.48E-07 & 1.17E-07 & 1.93E-08 & 1.18E-08 & 1.01E-08 & 8.78E-09 & 9.49E-09 & 2.32E-08 \\
Zn & 30 & 70  & 1.40E-30 & 1.40E-30 & 1.40E-30 & 1.46E-30 & 2.41E-30 & 5.45E-27 & 1.12E-25 & 2.45E-24 & 1.92E-23 & 5.58E-23 & 9.28E-23 & 9.14E-25 & 5.14E-26 \\
Ga & 31 & 69  & 3.43E-09 & 3.42E-09 & 3.44E-09 & 3.48E-09 & 3.42E-09 & 2.58E-09 & 2.06E-09 & 1.95E-09 & 1.97E-09 & 1.98E-09 & 1.97E-09 & 1.54E-09 & 7.93E-10 \\
Ga & 31 & 71  & 7.23E-12 & 7.21E-12 & 7.25E-12 & 7.35E-12 & 7.30E-12 & 6.01E-12 & 3.79E-12 & 3.07E-11 & 7.46E-11 & 1.10E-10 & 1.59E-10 & 2.71E-10 & 1.54E-10 \\
Ge & 32 & 70  & 1.04E-08 & 1.04E-08 & 1.04E-08 & 1.06E-08 & 1.09E-08 & 1.38E-08 & 1.74E-08 & 2.78E-08 & 4.55E-08 & 5.88E-08 & 7.64E-08 & 1.21E-07 & 8.71E-08 \\
Ge & 32 & 72  & 1.11E-09 & 1.10E-09 & 1.11E-09 & 1.13E-09 & 1.06E-09 & 4.07E-10 & 5.94E-11 & 6.47E-12 & 1.25E-11 & 2.42E-11 & 5.27E-11 & 3.68E-10 & 7.71E-10 \\
Ge & 32 & 73  & 1.80E-11 & 1.80E-11 & 1.81E-11 & 1.85E-11 & 1.81E-11 & 1.53E-11 & 1.60E-11 & 7.70E-12 & 6.35E-12 & 6.05E-12 & 5.66E-12 & 3.74E-12 & 1.64E-12 \\
Ge & 32 & 74  & 5.39E-27 & 5.39E-27 & 5.38E-27 & 6.00E-27 & 1.61E-26 & 1.92E-24 & 9.93E-24 & 1.44E-22 & 1.35E-21 & 2.55E-21 & 2.06E-21 & 1.25E-24 & 1.20E-26 \\




\hline

\end{tabular}}


==> model_comparisons_for_Type_Ias.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\@setckpt{Chandpters/model_comparisons_for_Type_Ias}{
\setcounter{page}{3}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{1}
\setcounter{affil}{7}
\setcounter{collab}{0}
\setcounter{linecount}{0}
\setcounter{part}{0}
\setcounter{section}{3}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{video}{0}
\setcounter{NAT@ctr}{0}
\setcounter{front@matter@foot@note}{0}
\setcounter{lastfootnote}{0}
\setcounter{remember@figure@num}{0}
\setcounter{remember@table@num}{0}
\setcounter{table@save}{0}
\setcounter{deluxe@table@num}{0}
\setcounter{LT@tables}{0}
\setcounter{LT@chunks}{0}
\setcounter{Item}{0}
\setcounter{Hfootnote}{0}
\setcounter{bookmark@seq@number}{3}
\setcounter{linenumber}{46}
\setcounter{LN@truepage}{2}
\setcounter{section@level}{1}
}


==> q.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\@setckpt{Chandpters/model_comparisons_for_Type_Ias}{
\setcounter{page}{3}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{1}
\setcounter{affil}{7}
\setcounter{collab}{0}
\setcounter{linecount}{0}
\setcounter{part}{0}
\setcounter{section}{3}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{video}{0}
\setcounter{NAT@ctr}{0}
\setcounter{front@matter@foot@note}{0}
\setcounter{lastfootnote}{0}
\setcounter{remember@figure@num}{0}
\setcounter{remember@table@num}{0}
\setcounter{table@save}{0}
\setcounter{deluxe@table@num}{0}
\setcounter{LT@tables}{0}
\setcounter{LT@chunks}{0}
\setcounter{Item}{0}
\setcounter{Hfootnote}{0}
\setcounter{bookmark@seq@number}{3}
\setcounter{linenumber}{46}
\setcounter{LN@truepage}{2}
\setcounter{section@level}{1}
}

